From Random Search to Bandit Learning in Metric Measure Spaces

Random Search is one of the most widely-used method for Hyperparameter Optimization, and is critical to the success of deep learning models. Despite its astonishing performance, little non-heuristic theory has been developed to describe the underlying working mechanism. This paper gives a theoretical accounting of Random Search. We introduce the concept of \emph{scattering dimension} that describes the landscape of the underlying function, and quantifies the performance of random search. We show that, when the environment is noise-free, the output of random search converges to the optimal value in probability at rate $ \widetilde{\mathcal{O}} \left( \left( \frac{1}{T} \right)^{ \frac{1}{d_s} } \right) $, where $ d_s \ge 0 $ is the scattering dimension of the underlying function. When the observed function values are corrupted by bounded $iid$ noise, the output of random search converges to the optimal value in probability at rate $ \widetilde{\mathcal{O}} \left( \left( \frac{1}{T} \right)^{ \frac{1}{d_s + 1} } \right) $. In addition, based on the principles of random search, we introduce an algorithm, called BLiN-MOS, for Lipschitz bandits in doubling metric spaces that are also endowed with a probability measure, and show that under mild conditions, BLiN-MOS achieves a regret rate of order $ \widetilde{\mathcal{O}} \left( T^{ \frac{d_z}{d_z + 1} } \right) $, where $d_z$ is the zooming dimension of the problem instance.

==> tex/algo-sketch.tex <==
\section{Nonconvex Optimization via CVaR Estimation, A Bandit Perspective} 

Suppose that $f$ is $1$-Lipschitz and all function evaluations are noiseless. 


For any cube $ q \subseteq \R^n $, the uniform random variable over $q$ (denoted $X_q$) induces a random variable $f (X_q)$. By Lipschitzness of $f$, we know that the range of $ f (X_q)  $, up to proper shifting, is contained in the interval $ [0, \D (q) ] $, where $ \D (q)$ is the diameter of $q$. 


\begin{assumption} 
    \label{assumption}
    For any cube $q$, let $X_q$ be the uniform random variable over $q$. Suppose that the function $f$ is $L$-Lipschitz on $[0,1]^d$ that satisfies the following conditions. 
    \begin{itemize} 
        \item There exists $\kappa_-, \kappa_+ > 0$ such that $ \kappa_- (1-\alpha) \D (q) \le \max_{x \in q} f (x) - \mathrm{CVaR}_\alpha ( f (X|_{q}) ) \le \kappa_+ (1-\alpha) \D (q) , \quad \forall \alpha \in (0,1) $. For notational simplicity, we also assume $\kappa_+ \ge 1$. 
        \item Let $p_{f(X|_q)}$ be the density function of the random variable $ f (X|_q) $. There exists $\nu >0$, such that $ p_{f(X|_q)} \ge \nu \D (q)^{-1} $. 
    \end{itemize} 
    % \begin{align*} 
    %     \max_{x \in q} f (x) - \mathrm{VaR}_\alpha (X|_{q}) \le \kappa (1-\alpha) \D (q) . 
    % \end{align*} 
\end{assumption} 


\begin{lemma}[Roman Vershynin(2020)]
    \label{lm1}
    $$
    ||X||_{\psi_2} := \inf \{t>0: \mathbb{E}\left[\exp \left(\frac{X^2}{t^2}\right)\right] \leq 2\}
    $$
    Consider a random vector $X \sim Unif([0,1]^n)$ and a Lipschitz function $f:[0,1]^n \rightarrow \mathbb{R}$, then 
    \begin{equation}
    \label{lm1eq1}
    ||f(X) - \mathbb{E}[f(X)]||_{\psi_2} \leq C ||f||_{Lip}
    \end{equation}
\end{lemma}

\begin{corollary}
    If $q$ is a cube with diameter $D(q)$, $X$ is a uniform random variable over $q$, and $f$ is a Lipschitz function with Lipschitz constant $L$ over $q$, then $f(X)$ is a $\frac{CD(q)}{L}$ - sub gaussian random variable, where $C$ is a constant.
\end{corollary}
\begin{proof}
    By Lemma\ref{lm1}, it holds that
    $$
    \mathbb{E}\left[\exp \left(\frac{\left(f(X)-\mathbb{E}f(X) \right)^2}{\frac{CL^2}{D(q)^2}} \right)\right] \leq 2.
    $$
    By Markov's inequality, 
    $$
    \begin{aligned}
    && \mathbb{P} \{ |f(X)-\mathbb{E}f(X)| \geq t\} & =  \mathbb{P} \{ (\exp(|f(X)-\mathbb{E}f(X)|^2))^{CL^2/D(q)^2} \geq (\exp(t^2))^{CL^2/D(q)^2}\}  \\
    && & \leq \exp\left(-\frac{t^2D(q)^2}{CL^2}\right)  \mathbb{E}\left[\exp \left(\frac{\left(f(X)-\mathbb{E}f(X) \right)^2}{\frac{CL^2}{D(q)^2}} \right)\right].
    \end{aligned}
    $$
    Therefore, 
    $$
    \forall t > 0,\enspace \mathbb{P} \{ |f(X)-\mathbb{E}f(X)| \geq t\} \leq 2\exp\left(-\frac{Ct^2D(q)^2}{L^2}\right)
    $$
\end{proof}

% ----------------------------------------------------

For simplicity, write $ f_q^* := \max_{x \in q} f (x) $ for any cube $q $. Let $ \wh{c}_{n,\alpha} (f (X_q)) $ be the $n$-sample estimator of $ \mathrm{CVaR}_\alpha ( f (X_q) )$. Apply Theorem \ref{thm:cvar-concen} to the distribution $f (X_q)$ with $ \epsilon = \delta =  \frac{1}{2} \( f_q^* - \mathrm{CVaR}_\alpha (f(X_q)) \) $ gives the following lemma.  
\begin{lemma}
    \label{lem:concen}
    Instate Assumption \ref{assumption}. Let $f$ be 1-Lipschitz. Let $ n $ and $\epsilon$ be two numbers such that $ ??? $. Then it holds that, for any cube $q \subseteq [0,1]^d$,  
    \begin{align*} 
        &\Pr \( \left| \wh{c}_{n, 1-(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4}} (f(X_q)) - \mathrm{CVaR}_{1-(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4}} (f(X_q)) \right| \le 2 \kappa_+  \( \frac{ \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n } \)^{1/4} \D (q) \) \ge 1- \epsilon \\ 
        &\Pr \( f_q^* - \wh{c}_{n, 1-(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4}} (f (X_q)) \le 6 \kappa_+  \( \frac{ \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n } \)^{1/4} \D (q) \) \ge 1 - \epsilon . 
    \end{align*} 
\end{lemma} 

\begin{proof} 
    We apply Theorem \ref{thm:cvar-concen} to the distribution $f (X_q)$ with $ \epsilon = \delta =  \frac{1}{2} \( f_q^* - \mathrm{CVaR}_\alpha (X_q) \) $, and get 
    \begin{align*} 
        & \; \Pr \( \left| \wh{c}_{n, \alpha} (f(X_q)) - \mathrm{CVaR}_\alpha (f(X_q)) \right| > \frac{1}{2} \( f_q^* - \mathrm{CVaR}_\alpha (X_q) \) \) \\
        \le& \;  
        2 \exp \( - \frac{n  (1-\alpha)^2 \( f_q^* - \mathrm{CVaR}_\alpha (X_q) \)^2 }{ 8 \( \D (q) \)^2} \) + 4 \exp \( -\frac{n (1 - \alpha)^2 \nu^2 \( f_q^* - \mathrm{CVaR}_\alpha (X_q) \)^2 }{ 256 \( \D (q) \)^{2}  } \) \\ 
        \le& \;  
        6 \exp \( - \frac{n  (1-\alpha)^4 \kappa_-^2 \min\{ 1, \nu^2 \} }{ 256 } \) . 
        % + 4 \exp \( -\frac{n (1 - \alpha)^2 \nu^2 \( f_q^* - \mathrm{CVaR}_\alpha (X_q) \)^2 }{ 256 \( \D (q) \)^{2d}  } \)  \\ 
    \end{align*} 
    Since $ f_q^* - \mathrm{CVaR}_\alpha (X|_{q}) \le \kappa_+ (1-\alpha) \D (q) $, it holds that  
    \begin{align*} 
        \Pr \( \left| \wh{c}_{n, \alpha} (f (X_q)) - \mathrm{CVaR}_\alpha (f(X_q)) \right| > \frac{ \kappa_+ }{2} \( 1 - \alpha \) \D (q) \) 
        % \le& \;  
        \le& \;  
        6 \exp \( - \frac{n  (1-\alpha)^4 \kappa_-^2 \min\{ 1, \nu^2 \} }{ 256 } \) .  
    \end{align*} 
    
    Now let $ 1 - \alpha = (\frac{ 256 \log (6/\epsilon) }{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4} \in (0,1) $. After rearranging terms, we have 
    \begin{align*} 
        \Pr \( \left| \wh{c}_{n, 1-(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4}} (f(X_q)) - \mathrm{CVaR}_{1-(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4}} (f(X_q)) \right| > 2 \kappa_+  \( \frac{ \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n } \)^{1/4} \D (q) \)  
        \le& \; 
        \epsilon , \quad \forall \epsilon \in (0,1) . 
    \end{align*} 
    
    
    Then with probability larger than $1 - \epsilon$, we have 
    \begin{align*} 
        & \; f_q^* - \wh{c}_{n, 1-(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4}} (f (X_q)) \\ 
        \le& \;  
        f_q^* - \mathrm{CVaR}_{1-( \frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4} } (f (X_q)) + \mathrm{CVaR}_{1-(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4} } (f (X_q)) - \wh{c}_{n, 1-(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4}} (f(X_q)) \\ 
        \le& \; 
        \kappa_+(\frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n })^{1/4} \D (q) + 2 \kappa_+  \( \frac{ \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n } \)^{1/4} \D (q) \\
        \le& \; 
        6 \kappa_+  \( \frac{ \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n } \)^{1/4} \D (q) , 
        % + \kappa_+ (1 - \alpha) \D (q) . 
    \end{align*} 
    where the last inequality follows from 1-Lipschitzness of $f$, $\frac{ 256 \log (6/\epsilon) }{ \kappa_-^2 \min\{ 1, \nu^2 \} n } \in (0,1)$ and $ \kappa_+ \ge 1 $. 

\end{proof}


Now, we arrive at an estimator whose confidence range looks very different from existing Lipschitz estimators in Lipschitz bandits literature. 

\section{Optimization Algorithm based on the CVaR Estimator} 







\subsection{Redefine and reiterate some notations first}

We will consider optimization over $[0,1]$. 

\begin{itemize} 
    \item For any interval $I$, let $X_I$ be the uniform random variable over $I$. 
    \item For simplicity, let 
    \begin{align*} 
        A_\epsilon =  \frac{ \log (6/\epsilon) }{ \kappa_-^2 \min \{ 1, \nu^2 \} } . 
        % \quad \text{ and } \quad C_\epsilon = \frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n } . 
    \end{align*} 
    \item For any interval $I$, let $f_I^*$ be the maximal value of $f$ over $I$.
    \item For any $n, \alpha$, let $\wh{c}_{n,\alpha} (f (X_I))$ denote the $n$-sample estimator of $\mathrm{CVaR}_\alpha ( f (X_I) ) $. 
\end{itemize} 

With the above notations, we have 
\begin{align*} 
    f_I^* - \wh{c}_{n, 1-(\frac{256 A_\epsilon }{ n })^{1/4} } (f ( X_I )) 
    \le 
    6 \kappa_+ \( \frac{ A_\epsilon }{ n } \)^{1/4} \mathcal{D} (I) . 
\end{align*} 
with high probability. 



\begin{algorithm}[h]
	\caption{Optimization via CVaR Optimization (over $[0,1]$)} 
	\label{alg} 
	\begin{algorithmic}[1]  
            \STATE \textbf{Assumption:} Suppose that the function $f$ has zooming dimension $d_z = 0$ and zooming constant $C_z$. 
		\STATE \textbf{Input:} Time horizon $T$. $\gamma > 1$. $\epsilon \in (0,1)$. 
		\STATE \textbf{Initialization:} Let $ \mathcal{A}_1 = \{ [0, \frac{1}{2}] , [\frac{1}{2}, 1] \} $. Let $ N_0 = 256A_\epsilon $. Let $ M = \lfloor \frac{ \log \( \frac{\gamma-1}{\gamma}\cdot \frac{T}{C_z N_0 } \) }{\log \gamma } \rfloor$. 
		\FOR{$m=1,2,\cdots,M$} 
                \STATE Compute $ n_m = N_0 \gamma^m $, $\alpha_m = 1-(\frac{256 A_\epsilon }{ n_m })^{1/4} $, $\rho_m = 6 \kappa_+ \( \frac{A_\epsilon}{n_m} \)^{1/4} 2^{-m}$. 
                \FOR{interval $I$ in $ | \mathcal{A}_{m} | $} 
                    \STATE Uniformly randomly sample $n_m$ points from $I$, and compute $ \wh{c}_{n_m, \alpha_m } (f (X_I)) $. 
                    \STATE Compute $ \wh{C}_m^{\max} := \max_I \wh{c}_{n_m, \alpha_m} f (X_I) $. 
                    \STATE Let $\mathcal{A}_{m+\frac{1}{2}} = \{ I \in  \mathcal{A}_m : \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m } (f (X_I)) \le \rho_m \}$. /* Elimination step */
                    \STATE Bisect the intervals in $\mathcal{A}_{m + \frac{1}{2}}$, and collect these intervals to form $ \mathcal{A}_{m+ 1 } $. 
                    % = \{ I: \in  \mathcal{A}_{m+\frac{1}{2}} : \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m } \le \rho_m \} $
                \ENDFOR 
		\ENDFOR
            \STATE \textbf{Output}: $\wh{C}_{M}^{\max}$. 
    % \STATE \textbf{Cleanup:} Arbitrarily play the remaining arms until all $T$ steps are used.  
	\end{algorithmic} 
\end{algorithm} 



% Divide the total time-horizon into $B$ batches. For each batch $b$, we define
% \begin{align*} 
%     d_b = 2^{-b} , 
%     % \quad \text{ and } \quad 
%     % n_b := \frac{\log (6/\epsilon)}{ \kappa_-^2 \min \{ 1, \nu^2 \} } \( \frac{6 \kappa_+}{ d_b } \)^4 
% \end{align*} 
% and play each cube in batch $b$ for $n_b$ times. 





% \textcolor{red}{Question:} Can we design more efficient algorithms based on this estimator? 



% Now let the good event be true. Consider a batch with cube diameter $ d_b $ and number of points $n_b$. For simplicity, define 
% \begin{align*}
%     \rho_b :=  6\kappa_+ \( \frac{A_\epsilon}{ n_b } \)^{1/4} d_b .
% \end{align*} 
% % and with samples in $q$ 

% For simplicity, we overload some notations and define 
% \begin{align*} 
%     % \wh{c}_{n, \frac{256 \log (6/\epsilon)}{ \kappa_-^2 \min\{ 1, \nu^2 \} n }} (f (X_q)) 
%     \wh{c}_b (q) := \wh{c}_{n_b, \frac{256 A_\epsilon }{  n_b }} (f (X_q)) 
%     % = d_b^2. 
% \end{align*} 

% Consider the following algorithm procedure. Let $ I_m^{\max} \in \arg\max_{q'} \wh{c}_b (I') $. 


% We \textbf{eliminate} a cube $q$ if 
% \begin{align*} 
%     \wh{c}_b (q) + \rho_b < \wh{c}_b ( I_m^{\max} )  
% \end{align*} 


\begin{proposition}
    \label{prop1}
    Suppose the zooming dimension $d_z= 0 $ and let $C_z$ be the zooming number. Then the $M$ batches use at most $T$ total arm pulls.  
\end{proposition}

\begin{proof}
    Note that arms covered by $\mathcal{A}_{m}$ is $2\rho_{m-1}$-optimal. If the zooming dimension $d_z = 0$, then there are at most $ C_z $ intervals in $\mathcal{A}_m$. Thus the total number of arm pulls satisfies 
    \begin{align*}
        \sum_{m=1}^M | \mathcal{A}_m | n_m 
        \le 
        C_z N_0 \sum_{m=1}^M \gamma^m 
        \le 
        T. 
    \end{align*}
\end{proof}


\begin{lemma}
    Fix total time horizon $T$, and let $\epsilon = \frac{1}{T^2}$. 
    Let 
    \begin{align*}
        \mathcal{E} := \{ f_I^* - \wh{c}_{n_m, \alpha_m} (f (X_I)) \le \rho_m, \; \; \forall m = 1,2,\cdots, M \; \text{ and } \; \forall I \in \mathcal{A}_m \}. 
    \end{align*} 
    Then 
    \begin{align*}
        \Pr \( \mathcal{E}\) \ge 1- \frac{1}{T}. 
    \end{align*}
\end{lemma} 
\begin{proof}
    Since the $M$ batches use at most $T$ total arm pulls, by Lemma \ref{lem:concen} and a union bound, we conclude the proof. 
\end{proof}


\begin{lemma}
    \label{lem:survive}
    Under the event $\mathcal{E}$, the optimal arm $x^*$ is not eliminated. 
\end{lemma}

\begin{proof}
    Let $I_m^*$ be the interval in $\mathcal{A}_m$ that contains $x^*$, and let $I_m^{\max} \in \arg \max_{I \in \mathcal{A}_m} \wh{c}_{n_m, \alpha_m} (f (X_I))$.
    Under the event $\mathcal{E}$, we have 
    \begin{align*} 
        \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} )) 
        = 
        \wh{c}_{n_m, \alpha_m} (f (X_{I_m^{\max}} )) - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} ))  
        \le 
        f_{I_m^{\max}}^* - f_{I_m^{*}}^* + \rho_m 
        \le 
        \rho_m , 
    \end{align*} 
    which implies that $ I_m^* $ is not eliminated. 
\end{proof} 


\begin{lemma}
    \label{lem:gap}
    Let event $\mathcal{E}$. In batch $m$, it holds that 
    \begin{align*} 
        f^* - \wh{c}_{n_{m-1} , \alpha_{m-1} } (f (X_{I_{m-1}'})) \le 2 \rho_{m-1} . 
    \end{align*} 
    % with high probability 
\end{lemma}


\begin{proof}
    
    Let $I_m^*$ be the cube in batch $m$ that contains the optimal arm, and let $I_m^{\max} = \arg \max_{I \in \mathcal{A}_m} \wh{c}_{n_m, \alpha_m} (f(X_I)) $. Then under event $\mathcal{E}$, for all $ I_{m-1}' \in \mathcal{A}_{m-1} $,  
    \begin{align*}
        f_{I_{m-1}^*}^* - \wh{c}_{n_{m-1} , \alpha_{m-1} } (f (X_{I_{m-1}'})) 
        \le& \;  
        \wh{c}_{n_{m-1} , \alpha_{m-1} } (I_{m-1}^*) + \rho_{m-1} - \wh{c}_{n_{m-1} , \alpha_{m-1} } (f (X_{I_{m-1}'}))  \tag{by Lemma \ref{lem:concen}} \\ 
        \le& \;  
        2 \rho_{m-1} . \tag{since $I_{m-1}'$ are not eliminated before batch $m-1$} 
    \end{align*}

    We conclude the proof by Lemma \ref{lem:survive} and thus $ f^* = f_{I_{m-1}^*}^* $. 
    
\end{proof} 



\begin{theorem}
    Fix $T$ and let $\epsilon = \frac{1}{T^2} $. With probability larger than $1 - \frac{1}{T}$, it holds that 
    \begin{align*}
        f^* - \wh{C}_M^{\max} \le O \( \( \frac{\gamma - 1}{\gamma}\cdot \frac{T}{ C_z N_0} \)^{-\frac{1}{4} - \log_\gamma 2 } \) . 
    \end{align*}
    In particular, if $\gamma = 2$, then the error bound is of order $ O \( \( \frac{T}{ 2C_z N_0 } \)^{-5/4} \) $. 
\end{theorem}

\begin{proof}
    By Lemma \ref{lem:gap}, $ f^* - \wh{C}_M^{\max} \le 2 \rho_{M} $. We conclude the proof by noting 
    \begin{align*}
        \rho_M 
        =& \; 
        6 \kappa_+ \( \frac{ A_\epsilon}{n_M} \)^{1/4} 2^{-M} \\
        =& \; 
        6 \kappa_+ A_\epsilon^{ \frac{1}{4} } N_0^{-\frac{1}{4}}\gamma^{-\frac{M}{4}} 2^{-M } \\
        =& \; 
        \frac{3}{2} \kappa_+ \(\frac{\gamma-1}{\gamma}\cdot \frac{T}{ C_z N_0} \)^{-\frac{1}{4} - \log_\gamma 2 } . 
    \end{align*} 
\end{proof}



\noindent Define the set of $r$-optimal arms as $S(r) = \{x\in \mathcal{A}:\Delta_x \leq r \}$. The $r$-zooming number is defined as
\begin{equation*}
    N_r := \# \{C:C \text{ is a cube with edge length } r \text{ and } C \subset S(r)\} \text{ (lack a constant)}.
\end{equation*}
In other words, $N_r$ is the $r$-covering number of the set $S(r)$.The zooming dimension is then defined as
\begin{equation*}
    d_z := \min \{d\geq 0:\exists a>0,N_r\leq ar^{-d},\forall r=2^{-i} \text{ for some } i \in \mathbb{N}\}.
\end{equation*}
We also define the zooming constant $C_z$ as the minimal $a$ that makes the above inequality hold for $d_z$,
\begin{equation*}
    C_z = \min\{a>0:N_r\leq ar^{-d_z},\forall r=2^{-i} \text{ for some } i \in \mathbb{N}\}.
\end{equation*}


\begin{proposition}
    When $d_z \geq 0$, let $M = \frac{\log \left(\frac{T}{\(6\kappa_+\)^{1-d_z}C_zN_0}\cdot \frac{2^{d_z}\gamma^{(d_z+3)/4}-1}{2^{d_z}\gamma}\right)}{\log (2^{d_z}\gamma^{(d_z+3)/4})}$. Then the $M$ batches use at most $T$ total arm pulls.
\end{proposition}

\begin{proof}
Noticing that the arms covered by $\mathcal{A}_m$ is $2\rho_{m-1}$-optimal, so the number of intervals in $\mathcal{A}_m$ is upper bounded by $\frac{2\rho_{m-1}}{r_m}N_{2\rho_{m-1}} \leq \frac{2\rho_{m-1}}{r_m}C_z(2\rho_{m-1})^{-d_z} = C_z \left( 6\kappa_+\gamma^{1/4}\right)^{1-d_z} \left( \gamma^{\frac{1}{4}d_z-\frac{1}{4}}2^{d_z}\right)^m$.

Following this, we have
\begin{equation*}
\begin{aligned}
    && \sum_{m=1}^M |\mathcal{A}_m|n_m & \leq \sum_{m=1}^M C_z \left( 6\kappa_+\gamma^{1/4}\right)^{1-d_z} \left( \gamma^{\frac{1}{4}d_z-\frac{1}{4}}2^{d_z}\right)^m \cdot N_0\gamma^m \\
    && & = \left( 6\kappa_+\gamma^{1/4}\right)^{1-d_z}C_zN_0 \sum_{m=1}^M (2^{d_z}\gamma^{\frac{1}{4}d_z + \frac{3}{4}})^m \\
    && & \leq \left( 6\kappa_+\gamma^{1/4}\right)^{1-d_z}C_zN_0 \cdot \frac{(2^{d_z}\gamma^{\frac{1}{4}d_z + \frac{3}{4}})^{M+1}}{2^{d_z}\gamma^{\frac{1}{4}d_z + \frac{3}{4}}-1} \\
    && & \leq T
\end{aligned}
\end{equation*}
\end{proof}

\begin{theorem}
When $d_z \ge 0$, with probability larger than $1-\frac{1}{T}$, it holds that
    \begin{equation*}
        f^* - \hat{C}_M^{\max} \leq \mathcal{O} \left( \left(\frac{T}{\(6\kappa_+\)^{1-d_z}C_zN_0}\cdot \frac{2^{d_z}\gamma^{(d_z+3)/4}-1}{2^{d_z}\gamma}\right) ^{-\log_{2^{d_z}\gamma^{(d_z+3)/4}} 2\gamma^{1/4}} \right)
    \end{equation*}
In particular, when $\gamma = 2$ and $d_z = 0$, the error bound is of order smaller than $\mathcal{O} \left( \left( \frac{T}{6\kappa_+ C_zN_0}\cdot \frac{2^{3/4}-1}{2} \right)^{-\frac{5}{3}} \right)$
\end{theorem}

\begin{proof}
    \begin{equation*}
    \begin{aligned}
    && f^* - \hat{C}_M^{\max} & \leq 2\rho_M \\
    && & = 6\kappa_+\left(\frac{A_{\epsilon}}{n_M}\right)^{\frac{1}{4}} 2^{-M+1} \\
    && & = 3\kappa_+ \gamma^{-\frac{1}{4}M}2^{-M} \\
    && & = 3\kappa_+ \left(\frac{T}{\(6\kappa_+\)^{1-d_z}C_zN_0}\cdot \frac{2^{d_z}\gamma^{(d_z+3)/4}-1}{2^{d_z}\gamma}\right) ^{-\log_{2^{d_z}\gamma^{(d_z+3)/4}} 2\gamma^{1/4}}
    \end{aligned}
    \end{equation*}
\end{proof}


~\\
\textbf{When n is a constant:}

Assume $n$ is a constant independent of $m$. Set $n = 256 A_{\epsilon} n_0$, where $ n_0 > 1$ (as $\alpha > 0$). Then the number of intervals in $\mathcal{A}_m$ is upper bounded by $\frac{2\rho_{m-1}}{r_m}N_{2\rho_{m-1}} \leq \frac{2\rho_{m-1}}{r_m}C_z(2\rho_{m-1})^{-d_z} = C_z \( 6\kappa_+ n_0^{-1/4}\)^{1-d_z} 2^{md_z}$.


\noindent 1)\quad When $d_z = 0$, let $M = \frac{T}{256 \times 6 C_z A_{\epsilon} \kappa_+ n_0^{\frac{3}{4}}}$, then 
\begin{equation*}
\begin{aligned}
    \sum_{m=1}^M n|\mathcal{A}_m| \leq \sum_{m=1}^M 256 \times 6 C_z A_{\epsilon} \kappa_+ n_0^{\frac{3}{4}} = 256 \times 6 C_z A_{\epsilon} \kappa_+ n_0^{\frac{3}{4}} M \leq T
\end{aligned}
\end{equation*}
With probability larger than $1-\frac{1}{T}$, it holds that 
\begin{equation*}
    f^* - \hat{C}_M^{\max} \leq 2\rho_{M} = 3\kappa_+ n_0^{-1/4}2^{-M} = 3\kappa_+ n_0^{-1/4}\times 2^{-\frac{T}{256\times 6 \kappa_+C_z A_{\epsilon} n_0^{\frac{3}{4}}}} \sim \mathcal{O} \left( 2^{-\frac{T}{\log T}} \right)
\end{equation*}


\noindent 2) \quad When $d_z > 0$, let $M = \frac{\log \left( \frac{T}{256 C_z A_{\epsilon} \( 6\kappa_+\)^{1-d_z} n_0^{(d_z+3)/4}} \cdot \frac{2^{d_z}-1}{2^{d_z}}\right)}{\log 2^{d_z}}$, then
\begin{equation*}
\begin{aligned}
    \sum_{m=1}^M n|\mathcal{A}_m| \leq \sum_{m=1}^M 256 C_z A_{\epsilon} \( 6\kappa_+\)^{1-d_z} n_0^{\frac{1}{4}d_z+\frac{3}{4}} 2^{md_z} \leq 256 C_z A_{\epsilon} \( 6\kappa_+\)^{1-d_z} n_0^{\frac{1}{4}d_z+\frac{3}{4}} \times \frac{2^{(M+1)d_z}}{2^{d_z}-1} \leq T
\end{aligned}
\end{equation*}
With probability larger than $1-\frac{1}{T}$, it holds that
\begin{equation*}
\begin{aligned}
    && f^* - \hat{C}_M^{\max} & \leq 2\rho_{M} = 3\kappa_+ n_0^{-1/4} 2^{-M} = 3\kappa_+ n_0^{-1/4} \left( \frac{T}{256 C_z A_{\epsilon} \( 6\kappa_+\)^{1-d_z} n_0^{(d_z+3)/4}} \cdot \frac{2^{d_z}-1}{2^{d_z}} \right)^{-\log_{2^{d_z}} 2} \\
    && & \sim \mathcal{O} \left( \left(\frac{T}{\log T} \right)^{-\frac{1}{d_z}} \right)
\end{aligned}
\end{equation*}

Since when $n_m = 256 A_{\epsilon}\gamma^m, d_z > 0$, the error order is $\mathcal{O} \left( \left(\frac{T}{\log T}\right) ^{-\log_{2^{d_z}\gamma^{(d_z+3)/4}} 2\gamma^{1/4}} \right)$, by noting that 
\begin{equation*}
     -\log_{2^{d_z}\gamma^{(d_z+3)/4}} 2\gamma^{1/4} > -\log_{2^{d_z}\gamma^{d_z/4}} 2\gamma^{1/4} = -\frac{1}{d_z},
\end{equation*}
choosing $n = 256 A_{\epsilon} n_0$, which is independent of $m$, achieves a smaller error order than choosing $n_m$.

%Since when $n_m = 256 A_{\epsilon}\gamma^m, d_z > 0$, the error order $\left(\frac{T}{\(6\kappa_+\)^{1-d_z}C_zN_0}\cdot \frac{2^{d_z}\gamma^{(d_z+3)/4}-1}{2^{d_z}\gamma}\right) ^{-\log_{2^{d_z}\gamma^{(d_z+3)/4}} 2\gamma^{1/4}}$ increases with $\gamma \in \mathbb{N}_+$ when $T$ is large enough, choosing $\gamma = 2$ guarantees a smaller error order than choosing $\gamma > 2, \gamma \in \mathbb{N}_+$. Therefore, in order to achieve the best convergence rate when $d_z > 0$, we only need to compare the error order when $n_m = 256 A_{\epsilon} \cdot 2^m$ and $n = 256 A_{\epsilon}n_0$, that is, to compare $\left(\frac{T}{\(6\kappa_+\)^{1-d_z}C_zN_0}\cdot \frac{2^{\frac{5}{4}d_z+\frac{3}{4}}}{2^{d_z+1}}\right) ^{-\frac{5}{5d_z+3}}$ and $ n_0^{-1/4} \left( \frac{T}{256 C_z A_{\epsilon} \( 6\kappa_+\)^{1-d_z} n_0^{(d_z+3)/4}} \cdot \frac{2^{d_z}-1}{2^{d_z}} \right)^{-\frac{1}{d_z}} $. It is obvious that the latter is of smaller order.



% \textbf{Let the zooming dimension be $0$}. 

% Let there be $B$ batches and $T$ total arm pulls, then we have 
% \begin{align*} 
%     \sum_{m=1}^M C_z n_m  = T , 
% \end{align*} 

% In batch $b$, we have 
% \begin{align*} 
%     f^* - \wh{c}_b (I_m^{\max}) 
%     \le 
%     f^* - \wh{c}_b (I_m^{*}) 
%     \le 
%     \rho_b . 
% \end{align*} 

% ---------------------------------------------------------------

% What about 

% \begin{lemma}
%     Let $\Delta_x := f (x^*) - f (x)$ be the optimality gap of arm $x$. Then for any arm $x$ that has not been eliminated before batch $b$, we have  
%     \begin{align*} 
%         \Delta_x \le 2 \rho_{b-1} + d_{b-1} . 
%     \end{align*} 
% \end{lemma} 

% \begin{proof}
%     % Then the optimality gap in batch $b$. 
%     For any arm $x$ that has not been eliminated before batch $b$, we have  
%     \begin{align*} 
%         \Delta_x 
%         = 
%         f^* - f (x) 
%         \le 
%         \wh{c}_{b-1} (q_{b-1}^*) + \rho_{b-1} - \wh{c}_{b-1} ( q_{b-1} (x) ) + d_{b-1},  
%     \end{align*} 
%     where $q_{b-1} (x)$ is the cube in batch $b-1$ that contains $x$. 
    
%     Since $ q_{b-1} (x) $ is not eliminated, it holds that 
%     % we have 
%     \begin{align*} 
%         \Delta_x 
%         \le 
%         \wh{c}_{b-1} (q_{b-1}^*) + \rho_{b-1} - \wh{c}_{b-1} ( q_{b-1} (x) ) + d_{b-1}
%         \le 
%         2 \rho_{b-1} + d_{b-1} 
%     \end{align*}
% \end{proof}

% Note that the above inequality holds under the following conditions: 

% Now we can eliminate cubes with high confidence. 

% With high confidence, we know that $ \wh{c}_{n, \alpha} \ge \wh{c}_{n, \alpha}  $
 
% \begin{proposition}
    
% \end{proposition}

% ----------------------------------------------------


% Let $X_1, \cdots, X_{n_1} $ be $i.i.d$ random variables such that $X_i \in P$ for all $i = 1,2,\cdots, n_1$. Let $Y_1, \cdots, Y_{n_2} $ be $i.i.d$ random variables such that $Y_i \in P \subseteq Q$ for all $i = 1,2,\cdots, n_2$. 

==> tex/algo.tex <==



\section{The Batched Lipschitz Narrowing Algorithms} 

  
% \subsection{The Try-And-Eliminate Procedure} 

% As suggested by its name, the Batched Lipschitz Narrowing algorithms progressively narrow the search space. Such algorithms are executed in batches. In each batch, the algorithm performs guided trials, and eliminate regions of low payoffs. After each iteration, the problem space becomes narrower, and the algorithm repeats this try-and-eliminate procedure until a pre-determined terminating condition is met. In Figure \ref{}, an example run of batched narrowing is provided. Two algorithms of this kind are formally summarized in Algorithms \ref{alg:small-d} and \ref{alg:large-d}. 

The Batched Lipschitz Narrowing algorithms, as the name implies, progressively narrow the search space. Such algorithms operate in batches, where they perform guided trials and eliminate low-payoff regions. After each batch, the problem space shrinks, and the algorithm repeats this try-and-eliminate process until a pre-determined termination condition is met. Figure \ref{} shows an example run of batched narrowing. We formally present two algorithms of this type --- Batched Lipschitz Narrowing (BLiN) and  Batched Lipschitz Narrowing with Maximum Ordered Statistics (BLiN-MOS).

\textcolor{red}{(need to specify $M$ in the algorithms.)} 

\begin{algorithm}[ht] 
	\caption{Batched Lipschitz Narrowing (BLiN)} 
	\label{alg:small-d} 
	\begin{algorithmic}[1]  
		\STATE \textbf{Input.} Arm set $\A=[0,1]^d$; time horizon $T$.
		\STATE \textbf{Initialization} Number of batches $M$; Edge-length sequence $\{r_m\}_{m=1}^{M+1}$; The first grid point $t_0=0$; Equally partition $\mathcal{A}$ to $r_1^d$ subcubes and define $\mathcal{A}_{1}$ as the collection of these subcubes. 
		% \STATE Compute $n_m=\frac{16\log T}{r_m^2}$ for $m=1,\cdots,B+1$.
		
		\FOR{$m=1,2,\cdots,M$}
			\STATE For each cube $q\in\mathcal{A}_m$, pick an arm $x_{q} $ from $q$.
			% \STATE Collect the rewards of all pulls up to $t_m$. Compute the average payoff $\wh{\mu}_m(C)=\frac{\sum_{i=1}^{n_m}y_{C,i}}{n_m}$ for each cube $C\in\mathcal{A}_m$.
% 			\STATE $tp=tp+n_m\cdot|\mathcal{A}_m|$.
			\STATE Compute   $Y_m^{\max}=\max_{q\in\mathcal{A}_m} f(x_q)$.
			\STATE Let $\mathcal{A}_{m+\frac{1}{2}} = \{ q \in \mathcal{A}_m: Y_m^{\max} - f (x_q) \le 2L r_m \} $. 
                % \STATE For each cube $C\in\mathcal{A}_m$, eliminate $C$ if $\wh{\mu}_m^{max}-\wh{\mu}_m(C)>4r_m$. Let $\mathcal{A}_m^+$ be set of cubes not eliminated. 
			\STATE Compute $t_{m+1}=t_m+(r_{m}/r_{m+1})^d\cdot|\mathcal{A}_{m + \frac{1}{2}} | $. 
                \IF{$t_{m+1}\geq T$}
                    \STATE Let $M^* = m$. \textbf{Terminate} the algorithm and \textbf{output} $ Y_{M^*}^{\max} $.  /* The last line of the algorithm is not executed if we enter this if condition */
                \ENDIF
                % If  or $m=B$ then let $M^* = M$ and \textbf{break}.
			\STATE Equally partition each cube in $\mathcal{A}_{m+\frac{1}{2}} $ into $\left(r_m/r_{m+1}\right)^d$ subcubes and define $\mathcal{A}_{m+1}$ as the collection of these subcubes. 
   % /*\textit{See Remark \ref{remark:race} for more details on cases where $\left(r_m/r_{m+1}\right)^d$ is not an integer.}*/
		\ENDFOR
            \STATE Let $M^* = M$ and \textbf{output:} $ Y_{M^*}^{\max} $. 
    % \STATE \textbf{Cleanup:} Arbitrarily play the remaining arms until all $T$ steps are used.  
	\end{algorithmic} 
\end{algorithm} 



\begin{algorithm}[ht] 
	\caption{Batched Lipschitz Narrowing with Max Order Statistics (BLiN-MOS)} 
	\label{alg:large-d} 
	\begin{algorithmic}[1]  
		\STATE \textbf{Input.} Arm set $\A=[0,1]^d$; time horizon $T$.
		\STATE \textbf{Initialization} Number of batches $B$; Edge-length sequence $\{r_m\}_{m=1}^{M+1}$; The first grid point $t_0=0$; Equally partition $\mathcal{A}$ to $r_1^d$ subcubes and define $\mathcal{A}_{1}$ as the collection of these subcubes. 
		% \STATE Compute $n_m=\frac{16\log T}{r_m^2}$ for $m=1,\cdots,B+1$. 
		\FOR{$m=1,2,\cdots,M$} 
                \STATE Compute $\alpha_m = r_m^k$, $\rho_m = L \alpha_m r_m$, and $ n_m = \frac{\log \epsilon }{ \log \(1 - \kappa_s \alpha_m^{d_s} \) }$, where $k > 0 $. 
                % $\alpha_m = 1-(\frac{256 A_\epsilon }{ n_m })^{1/4} $, $\rho_m = 6 \kappa_+ \( \frac{A_\epsilon}{n_m} \)^{1/4} 2^{-m}$. 
                % \FOR{cube $q \in \mathcal{A}_{m} $} 
                \STATE Uniformly randomly sample $n_m$ points $ X_{q}^1, X_{q}^2, \cdots, X_{q}^{n_m} $ from $q \in \mathcal{A}_m$. 
                % , and compute $ Y_{q, n_m } $. 
                \STATE Compute $ Y_{q,n_m} = \max \{ f (X_{q}^1), f(X_{q}^2), \cdots, f (X_{q}^{n_m}) \} $ and $ Y_m^{\max} := \max_{q \in \mathcal{A}_m } Y_{q,n_m} $. 
                \STATE Let $\mathcal{A}_{m+\frac{1}{2}} = \{ q \in  \mathcal{A}_m : {Y}_m^{\max} - {Y}_{q,n_m} \le \rho_m \}$. /* Elimination step */ 
                % \textcolor{red}{(some tricks for $r_m$??? )} 
                \STATE Compute $t_{m+1}=t_m+(r_{m}/r_{m+1})^d\cdot|\mathcal{A}_{m + \frac{1}{2}} | $. 
                \IF{$t_{m+1}\geq T$}
                    \STATE Let $M^* = m$. \textbf{Terminate} the algorithm and \textbf{output} $ Y_{M^*}^{\max} $.  /* The last line of the algorithm is not executed if we enter this if condition */
                \ENDIF 
                \STATE Dyadically partition the cubes in $\mathcal{A}_{m + \frac{1}{2}}$, and collect these cubes to form $ \mathcal{A}_{m+ 1 } $. 
                    % = \{ I: \in  \mathcal{A}_{m+\frac{1}{2}} : \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m } \le \rho_m \} $
                % \ENDFOR 
		\ENDFOR 
        \STATE Let $M^* = M$ and \textbf{output:} $ Y_{M^*}^{\max} $. 
        % \STATE \textbf{Output:} $ Y_{M}^{\max} $. 
	\end{algorithmic} 
\end{algorithm} 

% the problem space is narrower than the previous batch, and . 

% As demonstrated in Figure \ref{??}, s
Such procedures focus more resources on regions of promising function values. Both BLiN and BLiN-MOS are landscape-aware. Thus their convergence rates depend on $d_z$ and $d_s$. To fully unleash the power of BLiN and BLiN-MOS, we need to carefully choose the edge-length sequence $\{ r_m \}_{m=1}^{M+1}$. 
An immediate choice of $ \{ r_m \}_{m=1}^M $ is letting $ r_m = 2^{-m} $. This choice of the edge-length sequence leads to $O (\log T)$ rounds of communications. With a more careful choice of $ \{ r_m \}_{m=1}^M $, we can achieve a better communication complexity. This edge-length sequence is defined below in Definition \ref{def:ace}. 

\begin{definition} 
    \label{def:ace} 
    Denote $c_1 = \frac{d_z-1+k d_s }{(d+k d_s )(d_z+k d_s )}\log \frac{T}{\log T}$, $ c_{i+1} = \eta c_i,i\geq 1$, where $\eta = \frac{d+1-d_z}{d+k d_s }$. Let $a_n = \lfloor \sum_{i=1}^n c_i\rfloor$, $b_n = \lceil \sum_{i=1}^n c_i\rceil$. Define sequence $\{r_m\}_m $ as $r_m = \min \{ r_{m-1}, 2^{-a_n} \}$ for $m = 2n-1$ and $r_m = 2^{-b_n}$ for $m = 2n$.
    % (Here we suppose $\{r_m\}$ is a strictly decreasing sequence, see Remark \ref{rm:batch} for details). 
    Define sequence $\{\alpha_m\}_m$ as $\alpha_m = r_m^k,k>0$. 
\end{definition} 

% We start with some pro 

With the edge-length sequence defined above, we can state the main convergence results. 
% In particular, we need to pick $ \{ r_m \}_{m=1}^{M+1} $ so that 
The convergence rates depend on zooming dimension $d_z$ and scattering dimension $d_s$, as stated in Theorem \ref{thm:small-d}, Theorem \ref{thm:large-d} and Corollary \ref{cor1}. 

% To 

% This dependence on $d_s$ and $d_z$ means that BLiN and BLiN-MOS are landscape-aware, and adaptively narrows the domain. 


% in the following Theorems and Corollaries. 
% Theorems \ref{thm:small-d} and \ref{thm:large-d}. 

\begin{theorem}
% [\textcolor{red}{a theorem for algorithm \ref{alg:small-d} }]
    \label{thm:small-d}
    % \label{thm:ace}
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:small-d}. 
    Output arm $\widetilde{x}^*$ of BLiN algorithm with total time horizon $T$ and ACE Sequence $\{r_m\}$ satisfies 
    \begin{equation*} 
        \Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z}},
    \end{equation*}
    where $d_z$ is the zooming dimension and $c$ is a constant. In addition, BLiN needs $\mathcal{O}(\log\log T)$ batches to achieve this optimality gap. 
    % regret.
    % When $d_z = 0$, XXXXX 

    % When $d_z > 0$, XXXXX 
    
\end{theorem} 

% ----------------------------------------------------

% \begin{definition}
%     \label{def:opt-batch}
%     Denote $c_1 = \frac{d_z-1+k d_s }{(d+k d_s )(d_z+k d_s )}\log \frac{T}{\log T}$, $ c_{i+1} = \eta c_i,i\geq 1$, where $\eta = \frac{d+1-d_z}{d+k d_s }$. Let $a_n = \lfloor \sum_{i=1}^n c_i\rfloor$, $b_n = \lceil \sum_{i=1}^n c_i\rceil$. Define sequence $\{r_m\}$ as $r_m = 2^{-a_n}$ for $m = 2n-1$ and $r_m = 2^{-b_n}$ for $m = 2n$ (Here we suppose $\{r_m\}$ is a strictly decreasing sequence, see Remark \ref{rm:batch} for details). Define sequence $\{\alpha_m\}$ as $\alpha_m = r_m^k,k>0$.
% \end{definition}

\begin{theorem} 
    \label{thm:opt-batch} 
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:large-d}. 
    Let $T$ be the total time horizon such that $ (d+1-d_z) \log \frac{T}{\log T} - d d_z > 0 $ and let $\epsilon = \frac{1}{T^2}$. Let $ k \in \( 0, \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} \] $. Let $M \ge 2\times \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} +1$. Apply the sequence $\{r_m\}_{m=1}^{M}$ in Definition \ref{def:ace} to Algorithm \ref{alg:large-d}. 
    % With fixed budget $T$, 
    % the final simple regret satisfies 
    Then with probability exceeding $1 - \frac{1}{T}$, the final optimality gap satisfies  
    \begin{equation*} 
        f^*_q - Y^{\max}_{M^*} \leq cL\left(\frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }},
    \end{equation*} 
    where $Y^{\max}_{M^*}$ is the output of Algorithm \ref{alg:large-d} and $c$ is a constant independent of $T$. 
    % In addition, 
    % Moreover, only $2\times \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} +1$ total batches are needed to achieve this optimality gap. 
\end{theorem} 

\textcolor{red}{Since the lower bound of $\tilde{C}$ in Remark 1 is related to $k$, ranges of $k$ and $T$ in Theorem 3 and Corollary 1 need to be modified. If $\tilde{C}$ is set as $\tilde{C} = \frac{d+1-d_z}{d_z - 1 + kd_s}$, then $k \leq \frac{ \left( \log \frac{T}{\log T} - d - d_z\right) + \sqrt{\left( \log \frac{T}{\log T} - d - d_z\right)^2 + 4\left( (d_z-1)\log \frac{T}{\log T} - d d_z \right)} }{2d_s}$, and $\log \frac{T}{\log T} > \max\{d+d_z, \; d-d_z+2 + 2\sqrt{d-d_z+1 } \}$ is sufficient.}
% 
% ----------------------------------------------------

% Theorem \ref{thm:opt-batch} 


The results of Theorem \ref{thm:opt-batch} can be rephrased as follows. 

\begin{corollary} 
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:large-d} with $\epsilon = \frac{1}{T^2}$ and edge-length sequence defined in Definition \ref{def:ace}. For each total time horizon $ T \in \mathbb{N} $ such that $ (d+1-d_z) \log \frac{T}{\log T} - d d_z > 0 $, let $ k = \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} $. 
    % Define the edge-length sequence as 
    % $ Let $ \epsilon = \frac{1}{T^2} $ and 
    Then there exists a sequence $ \{ G_T \}_{T} $ such that (1) $ G_T = \mathcal{O} \( \( \frac{T}{\log T} \)^{-\frac{1}{d_s}} \) $, and (2) for each $T \in \mathbb{N}$,
    with probability exceeding $ 1 - \frac{1}{T} $, the final optimality gap of Algorithm \ref{alg:large-d} is no larger than $ G_T $.  
\end{corollary} 

\begin{proof}
    For any $T$, we let $ k $ take the maximum possible value in Theorem \ref{thm:opt-batch}. We know as $T$ approaches infinity, the value of $ \( \frac{ \kappa T (2^{d_z + kd_s} -1) }{2 C_z \log (T ) 2^{d_z + kd_s}} \)^{- \frac{ 1+k }{d_z + kd_s}} $ is of order $ \mathcal{O} \( \( \frac{T}{\log T} \)^{-\frac{1}{d_s}} \) $.
\end{proof} 


When $d_z \ge d_s$, we have $ -\frac{1+k}{d_z + k d_s} \le - \frac{1}{d_z} $. In this case, BLiN-MOS outperforms BLiN. When $d_z < d_s$, we have $ -\frac{1+k}{d_z + k d_s} > - \frac{1}{d_z} $. In this case, BLiN outperforms BLiN-MOS. 
% Moreover, when $d_z > d_s$, $-\frac{1+k}{d_z+k d_s}$ is decreasing with respect to $k$. 

The proof to Theorems \ref{thm:small-d} and \ref{thm:opt-batch} follow a similar path. Next we present the proof for Theorem \ref{thm:opt-batch}, and the proof of Theorem \ref{thm:small-d} can be found in the appendix. 

% ---------------------------------------------------- 

\begin{proof}[Proof of Theorem \ref{thm:opt-batch}] 
    Denote $\tilde{r}_n = 2^{-\sum_{i=1}^n c_i}$. 
    
    \textbf{Case I}: $m = 2n-1$. In this case, we have $r_m \geq \tilde{r}_n, r_{m-1} \leq \tilde{r}_{n-1}$. 
    Since $\Delta_x \leq 3Lr_{m-1}$ for any $x \in \cup_{q_m\in \mathcal{A}_m}q_m$, any cube in $\mathcal{A}_{m-\frac{1}{2}}$ is a subset of $S(3Lr_{m-1})$. Therefore,
    \begin{equation*}
        |\mathcal{A}_{m-\frac{1}{2}}| \leq N_{r_{m-1}} \leq C_z r_{m-1}^{-d_z}.
    \end{equation*}
    After partitioning $\mathcal{A}_{m-\frac{1}{2}}$ into $\mathcal{A}_m$, we get
    \begin{equation*}
        |\mathcal{A}_m| = \left(\frac{r_{m-1}}{r_m}\right)^d |\mathcal{A}_{m-\frac{1}{2}}| \leq \left(\frac{\tilde{r}_{n-1}}{\tilde{r}_n}\right)^d \cdot C_z r_{m-1}^{-d_z}.
    \end{equation*}
    Denote the total budget of the $m$-th batch as $N_m$, then
    \begin{equation*}
    \begin{aligned}
        && N_m = |\mathcal{A}_m| \cdot n_m & 
        \leq \left(\frac{r_{m-1}}{\tilde{r}_n}\right)^d \cdot C_z r_{m-1}^{-d_z} \cdot \frac{\log (1/\epsilon)}{\kappa_s \alpha_m^{ d_s }} 
        \leq \frac{C_z \log (1/\epsilon)}{\kappa_s } \cdot \frac{ \tilde{r}_{n-1}^{d-d_z+1} \cdot \tilde{r}_n^{-k d_s -d} }{r_{m-1}} \\
        && & = \frac{C_z \log (1/\epsilon)}{\kappa_s r_{m-1}} \cdot 2^{(d_z+k d_s -1)\sum_{i=1}^{n-1}c_i + (k 
        d_s +d)c_n}
    \end{aligned}
    \end{equation*}
    Define $C_n = (d_z+k d_s -1)\sum_{i=1}^{n-1}c_i + (k d_s +d)c_n$, then $C_n - C_{n-1} = (d_z-d-1)c_{n-1} + (k d_s +d)c_n = 0$. So for any $n > 1$, we have $C_n = C_1 = (k d_s +d)c_1$. Consequently, we obtain the upper bound of $N_m$ for $m = 2n-1$ as follows,
    \begin{equation*}
        N_m \leq \frac{C_z \log (1/\epsilon)}{\kappa_s r_{m-1}} \cdot \left(\frac{T}{\log T}\right)^{\frac{d_z+k d_s -1}{d_z+k d_s }}.
    \end{equation*}

    \textbf{Case II}: $m = 2n$.  Note that $r_{m-1} = \min\{r_{m-2},2^{-a_n} \} = r_{m-2}$ happens only when $\lceil \sum_{i=1}^{n-1}c_i \rceil > \lfloor \sum_{i=1}^{n}c_i \rfloor$. If the previous inequality holds, then $r_m = 2^{-\lceil \sum_{i=1}^{n}c_i \rceil } = 2^{-\lfloor \sum_{i=1}^{n}c_i \rfloor - 1} \geq 2^{-\lceil \sum_{i=1}^{n-1}c_i \rceil } = r_{m-2}$, which contradicts the assumption that $\{b_n\}$ is a strictly increasing sequence. Therefore, it must hold that $r_{m-1} = 2^{-a_n} = 2^{-b_n + 1} = 2r_m$. We thus conclude from Lemma \ref{lem:opt-gap} that any cube in $\mathcal{A}_m$ is a subset of $S(6Lr_m)$.  Therefore,
    \begin{equation*}
        N_m = |\mathcal{A}_m| \cdot n_m 
        \leq \frac{C_z\log (1/\epsilon)}{\kappa_s} \cdot r_m^{-d_z} \cdot r_m^{-k d_s }
    \end{equation*}

    Since the total budgets of all $M^*$ batches is $T$, 
    \begin{equation*}
    \begin{aligned}
        && T & \leq \sum_{m=2n-1, m\leq M^*} N_m + \sum_{m=2n, m\leq M^*} N_m \\
        && & \leq \frac{2C_z}{\kappa} \left( \sum_{m=2n-1, m\leq M^*} \frac{1}{r_{m-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k d_s }} + \sum_{m=2n, m\leq M^*} r_m^{-d_z-k d_s } \cdot \log T\right)
    \end{aligned}
    \end{equation*}
    
    Since $\{b_n\}$ is strictly increasing, we know that $r_{m} = 2r_{m+1} \geq 2\min\{r_{m+1},2^{-a_{\frac{m+1}{2}}}\} = 2r_{m+2}$ when $m$ is odd and $r_{m} \geq 2 r_{m+2}$ when $m$ is even. So $r_{m+2} \leq \frac{1}{2} r_m$ holds for any $m \in \mathbb{N}$. Following this, when $M^*$ is odd, $\sum_{m=2n-1,m\leq M^*} \frac{1}{r_{m-1}} \leq \left( \sum_{n=0}\frac{1}{2^n} \right) \cdot \frac{1}{r_{M^*-1}} = \frac{2}{r_{M^*-1}}$, $ \sum_{m=2n, m\leq M^*} \frac{1}{r_m^{d_z+k 
    d_s }} \leq \left(\sum_{n=0} \frac{1}{2^{n(d_z+k d_s )}}\right) \cdot {\frac{1}{r_{M^*-1}^{d_z+k d_s }}} = \frac{2}{r_{M^*-1}^{d_z+k 
    d_s }}$. Therefore, 
    \begin{equation*}
        T \leq \frac{4C_z}{\kappa_s} \cdot \left( \frac{1}{r_{M^*-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k 
        d_s }} + \frac{1}{r_{M^*-1}^{d_z+k d_s }} \cdot \log T \right).
    \end{equation*}
    Set $C = \max\{8C_z/\kappa_s,(8C_z/\kappa_s)^{\frac{1}{d_z+k 
    d_s }}\}$. We claim that $r_{M^*-1} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$ must hold. Otherwise, 
    \begin{equation*}
        \frac{4C_z}{\kappa_s} \cdot \left( \frac{1}{r_{M^*-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k d_s }} + \frac{1}{r_{M^*-1}^{d_z+k d_s }} \cdot \log T \right) < T,
    \end{equation*} 
    which yields contradiction. So we obtain $r_{M^*-1} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$, and $r_{M^*} \leq r_{M^*-1} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$.

    Similarly, when $M^*$ is even, we have
    \begin{equation*}
        T \leq \frac{4C_z\log T}{\kappa_s} \cdot \left( \frac{1}{r_{M^*}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} + \frac{1}{r_{M^*}^{d_z+k d_s }}\right).
    \end{equation*}
    Implementing the same deduction process as when $M^*$ is odd, we get $r_{M^*} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$.

    With $r_{M^*}$ upper bounded as above, the simple regret of the last batch $M^*$ can achieve an order smaller than or equal to $\mathcal{O}\left( \left( \frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }} \right)$:
    \begin{equation}
        \label{eq:simple-regret}
        f^*_q - Y^{\max}_{M^*} \leq \rho_{M^*} = L\alpha_{M^*} r_{M^*} = L r_{M^*}^{1+k } \leq cL\left(\frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }},
    \end{equation}
    where $c$ is a constant.

    To see that only $ O (\log \log T) $ batches are needed, we note that $\tilde{r}_{M} = 2^{-\sum_{i=1}^{M} c_i} = 2^{-c_1 \cdot \frac{1-\eta^{M}}{1-\eta}} = \left( \frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s } + \frac{\eta^{M}}{d_z+k d_s }}$. By letting $\frac{\eta^{M^{**}}}{d_z+k d_s } \leq \frac{ \textcolor{red}{\tilde{C}} }{\log \frac{T}{\log T}}$ ($\tilde{C}$ is a constant determined in Remark \ref{rm:batch} ), that is, choosing $M^{**} \geq \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s ) \textcolor{red}{ - \log \tilde{C} } }{\log \frac{d+k d_s }{d+1-d_z}}$, we can achieve $\tilde{r}_{M^{**}} \leq \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$. Since $r_m \leq \tilde{r}_{M^{**}}$ for $m\geq 2M^{**}$, only $2M^{**}+1$ batches are needed to achieve the simple regret in (\ref{eq:simple-regret}).
    

    Finally, the choice of $k$ in the final optimality gap is not arbitrary. 
    To ensure at least one round of narrowing, we need to ensure that $M^* \ge 1$. By (\ref{eq:lower-M-1}), it is sufficient to ensure that 
    \begin{align*}
        \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} \ge 1, 
    \end{align*}
    which implies 
    \begin{align*} 
        % \frac{1-d_z}{d_s} < 
        k 
        \le 
        \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} . 
        % k \le \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } . 
    \end{align*} 
\end{proof}


----------------------------------------------------

----------------------------------------------------


\begin{theorem}
    \label{thm:large-d} 
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:large-d}. Let $ T $ be the total time horizon, and let $ \epsilon = \frac{1}{T^2} $. In addition, let $T$ be large enough so that $ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z  > 0 $. Let $ k \in \( 0, \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } \] $. Define the edge-length sequence as $ r_m = 2^{-m}$. 
    % $ Let $ \epsilon = \frac{1}{T^2} $ and 
    Then with probability exceeding $ 1 - \frac{1}{T} $, the final optimality gap of Algorithm \ref{alg:large-d} is no larger than $ L \( \frac{ \kappa T (2^{d_z + kd_s} -1) }{2 C_z \log (T ) 2^{d_z + kd_s}} \)^{- \frac{ 1+k }{d_z + kd_s}} $.  
\end{theorem} 


\begin{corollary} 
    \label{cor1}
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:large-d} with $\epsilon = \frac{1}{T^2}$ and edge-length sequence $ r_m = 2^{-m} $. For each total time horizon $ T \in \mathbb{N} $ such that $ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 8 C_z \log ( T ) \kappa_s T } }{4 C_z \log ( T ) } \) - d_z  > 0 $, let $ k = \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 8 C_z \log ( T ) \kappa_s T } }{4 C_z \log ( T ) } \) - d_z }{ d_s } $. 
    % Define the edge-length sequence as 
    % $ Let $ \epsilon = \frac{1}{T^2} $ and 
    Then there exists a sequence $ \{ G_T \}_{T} $ such that (1) $ G_T = O \( \( \frac{T}{\log T} \)^{-\frac{1}{d_s}} \) $, and (2) for each $T \in \mathbb{N}$,
    with probability exceeding $ 1 - \frac{1}{T} $, the final optimality gap of Algorithm \ref{alg:large-d} is no larger than $ G_T $.  
\end{corollary} 

\begin{proof} 
    % It suffices to consider large $T$. 
    % When $k = \frac{}{} $
    By letting $ k = \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 8 C_z \log ( T ) \kappa_s T } }{4 C_z \log ( T ) } \) - d_z }{ d_s } $ in Theorem \ref{thm:large-d}, we know as $T$ approaches infinity, the value of $ \( \frac{ \kappa T (2^{d_z + kd_s} -1) }{2 C_z \log (T ) 2^{d_z + kd_s}} \)^{- \frac{ 1+k }{d_z + kd_s}} $ is of order $ O \( \( \frac{T}{\log T} \)^{-\frac{1}{d_s}} \) $. 
\end{proof} 

In addition, BLiN-MOS only needs $O (\log \log T)$ rounds of communications to asymptotically achieve the $O (T^{-\frac{1}{d_s}})$ regret bound, as stated in the following theorem. 
 
% \textcolor{red}{(Draw a figure to illustrate the algorithm procedure. )} 

% \subsection{When $d_z$ is small}
% : Simple is Good} 

% \textcolor{red}{Task for Yasong: Summarize some results from \citep{feng2023hpo}. } 

% \input{./tex/blie-theory.tex}

% \begin{lemma}
%     \label{lem:survive-small} 
%     Instate Assumption \ref{assumption:lip}. 
%     Throughout the entire procedure of Algorithm \ref{alg:small-d}, the optimal arm $x^*$ is not eliminated. 
% \end{lemma} 

% \begin{proof}
%     For any batch $m$, let $q_m^*$ be the cube in $\A_m$ that contains $x^*$, and let $q_m^{\max}$ be the cube in batch $m$ such that $ f (x_{q_m^{\max}}) = Y_m^{\max} $. Then for any $m = 1,2,\cdots$, we have 
%     \begin{align*}
%         Y_m^{\max} - f ( x_{q_m^*} ) 
%         = 
%         f ( x_{q_m^{\max}} ) - f ( x_{q_m^*} ) 
%         \overset{(i)}{\le} 
%         f ( x_{q_m^{\max}} ) - f^*  + L 2^{-m} 
%         \le 
%         L 2^{-m} , 
%     \end{align*}
%     where $(i)$ follows from Lipschitzness of $f$. 
%     The above derivation implies that $ q_m^* $ is not eliminated. Thus $x^*$ is not eliminated. 
%     % Let $q_m^*$ be a cube in $\mathcal{A}_m$ that contains $x^*$, and let $q_m^{\max} \in \arg \max_{q \in \mathcal{A}_m} {Y}_{q, n_m}^{\max} $.
%     % Under the event $\mathcal{E}$, we have 
%     % \begin{align*} 
%     %     \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} )) 
%     %     = 
%     %     \wh{c}_{n_m, \alpha_m} (f (X_{I_m^{\max}} )) - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} ))  
%     %     \le 
%     %     f_{I_m^{\max}}^* - f_{I_m^{*}}^* + \rho_m 
%     %     \le 
%     %     \rho_m , 
%     % \end{align*} 
%     % which implies that $ I_m^* $ is not eliminated. 
% \end{proof} 

% \begin{lemma} 
%     \label{lem:y-gap-small}
%     % Let $ f^* = \max_{x \in [0,1]^d} f (x) $. 
%     % Under event $\mathcal{E}$, 
%     Instate Assumption \ref{assumption:lip}. Then it holds that 
%     $f^* - Y_{m}^{\max} \le L2^{-m}$ for all $m = 1,2,\cdots$. 
% \end{lemma} 

% \begin{proof} 
%     Let $ q_m^* $ be the cube in $\mathcal{A}_m$ that contains $x^*$, and let $q_m^{\max}$ be the cube in batch $m$ such that $ f (x_{q_m^{\max}}) = Y_m^{\max} $. Then we have 
%     \begin{align*} 
%         f^* - Y_{m}^{\max} 
%         = 
%         f_{q_m^*}^{\max} - f (x_{q_m^{\max}})
%         \le 
%         f ( x_{q_m^*} ) + L2^{-m} - Y_{m}^{\max} 
%         \le 
%         L 2^{-m} . 
%     \end{align*} 
% \end{proof} 


% \begin{lemma} 
%     \label{lem:opt-gap-small}
%     Instate Assumption \ref{assumption:lip}.  The arms in $\mathcal{A}_m$ are $ L 2^{-m+1} $-optimal for all $ m = 1, 2, \cdots $. 
% \end{lemma} 

% \begin{proof} 
%     % The arms in $\mathcal{A}_m$ are 
%     Let $q$ be a cube in $\mathcal{A}_m $. By Lemma \ref{lem:y-gap-small}, we have 
%     \begin{align*}
%         % f_{q_m^*}^{\max} - f_q^{\max} 
%         % \le 
%         f_{q_m^*}^{\max} - f_q^{\max} 
%         \le 
%         Y_{q_m^*,n_m} + L 2^{-m} - Y_{q,n_m} 
%         \le 
%         Y_{m}^{\max} + L 2^{-m} - Y_{q,n_m} 
%         \le 
%         L 2^{- 2 m + 1 }, 
%     \end{align*}
%     where the last inequality follows from the fact that $ q $ is not eliminated. The above inequalities imply that
%     % it holds that 
%     \begin{align*}
%         f^* - f_{q}^{\min} 
%         \le 
%         f_{q_m^*}^{\max} - f_q^{\max} + L 2^{-m} 
%         \le
%         L 2^{-m} + L 2^{-2m+1} 
%         \le 
%         L 2^{-m+1}. 
%         % 
%     \end{align*}
% \end{proof} 



% -----------------------------------------------------------------


% We let $B$ be the total number of batches of the BLiE run ($B-1$ batches in the for-loop and $1$ clean-up batch), and $N_m$ be the total budget of batch $m$. In the following analysis, we bound $N_m$ for $m=2k-1$ and $m=2k$ separately, and then obtain the simple regret upper bound.

% Firstly, we consider the case $m=2k-1$. For convenience, we let $\widetilde{r}_k=2^{-\sum_{i=1}^kc_i}$, and thus we have $\widetilde{r}_{k-1}\geq r_{m-1}\geq r_m\geq \widetilde{r}_{k}$. Recall that $\mathcal{A}_{m-1}^+$ is set of cubes not eliminated in batch $m-1$, and $\cup_{C\in\mathcal{A}_{m-1}^+}C=\cup_{C^\prime\in\mathcal{A}_m}C^\prime$. Lemma \ref{lem:eli} implies that each cube in $\mathcal{A}_{m-1}^+$ is a subset of $S((4L+4)r_{m-1})$, and thus $\left|\mathcal{A}_{m-1}^+\right|\leq N_{r_{m-1}}\leq C_z\cdot r_{m-1}^{-d_z}$. The total budget of batch $m$ is
% \begin{align*}
%     N_m=& \; |\mathcal{A}_m|\cdot n_m = \left(\frac{r_{m-1}}{r_m}\right)^d\left|\mathcal{A}_{m-1}^+\right|\cdot n_m\\
%     \leq& \; C_z\cdot\frac{r_{m-1}^{d+1-d_z}\cdot r_m^{-d-\beta}}{r_{m-1}} 
%     \leq C_z\cdot\frac{\widetilde{r}_{k-1}^{d+1-d_z}\cdot\widetilde{r}_k^{-d-\beta}}{r_{m-1}}.
% \end{align*}
% For the numerator, we have
% \begin{align*}
%     \widetilde{r}_{k-1}^{d+1-d_z}\cdot\widetilde{r}_k^{-d-\beta}
%     =& \; 2^{-\left(\sum_{i=1}^{k-1}c_i\right)(d+1-d_z)+\left(\sum_{i=1}^{k}c_i\right)(d+\beta)} \\ 
%     =& \; 2^{\left(\sum_{i=1}^{k-1}c_i\right)(d_z+\beta-1)+c_m(d+\beta)}.
% \end{align*}
% Define $C_m=\left(\sum_{i=1}^{k-1}c_i\right)(d_z+\beta-1)+c_m(d+\beta)$. Since $c_m=c_{m-1}\cdot\frac{d+1-d_z}{d+\beta}$, calculation shows that $C_m = (\sum_{i=1}^{m-2} c_i) (d_z+\beta-1)  + c_{m-1}(d+\beta)+ c_{m-1}(d_z+\beta-1-d-\beta)+c_m(d+\beta)=C_{m-1}$. Thus for any $m$, we have $C_M=C_1=\frac{d_z+\beta-1}{d_z+\beta}\log T$. Hence,
% \begin{equation*}
%     N_m\leq C_z\cdot2^{\frac{d_z+\beta-1}{d_z+\beta}\log T}/r_{m-1}=C_z\cdot T^{\frac{d_z+\beta-1}{d_z+\beta}}/r_{m-1}.
% \end{equation*}

% Secondly, we consider the case $m=2k$. Lemma \ref{lem:eli} implies that each cube in $\mathcal{A}_m$ is a subset of $S(8L+8)r_m$. Similar argument to the first case shows that $\left|\mathcal{A}_m\right|\leq C_z\cdot r_m^{-d_z}$ and $N_m\leq C_z\cdot r_m^{-(d_z+\beta)}$.

% % The rounding step in Definition \ref{def:ace} yields that $r_m\leq\frac{r_{m-1}}{2}$ for any $m$. 
% Line 7 of Algorithm \ref{BLiN} ensures that the sum of budgets of full $B$ batches is greater than $T$. Therefore, combining the above two cases, we have
% \begin{align}\label{upp-budget-ace}
%     T\leq&\sum_{\substack{m=2k-1, \\ m\leq B }}C_z \cdot\frac{T^{\frac{d_z+\beta-1}{d_z+\beta}}}{r_{m-1}}+\sum_{\substack{m=2k,\\m\leq B}}C_z\cdot \frac{1}{r_m^{d_z+\beta}}.
% \end{align}

% % \begin{align}\label{upp-budget-ace}
% %     T\leq&\sum_{\substack{m=2k-1, \\ m\leq B }}C_z\cdot T^{\frac{d_z+\beta-1}{d_z+\beta}}\cdot\frac{1}{r_{m-1}}+\sum_{\substack{m=2k,\\m\leq B}}C_z\cdot \frac{1}{r_m^{d_z+\beta}}\nonumber\\
% %     \leq&2C_z\cdot T^{\frac{d_z+\beta-1}{d_z+\beta}}\cdot\frac{1}{r_{B}}+2C_z\cdot\frac{1}{r_{B}^{d_z+\beta}}.
% % \end{align}
% The rounding step in Definition \ref{def:ace} yields that $r_m\leq\frac{r_{m-1}}{2}$ for any $m$. If $B$ is odd, from (\ref{upp-budget-ace}) we have $T\leq2C_z\cdot T^{\frac{d_z+\beta-1}{d_z+\beta}}\cdot\frac{1}{r_{B-1}}+2C_z\cdot\frac{1}{r_{B-1}^{d_z+\beta}}$.  We set $c_r=\max\{(4C_z)^\frac{1}{d_z+\beta}, 4C_z\}$, then $\frac{1}{c_r^{d_z+\beta}}+\frac{1}{c_r}\leq\frac{1}{2C_z}$ and the above inequality implies that $r_{B-1}\leq c_r\cdot T^{-\frac{1}{d_z+\beta}}$. Lemma \ref{lem:eli} shows that $\Delta_x\leq(4L+4)r_{B-1}$ for any $x\in\cup_{C\in\mathcal{A}_B}C$, so we have $\Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z+\beta}}$, where $c=(8L+8)\cdot\max\{c_r, 1\}$. If $B$ is even, similar arguments also yleid that $\Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z+\beta}}$. See Appendix \ref{app:race} for details.

% Finally, we consider the communication bound. For any $B^*$, $\widetilde{r}_{B^*}=2^{-\sum_{i=1}^{B^*}c_i}=2^{-c_1\cdot\frac{1-\eta^{B^*}}{1-\eta}}=T^{-\frac{1}{d_z+\beta}}\cdot T^{\frac{\eta^{B^*}}{d_z+\beta}}$. Then by choosing $B^*\geq\frac{\log\log T-\log(d_z+\beta)}{\log\frac{d+\beta}{d+1-d_z}}$, we have $\frac{\eta^{B^*}}{d_z+\beta}\leq\log T$ and $\widetilde{r}_{B^*}\leq T^{-\frac{1}{d_z+\beta}}$. Definition \ref{def:ace} shows that $r_m<\widetilde{r}_{B^*}$ for any $m\geq2B^*$. As a consequence, no more than $\hat{B}=\frac{2\log\log T}{\log\frac{d+\beta}{d+1-d_z}} + 1$ batches are needed to achieve $r_{\hat{B}-1}\leq T^{-\frac{1}{d_z+\beta}}$ and $\Delta_{\widetilde{x}^*}\leq (4L+4)T^{-\frac{1}{d_z+\beta}}\leq c\cdot T^{-\frac{1}{d_z+\beta}}$.

-----------------------------------------------------------------



\subsection{When $d_s$ is small} 
% : Max Order Statistics (MOS) is Helpful} 


% \begin{assumption}
%     \label{assumption:ord}
%     % We assume that the following items are true. 
%     % \begin{itemize}
%     There exists $\kappa \in (0,1) $, such that for any $\alpha \in [0, \frac{ 1 }{2} ]$, and any cube $q$
%     \begin{align*} 
%         \Pr \( f ( X_q ) \le f_q^{\max} -  \alpha ( f_q^{\max} - f_q^{\min} ) \) 
%         \le 
%         1 - \kappa \alpha . 
%     \end{align*} 
% \end{assumption}


Let $X_q$ denote the uniform random variable over $ q $.  




Consider $iid$ random variables $X_q^1, X_q^2, \cdots, X_q^n \in q $ and $Y_{q,n} = \max\{ f (X_q^1), f(X_q^2), \cdots, f(X_q^n) \} $. 
\begin{align*} 
    \Pr \( Y_{q,n} \le x \) 
    = 
    \prod_{i=1}^n \Pr \( f(X_q^i) \le x \) . 
\end{align*} 





% \begin{algorithm}[h]
% 	\caption{Optimization via Max Order Statistic (over $[0,1]^d$)} 
% 	\label{alg:new} 
% 	\begin{algorithmic}[1]  
%             \STATE \textbf{Assumption:} Suppose that the function $f$ has zooming dimension $d_z$ and zooming constant $C_z$. 
% 		\STATE \textbf{Input:} Time horizon $T$. $\epsilon \in (0,1)$. 
% 		\STATE \textbf{Initialization:} 
%   % Let $ \mathcal{A}_1 = \{ [0, \frac{1}{2}] , [\frac{1}{2}, 1] \} $. Let $ N_0 = 256A_\epsilon $. Let $ M = \lfloor \frac{ \log \( \frac{\gamma-1}{\gamma}\cdot \frac{T}{C_z N_0 } \) }{\log \gamma } \rfloor$. 
% 		\FOR{$m=1,2,\cdots,M$} 
%                 \STATE Compute $ n_m = \frac{\log \epsilon }{ \log \(1 - \kappa 2^{-m} \) } $. 
%                 % $\alpha_m = 1-(\frac{256 A_\epsilon }{ n_m })^{1/4} $, $\rho_m = 6 \kappa_+ \( \frac{A_\epsilon}{n_m} \)^{1/4} 2^{-m}$. 
%                 \FOR{cube $q \in \mathcal{A}_{m} $} 
%                     \STATE Uniformly randomly sample $n_m$ points from $q$, and compute $ Y_{q, n_m } $. 
%                     \STATE Compute $ Y_m^{\max} := \max_{q \in \mathcal{A}_m } Y_{q,n_m} $. 
%                     \STATE Let $\mathcal{A}_{m+\frac{1}{2}} = \{ q \in  \mathcal{A}_m : {Y}_m^{\max} - {Y}_{q,n_m} \le \rho_m \}$. /* Elimination step */
%                     \STATE Dyadically partition the cubes in $\mathcal{A}_{m + \frac{1}{2}}$, and collect these intervals to form $ \mathcal{A}_{m+ 1 } $. 
%                     % = \{ I: \in  \mathcal{A}_{m+\frac{1}{2}} : \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m } \le \rho_m \} $
%                 \ENDFOR 
% 		\ENDFOR
%             \STATE \textbf{Output}: $Y_{M}^{\max}$. 
%     % \STATE \textbf{Cleanup:} Arbitrarily play the remaining arms until all $T$ steps are used.  
% 	\end{algorithmic} 
% \end{algorithm} 


\begin{lemma}
    \label{lem:hp}
    Instate Assumptions \ref{assumption:lip}. For any $\alpha \in (0,1)$, any positive integer $n$ and any cube $q^*$ such that $x^* \in q^*$, it holds that 
    \begin{align*}
        \Pr \( f_{q^*}^{\max} - Y_{q^*,n} > \alpha L \D (q^*) \) 
        \le& \;  
        % \Pr \( f_q^{\max} - Y_{q,n} \ge \alpha \( f_q^{\max} - f_q^{\min} \) \) \\ 
        % =& \; 
        % \Pr \(  Y_{q,n} \le f_q^{\max} - \alpha \( f_q^{\max} - f_q^{\min} \) \) \\ 
        % =& \; 
        % \prod_{i=1}^n \Pr \( f ( X_q^i ) \le f_q^{\max} - \alpha \( f_q^{\max} - f_q^{\min} \) \) \\ 
        % \le& \; 
        (1 - \kappa_s \alpha^{d_s} )^n . 
    \end{align*}
    
    % Fix any $\epsilon \in (0,1)$, and let $ n_m = \frac{\log \epsilon}{(1 - \kappa 2^{-m})} $. Then we have 
    % \begin{align*} 
    %     \Pr \( f_q^{\max} - Y_{q,n_m} \le 2^{-m} \) \ge 1 - \epsilon .  
    % \end{align*} 
\end{lemma}

\begin{proof}
    It holds that 
    \begin{align*}
        \Pr \( f_{q^*}^{\max} - Y_{q^*,n} > \alpha L \D (q^*) \) 
        \le& \;  
        \Pr \( f_{q^*}^{\max} - Y_{q^*,n} > \alpha \( f_{q^*}^{\max} - f_{q^*}^{\min} \) \) \tag{by $L$-Lipschitzness} \\ 
        =& \; 
        \Pr \(  Y_{q^*,n} < f_{q^*}^{\max} - \alpha \( f_{q^*}^{\max} - f_{q^*}^{\min} \) \) \\ 
        =& \; 
        \prod_{i=1}^n \Pr \( f ( X_{q^*}^i ) < f_{q^*}^{\max} - \alpha \( f_{q^*}^{\max} - f_{q^*}^{\min} \) \) \\ 
        \le& \;  
        \( 1 - \kappa_s \alpha^{d_s} \)^n , 
        % \tag{by Assumption \ref{assumption:ord} and that $\{ X_{q^*}^i\}_{i=1}^n $ are $iid$} 
    \end{align*} 
    where the last inequality follows from Definition of scattering dimension and that $\{ X_{q^*}^i\}_{i=1}^n $ are $iid$.  
\end{proof} 

\begin{lemma} 
    \label{lem:event}
    Denote $ \rho_m = L \alpha_m r_m$. Let $n_m$ be defined as in Algorithm \ref{alg:large-d}. Let 
    \begin{align*} 
        \mathcal{E} := \left\{ f_q^{\max} - Y_{q,n_m} \le \rho_m, \; \forall m = 1,2,\cdots, M,\; \text{ and } \;  \forall q \in \mathcal{A}_m \text{ such that } x^* \in q \right\} , 
    \end{align*} 
    and let $\epsilon = \frac{1}{T^2}$. 
    Then $\Pr \( \mathcal{E}\) \ge 1 - \frac{1}{T}$. 
\end{lemma} 

\begin{proof} 

    Since at most $T$ arms are pulled, there are at most $T$ cubes that contain arms. We apply Lemma \ref{lem:hp} and take a union bound over these cubes to conclude the proof. 
\end{proof} 

\begin{proposition}
    \label{prop:inc}
    Let $\kappa \in (0,1]$ and $\gamma > 1$. 
    For any $ x \in [1,\infty) $, it holds that 
    \begin{align*}
        - \frac{\gamma^{x}}{\gamma \log (1 - \frac{\kappa}{\gamma}) } \le - \frac{1}{\log(1 - \kappa \gamma^{-x})} \le \frac{\gamma^{x}}{\kappa}. 
    \end{align*} 

\end{proposition}

\begin{proof}
    Consider function $h: [1, \infty ) \to \R$ defined as 
    \begin{align*} 
        h (x) = - \frac{\kappa }{ \gamma^x \log(1 - \kappa \gamma^{-x}) } . 
    \end{align*} 
    Clearly, $h(1) = - \frac{\kappa }{ \gamma \log (1 - \frac{\kappa}{\gamma}) } $. By noting $ \log(1 - \kappa \gamma^{-x}) = - \kappa \gamma^{-x} + o (\gamma^{-x})$ when $x$ is large, we know that 
    \begin{align*}
        \lim_{x \to \infty} h (x) = 1. 
    \end{align*} 
    Also, we know that 
    \begin{align*}
        h' (x) = \frac{\kappa \gamma^x \log \gamma}{ (\gamma^x \log (1 - \kappa \gamma^{-x}) )^2 } \( \log \( 1 - \kappa \gamma^{-x} \) + \frac{\kappa \gamma^{-x}}{1 - \kappa \gamma^{-x}} \). 
    \end{align*}
    Since $ \log (1-z) \ge \frac{-z}{\sqrt{1-z}} $ for all $z \in (0,1)$, we know $ h' (x) > 0 $ for all $x \in [1,\infty)$. 
    Thus $ h $ is increasing over $ [1,\infty) $. Therefore $ - \frac{\gamma^{x}}{\gamma \log (1 - \frac{\kappa}{\gamma}) } \le - \frac{1}{\log(1 - \kappa \gamma^{-x})} \le \frac{\gamma^{x}}{\kappa} $ for all $x \in [1,\infty)$. 
\end{proof}









\iffalse
\begin{lemma}
    \label{lem:survive} 
    Under the event $\mathcal{E}$, the optimal arm $x^*$ is not eliminated. 
\end{lemma} 

\begin{proof}
    Let $q_m^*$ be the cube in batch $m$ that contains $x^*$. Let $q_m^{\max}$ be the cube in batch $m$ such that $ Y_{q_m^{\max},n} =   Y_m^{\max} $. Then we have 
    \begin{align*}
        Y_m^{\max} - Y_{q_m^*,n}  
        = 
        Y_{q_m^{\max}}^{\max} - Y_{q_m^*,n}  
        \le 
        f_{q_m^{\max}}^{\max} - f_{q_m^{*}}^{\max} + L 2^{-2m} 
        \le 
        L 2^{-2m} , 
    \end{align*}
    which implies that $ q_m^* $ is not eliminated. Thus $x^*$ is not eliminated. 
    % Let $q_m^*$ be a cube in $\mathcal{A}_m$ that contains $x^*$, and let $q_m^{\max} \in \arg \max_{q \in \mathcal{A}_m} {Y}_{q, n_m}^{\max} $.
    % Under the event $\mathcal{E}$, we have 
    % \begin{align*} 
    %     \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} )) 
    %     = 
    %     \wh{c}_{n_m, \alpha_m} (f (X_{I_m^{\max}} )) - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} ))  
    %     \le 
    %     f_{I_m^{\max}}^* - f_{I_m^{*}}^* + \rho_m 
    %     \le 
    %     \rho_m , 
    % \end{align*} 
    % which implies that $ I_m^* $ is not eliminated. 
\end{proof} 

\begin{lemma} 
    \label{lem:y-gap}
    Let $ f^* = \max_{x \in [0,1]^d} f (x) $. 
    Under event $\mathcal{E}$, $f^* - Y_{m}^{\max} \le L2^{-2m}$. 
\end{lemma} 

\begin{proof} 
    Let $ q_m^* $ be the cube in $\mathcal{A}_m$ that contains $x^*$. Then we have 
    \begin{align*} 
        f^* - Y_{m}^{\max} 
        = 
        f_{q_m^*} - Y_{m}^{\max} 
        \le 
        Y_{q_m^*, n_m} + L2^{-2m} - Y_{m}^{\max} 
        \le 
        L 2^{-2m} . 
    \end{align*} 
\end{proof} 


\begin{lemma} 
    \label{lem:opt-gap}
    Under event $\mathcal{E}$, the arms in $\mathcal{A}_m$ are $ L 2^{-m+1} $-optimal for all $ m = 1,2,\cdots, M $. 
\end{lemma} 

\begin{proof} 
    % The arms in $\mathcal{A}_m$ are 
    Let $q$ be a cube in $\mathcal{A}_m $. By Lemma \ref{lem:y-gap}, we have 
    \begin{align*}
        % f_{q_m^*}^{\max} - f_q^{\max} 
        % \le 
        f_{q_m^*}^{\max} - f_q^{\max} 
        \le 
        Y_{q_m^*,n_m} + L 2^{-2m} - Y_{q,n_m} 
        \le 
        Y_{m}^{\max} + L 2^{-2m} - Y_{q,n_m} 
        \textcolor{red}{\le 
        L 2^{-2m+1}}, 
    \end{align*}
    where the last inequality follows from the fact that $ q $ is not eliminated. The above inequalies imply that
    % it holds that 
    \begin{align*}
        f^* - f_{q}^{\min} 
        \le 
        f_{q_m^*}^{\max} - f_q^{\max} + L 2^{-m} 
        \le
        \textcolor{red}{L 2^{-m} + L 2^{-2m+1} 
        \le 
        L 2^{-m+1}}. 
        % 
    \end{align*}
\end{proof} 
\fi


\begin{lemma}
    \label{lem:survive}
    Under the event $\mathcal{E}$, the optimal arm $x^*$ is not eliminated.
\end{lemma}

\begin{proof}
    Let $q^*_m$ be the cube in batch $m$ that contains $x^*$. Let $q_m^{\max}$ be the cube in batch $m$ such that $Y_{q_m^{\max},n_m} = Y_m^{\max}$. Then we have
    \begin{equation*}
    Y_m^{\max} - Y_{q_m^*,n_m} = Y_{q_m^{\max},n_m} - Y_{q_m^*,n_m} \leq f_{q_m^{\max}}^{\max} - f^{\max}_{q^*_m} + \rho_m \leq \rho_m,
    \end{equation*}
    which implies that $q^*_m$ is not eliminated in batch $m$. Thus $x^*$ is not eliminated.
\end{proof}


\begin{lemma}
    \label{lem:y-gap}
    Let $f^* = \max_{x\in [0,1]^d}f(x)$. Under event $\mathcal{E}$, $f^*-Y_m^{\max} \leq \rho_m$.
\end{lemma}

\begin{proof}
    Let $q^*_m$ be the cube in $\mathcal{A}_m$ that contains $x^*$. Then we have
    \begin{equation*}
    f^* - Y_m^{\max} = f^{\max}_{q^*_m} - Y_{q_m^{\max},n_m} \overset{(i)}{\leq} Y_{q^*_m,n_m} + \rho_m - Y_{q_m^{\max},n_m} \leq \rho_m, 
    \end{equation*}
    where $(i)$ follows from the definition of $\mathcal{E}$ (in Lemma \ref{lem:event}).
    % the first inequality holds because we indicated in Lemma \ref{lem:survive} that $q^*_m$ is not eliminated in batch $m$.
\end{proof}


\begin{lemma}
    \label{lem:opt-gap}
    Under event $\mathcal{E}$, for any $m = 1,2,\cdots,M$, any $q_m \in \mathcal{A}_m$ and any $x\in q_m$, $\Delta_x$ satisfies
    $$
    \Delta_x \leq 3Lr_{m-1},
    $$
    where $L$ is the Lipschitz constant of $f(x)$.
\end{lemma}

\begin{proof}
    Let $q_m$ be a cube in $\mathcal{A}_m$ and let $x \in q_m$. By the Lipschitzness of $f$, we have
    \begin{equation*}
        |f(x) - Y_{q_m,n_m}| \leq Lr_m
    \end{equation*}
    Denote $Par(q_m)$ as the cube in $\mathcal{A}_{m-1}$ which contains $q_m$. Since $x \in q_m$, we know $x \in Par(q_m)$ and $Par(q_m)$ is not eliminated after batch $m-1$. Hence, it follows that $Y_{m-1}^{\max} - Y_{Par(q_m),n_{m-1}} \leq \rho_{m-1}$. Therefore,
    \begin{equation*}
    \begin{aligned}
        && f^* - f(x) & \leq Y_{m-1}^{\max} + \rho_{m-1} - Y_{Par(q_m),n_{m-1}} + Lr_{m-1} \\
        && & \leq 2\rho_{m-1} + Lr_{m-1} \\
        && & \leq 3Lr_{m-1}
    \end{aligned}
    \end{equation*}
    
\end{proof}



% \begin{lemma} 
%     Let $ f^* = \max_{x \in [0,1]^d} f (x) $. 
%     Under event $\mathcal{E}$, $f^* - Y_{m}^{\max} \le L2^{-2m}$. 
% \end{lemma} 

% \begin{proof} 
%     Let $ q_m^* $ be the cube in $\mathcal{A}_m$ that contains $x^*$. Then we have 
%     \begin{align*} 
%         f^* - Y_{m}^{\max} 
%         = 
%         f_{q_m^*} - Y_{m}^{\max} 
%         \le 
%         Y_{q_m^*, n_m} + L2^{-2m} - Y_{m}^{\max} 
%         \le 
%         L 2^{-2m} . 
%     \end{align*} 
% \end{proof} 

% So the simple regret is 
% \begin{align*}
    
% \end{align*}

% \textcolor{red}{some }

% \section*{Some Draft Below} 

\begin{proof}[Proof of Theorem \ref{thm:large-d}]
    
    Let $d_z$ be the zooming dimension. Then by Lemma \ref{lem:opt-gap}, we have 
    \begin{align*} 
        | \mathcal{A}_m | \le C_z 2^{m d_z}. 
    \end{align*} 
    
    
    In total we play $T$ arms, and thus 
    \begin{align*} 
        \sum_{m=1}^{M^*} | \mathcal{A}_m | n_m = T . 
    \end{align*} 
    Since $ | \mathcal{A}_m | \le C_z 2^{m d_z}$ and $n_m \le \frac{\log (1/\epsilon)}{\kappa_s } 2^{k d_s m} $, the above implies 
    \begin{align*} 
        \frac{C_z \log (1/\epsilon)}{\kappa_s } \sum_{m = 1}^{M^*}  2^{(d_z + k d_s ) m} \ge T . 
    \end{align*}
    
    Rearranging terms gives 
    \begin{align} 
        M^* \ge \frac{ \log \( \frac{ \kappa_s T (2^{d_z + k d_s} -1) }{C_z \log (1 / \epsilon ) 2^{d_z + k d_s}} \) }{ (d_z + k d_s) \log 2 } . \label{eq:lower-M-1}
    \end{align} 
    
    Therefore, the final simple regret is smaller than or equals to 
    \begin{align*} 
        f^*_q - Y^{\max}_{M^*}
        =
        \rho_{M^*}
        \le 
        L \( \frac{ \kappa T (2^{d_z + k d_s} -1) }{C_z \log (1 / \epsilon ) 2^{d_z + k d_s }} \)^{- \frac{ 1+k }{d_z + k d_s}} . 
    \end{align*} 

    % Finally, let us check the 
    The choice of $k$ in the above inequality is not arbitrary. 
    To ensure at least one round of narrowing, we need to ensure that $M^* \ge 1$. By (\ref{eq:lower-M-1}), it is sufficient to ensure that 
    \begin{align*}
        \frac{ \log \( \frac{\kappa_s T \( 2^{d_z + k d_s} - 1 \) }{ C_z \log (1/\epsilon) 2^{d_z + k d_s} } \) }{ (d_z + k d_s) \log 2 } \ge 1, 
    \end{align*}
    which implies 
    \begin{align*} 
        k \le \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } . 
    \end{align*} 

    Since $ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z > 0 $, the high probability optimality gap in the theorem statement is true for any fixed $ k \in \( 0, \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } \] $. 

\end{proof} 



------------------------------------------------------------


% \subsection{Only Very Few Batches Are Needed}  

% \begin{definition}
%     \label{def:opt-batch}
%     Denote $c_1 = \frac{d_z-1+k d_s }{(d+k d_s )(d_z+k d_s )}\log \frac{T}{\log T}$, $ c_{i+1} = \eta c_i,i\geq 1$, where $\eta = \frac{d+1-d_z}{d+k d_s }$. Let $a_n = \lfloor \sum_{i=1}^n c_i\rfloor$, $b_n = \lceil \sum_{i=1}^n c_i\rceil$. Define sequence $\{r_m\}$ as $r_m = 2^{-a_n}$ for $m = 2n-1$ and $r_m = 2^{-b_n}$ for $m = 2n$ (Here we suppose $\{r_m\}$ is a strictly decreasing sequence, see Remark \ref{rm:batch} for details). Define sequence $\{\alpha_m\}$ as $\alpha_m = r_m^k,k>0$.
% \end{definition}

% \begin{theorem} 
%     \label{thm:opt-batch} 
%     Instate Assumption \ref{assumption:lip}. Apply the sequence $\{r_m\}$ in Definition \ref{def:opt-batch} to Algorithm \ref{alg:large-d}. 
%     Let $T$ be the total time horizon such that $ (d+1-d_z) \log \frac{T}{\log T} - d d_z > 0 $ and let $\epsilon = \frac{1}{T^2}$. Let $ k \in \( 0, \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} \] $. 
%     % With fixed budget $T$, 
%     % the final simple regret satisfies 
%     Then with probability exceeding $1 - \frac{1}{T}$, the final optimality gap satisfies  
%     \begin{equation*} 
%         f^*_q - Y^{\max}_M \leq cL\left(\frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }},
%     \end{equation*} 
%     where $M$ denotes the last batch, $Y^{\max}_M$ is the estimate of $f^*_q$ after $M$ batches and $c$ is a constant independent of $T$. Moreover, only $2\times \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} +1$ total batches are needed to achieve this simple regret.
% \end{theorem} 




\begin{proof}
    Following an argument similar to that for Corollary \ref{cor1}, we conclude the proof. 
\end{proof}


% --------------------------------------------

% Note that to ensure at least one round of narrowing. We need to ensure 
% \begin{align*} 
%     \frac{\log \log \frac{T}{\log T} - \log (d_z + k d_s)}{ \log \frac{d+k d_s}{d+1 - d_z} } \ge 1, 
% \end{align*} 
% which implies 
% \begin{align*} 
%     && & k > \frac{1-d_z}{d_s}, \\
%     && & k 
%     \le 
%     \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} .
% \end{align*} 



% With this choice of $k$, the simple regret, with probability exceeding $1 - \frac{1}{T}$, is bounded by  
% \begin{align*}
%     c L \( \frac{T}{\log T} \)^{- p (T, d, d_z, d_s) }, 
% \end{align*}
% where $p(T,d, d_z,d_s) = \frac{ \frac{\sqrt{(d+d_z)^2 + 4 \( (d+1-d_z)\log \frac{T}{\log T} - d d_z \) } - (d+d_z)}{2d_s} + 1}{ \frac{\sqrt{(d+d_z)^2 + 4 \( (d+1-d_z) \log \frac{T}{\log T} - d d_z \) } - (d+d_z)}{2}  + d_z} $. 

% -------------------------------------------- 


\begin{lemma}
    \label{lem:nm}
    When $\kappa \in (0,1]$, $\alpha_m$ defined in Definition \ref{def:opt-batch} satisfies
    \begin{equation*}
        -\frac{1}{\log (1-\kappa \alpha_m^{d_s} )} \leq \frac{1}{\alpha_m^{d_s} \kappa}, \forall m \geq 1
    \end{equation*}
    In particular, for $n_m = \frac{\log \epsilon}{\log (1-\kappa_s  \alpha_m^{d_s})}$, it holds that $n_m \leq \frac{\log (1/\epsilon)}{\kappa_s \alpha_m^{d_s}}$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:nm}]
    Let $g(m) = -\frac{1}{\alpha_m^{-d_s } \log (1-\kappa \alpha_m^{ d_s })}$. From the fact that the sequence $\{\alpha_m^{d_s}\}$ is decreasing with respect to $m$ and $h(x) = -\frac{1}{x^{-1} \log(1-\kappa x)}$ is a decreasing function regarding $x \in (0,1]$, we know $\{g(m)\}$ is a sequence increasing with $m$. Since $0 < \eta < 1$, we have $\sum_{i=1}^{\infty} c_i = \frac{c_1}{1-\eta} < \infty $, which implies that both $\lim_{n\rightarrow +\infty} 2^{-kd_s \lfloor \sum_{i=1}^n c_i \rfloor} $ and $\lim_{n\rightarrow +\infty} 2^{-kd_s \lceil \sum_{i=1}^n c_i \rceil} $ are strictly larger than $0$. Hence, 
    \begin{equation*}
        \lim_{m\rightarrow +\infty} g(m) \leq \lim_{x\rightarrow 0} -\frac{x}{\log (1-\kappa x)} = \frac{1}{\kappa}\\
    \end{equation*}
    We thus obtain $g(m)\leq \frac{1}{\kappa}, \enspace i.e.\enspace -\frac{1}{\log (1-\kappa \alpha_m^{ d_s })} \leq \frac{1}{\alpha_m^{ d_s } \kappa}$.
\end{proof}


\iffalse
\begin{proof}[Proof of Theorem \ref{thm:opt-batch}]
    Denote $\tilde{r}_n = 2^{-\sum_{i=1}^n c_i}$. 
    
    When $m = 2n-1$, $r_m \geq \tilde{r}_n, r_{m-1} \leq \tilde{r}_{n-1}$. 
    Since $\Delta_x \leq 3Lr_{m-1}$ for any $x \in \cup_{q_m\in \mathcal{A}_m}q_m$, any cube in $\mathcal{A}_{m-\frac{1}{2}}$ is a subset of $S(3Lr_{m-1})$. Therefore,
    \begin{equation*}
        |\mathcal{A}_{m-\frac{1}{2}}| \leq N_{r_{m-1}} \leq C_z r_{m-1}^{-d_z}.
    \end{equation*}
    After partitioning $\mathcal{A}_{m-\frac{1}{2}}$ into $\mathcal{A}_m$, we get
    \begin{equation*}
        |\mathcal{A}_m| = \left(\frac{r_{m-1}}{r_m}\right)^d |\mathcal{A}_{m-\frac{1}{2}}| \leq \left(\frac{\tilde{r}_{n-1}}{\tilde{r}_n}\right)^d \cdot C_z r_{m-1}^{-d_z}.
    \end{equation*}
    Denote the total budget of the $m$-th batch as $N_m$, then
    \begin{equation*}
    \begin{aligned}
        && N_m = |\mathcal{A}_m| \cdot n_m & 
        \leq \left(\frac{r_{m-1}}{\tilde{r}_n}\right)^d \cdot C_z r_{m-1}^{-d_z} \cdot \frac{\log (1/\epsilon)}{\kappa_s \alpha_m^{ d_s }} 
        \leq \frac{C_z \log (1/\epsilon)}{\kappa_s } \cdot \frac{ \tilde{r}_{n-1}^{d-d_z+1} \cdot \tilde{r}_n^{-k d_s -d} }{r_{m-1}} \\
        && & = \frac{C_z \log (1/\epsilon)}{\kappa_s r_{m-1}} \cdot 2^{(d_z+k d_s -1)\sum_{i=1}^{n-1}c_i + (k 
        d_s +d)c_n}
    \end{aligned}
    \end{equation*}
    Define $C_n = (d_z+k d_s -1)\sum_{i=1}^{n-1}c_i + (k d_s +d)c_n$, then $C_n - C_{n-1} = (d_z-d-1)c_{n-1} + (k d_s +d)c_n = 0$. So for any $n > 1$, we have $C_n = C_1 = (k d_s +d)c_1$. Consequently, we obtain the upper bound of $N_m$ for $m = 2n-1$ as follows,
    \begin{equation*}
        N_m \leq \frac{C_z \log (1/\epsilon)}{\kappa_s r_{m-1}} \cdot \left(\frac{T}{\log T}\right)^{\frac{d_z+k d_s -1}{d_z+k d_s }}.
    \end{equation*}

    When $m = 2n$, $r_{m-1} = \min\{r_{m-2},2^{-a_n} \} = \min \{2^{-b_{n-1}} , 2^{-a_n} \}$. $r_{m-1} = r_{m-2}$ only happens when $\lceil \sum_{i=1}^{n-1}c_i \rceil > \lfloor \sum_{i=1}^{n}c_i \rfloor$. Under this circumstance, $r_m = 2^{-\lceil \sum_{i=1}^{n}c_i \rceil } = 2^{-\lfloor \sum_{i=1}^{n}c_i \rfloor - 1} \geq r_{m-2}$, which contradicts the assumption that $\{r_m\}$ is strictly decreasing. Therefore, it must hold that $r_{m-1} = 2^{-a_n} = 2^{-b_n + 1} = 2r_m$. We conclude from Lemma \ref{lem:opt-gap} that any cube in $\mathcal{A}_m$ is a subset of $S(6Lr_m)$.  Therefore,
    \begin{equation*}
        N_m = |\mathcal{A}_m| \cdot n_m 
        \leq \frac{C_z\log (1/\epsilon)}{\kappa_s} \cdot r_m^{-d_z} \cdot r_m^{-k d_s }
    \end{equation*}

    Since the total budgets of all $M$ batches is $T$, 
    \begin{equation*}
    \begin{aligned}
        && T & \leq \sum_{m=2n-1, m\leq M} N_m + \sum_{m=2n, m\leq M} N_m \\
        && & \leq \frac{2C_z}{\kappa} \left( \sum_{m=2n-1, m\leq M} \frac{1}{r_{m-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k d_s }} + \sum_{m=2n, m\leq M} r_m^{-d_z-k d_s } \cdot \log T\right)
    \end{aligned}
    \end{equation*}
    
    From the assumption that $\{r_m\}$ is strictly decreasing, we know $r_m \leq \frac{1}{2}r_{m-1}$ for any $m$. When $M$ is odd, $\sum_{m=2n-1,m\leq M} \frac{1}{r_{m-1}} \leq \left( \sum_{n=0}\frac{1}{2^n} \right) \cdot \frac{1}{r_{M-1}} = \frac{2}{r_{M-1}}$, $ \sum_{m=2n, m\leq M} \frac{1}{r_m^{d_z+k 
    d_s }} \leq \left(\sum_{n=0} \frac{1}{2^{n(d_z+k d_s )}}\right) \cdot {\frac{1}{r_{M-1}^{d_z+k d_s }}} = \frac{2}{r_{M-1}^{d_z+k 
    d_s }}$. Therefore, 
    \begin{equation*}
        T \leq \frac{4C_z}{\kappa_s} \cdot \left( \frac{1}{r_{M-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k 
        d_s }} + \frac{1}{r_{M-1}^{d_z+k d_s }} \cdot \log T \right).
    \end{equation*}
    Set $C = \max\{8C_z/\kappa_s,(8C_z/\kappa_s)^{\frac{1}{d_z+k 
    d_s }}\}$. If $r_{M-1} > C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$, then 
    \begin{equation*}
        \frac{4C_z}{\kappa_s} \cdot \left( \frac{1}{r_{M-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k d_s }} + \frac{1}{r_{M-1}^{d_z+k d_s }} \cdot \log T \right) < T,
    \end{equation*} 
    which yields contradiction. So we obtain $r_{M-1} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$, and $r_M \leq \frac{1}{2} C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$.

    Similarly, when $M$ is even, we have
    \begin{equation*}
        T \leq \frac{4C_z\log T}{\kappa_s} \cdot \left( \frac{1}{r_M} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} + \frac{1}{r_M^{d_z+k d_s }}\right).
    \end{equation*}
    Implementing the same deduction process as when $M$ is odd, we get $r_M \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$.

    With $r_M$ upper bounded as above, the simple regret of the last batch $M$ can achieve an order smaller than or equal to $\mathcal{O}\left( \left( \frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }} \right)$:
    \begin{equation}
        \label{eq:simple-regret}
        f^*_q - Y^{\max}_M \leq \rho_M = L\alpha_M r_M = L r_M^{1+k } \leq cL\left(\frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }},
    \end{equation}
    where $c$ is a constant.

    To see that only $ O (\log \log T) $ batches are needed, we note that $\tilde{r}_{M} = 2^{-\sum_{i=1}^{M} c_i} = 2^{-c_1 \cdot \frac{1-\eta^{M}}{1-\eta}} = \left( \frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s } + \frac{\eta^{M}}{d_z+k d_s }}$. By letting $\frac{\eta^{M^*}}{d_z+k d_s } \leq \frac{ \textcolor{red}{\tilde{C}} }{\log \frac{T}{\log T}}$ ($\tilde{C}$ is a constant determined in Remark \ref{rm:batch} ), that is, choosing $M^* \geq \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s ) \textcolor{red}{ - \log \tilde{C} } }{\log \frac{d+k d_s }{d+1-d_z}}$, we can achieve $\tilde{r}_{M^*} \leq \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$. Since $r_m \leq \tilde{r}_{M^*}$ for $m\geq 2M^*$, only $2M^*+1$ batches are needed to achieve the simple regret in (\ref{eq:simple-regret}).
    

    Finally, the choice of $k$ in the final optimality gap is not arbitrary. 
    To ensure at least one round of narrowing, we need to ensure that $M \ge 1$. By (\ref{eq:lower-M-1}), it is sufficient to ensure that 
    \begin{align*}
        \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} \ge 1, 
    \end{align*}
    which implies 
    \begin{align*} 
        % \frac{1-d_z}{d_s} < 
        k 
        \le 
        \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} . 
        % k \le \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } . 
    \end{align*} 

    % Since $ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z > 0 $, the high probability optimality gap in the theorem statement is true for any fixed $ k \in \( 0, \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } \] $. 
\end{proof}
\fi



\begin{remark}
    \label{rm:batch}
    If $c_i \geq 1$ for $i = 1,2,\cdots,M^*$, then it must hold that $\lceil \sum_{i=1}^n c_i \rceil > \lceil \sum_{i=1}^{n-1} c_i \rceil$ for $n = 1,2,\cdots,M^*$, which implies that the odd terms of $\{r_m\}$ are strictly decreasing when $m = 1,2,\cdots,2M^*$. To ensure this, we let $c_{M^*} = c_1\eta^{M^*-1} \geq 1$, which is equivalent to $M^* \leq \frac{\log \log \frac{T}{\log T} + \log(d_z-1+kd_s) - \log (d_z+kd_s) - \ log(d+1-d_z) }{\log \frac{d + kd_s}{d+1-d_z}}$. Let $\log \tilde{C} \geq \log \frac{d+1-d_z}{d_z - 1 + kd_s}$ and let $T$ be large enough such that $\log \log \frac{T}{\log T} > \log (d_z + kd_s) + \log \tilde{C}$.
\end{remark}



% \begin{assumption}
%     \label{assumption:ord}
%     There exists $\kappa \in (0,1) $, such that for any $\alpha \in [0, \frac{ 1 }{2} ]$, and any cube $q \subseteq [0,1]^d$ 
%     \begin{align*} 
%         \Pr \( f ( X_q ) \le f_q^{\max} -  \alpha ( f_q^{\max} - f_q^{\min} ) \) 
%         \le 
%         1 - \kappa \alpha . 
%     \end{align*} 
% \end{assumption}







==> tex/blin.tex <==
\section{Comparison to Lipschitz Bandit Algorithms} 
% versus Random Search} 

The BLiN algorithm was recently introduced as an optimal solver for Lipschitz bandits with batched feedback \citep{fenglipschitz}. In particular, BLiN is simultaneously achieves state-of-the-art regret rate, optimal space and time complexity, and optimal communication bound. Later, 
% the authors found that the 
BLiN was applied to HPO tasks, and \citet{feng2023hpo} found that when the zooming dimension is small, BLiN outperforms existing HPO methods, and founds a better noise schedule for diffusion models \citep{}, compared to existing HPO methods. In this section, we compare Random Search and BLiN, using the notions of scattering dimension and zooming dimension. We summarize the procedure of BLiN in Algorithm \ref{alg:small-d}. 


\begin{algorithm}[ht] 
	\caption{Batched Lipschitz Narrowing (BLiN)} 
	\label{alg:small-d} 
	\begin{algorithmic}[1]  
		\STATE \textbf{Input.} Arm set $\A=[0,1]^d$; time horizon $T$.
		\STATE \textbf{Initialization} Number of batches $M$; Edge-length sequence $\{r_m\}_{m=1}^{M+1}$; The first grid point $t_0=0$; Equally partition $\mathcal{A}$ to $r_1^d$ subcubes and define $\mathcal{A}_{1}$ as the collection of these subcubes. 
		% \STATE Compute $n_m=\frac{16\log T}{r_m^2}$ for $m=1,\cdots,B+1$.
		
		\FOR{$m=1,2,\cdots,M$}
			\STATE For each cube $q\in\mathcal{A}_m$, pick an arm $x_{q} $ from $q$.
			% \STATE Collect the rewards of all pulls up to $t_m$. Compute the average payoff $\wh{\mu}_m(C)=\frac{\sum_{i=1}^{n_m}y_{C,i}}{n_m}$ for each cube $C\in\mathcal{A}_m$.
% 			\STATE $tp=tp+n_m\cdot|\mathcal{A}_m|$.
			\STATE Compute   $Y_m^{\max}=\max_{q\in\mathcal{A}_m} f(x_q)$.
			\STATE Let $\mathcal{A}_{m+\frac{1}{2}} = \{ q \in \mathcal{A}_m: Y_m^{\max} - f (x_q) \le 2L r_m \} $. 
                % \STATE For each cube $C\in\mathcal{A}_m$, eliminate $C$ if $\wh{\mu}_m^{max}-\wh{\mu}_m(C)>4r_m$. Let $\mathcal{A}_m^+$ be set of cubes not eliminated. 
			\STATE Compute $t_{m+1}=t_m+(r_{m}/r_{m+1})^d\cdot|\mathcal{A}_{m + \frac{1}{2}} | $. 
                \IF{$t_{m+1}\geq T$}
                    \STATE Let $M^* = m$. \textbf{Terminate} the algorithm and \textbf{output} $ Y_{M^*}^{\max} $.  /* The last line of the algorithm is not executed if we enter this if condition */
                \ENDIF
                % If  or $m=B$ then let $M^* = M$ and \textbf{break}.
			\STATE Equally partition each cube in $\mathcal{A}_{m+\frac{1}{2}} $ into $\left(r_m/r_{m+1}\right)^d$ subcubes and define $\mathcal{A}_{m+1}$ as the collection of these subcubes. 
   % /*\textit{See Remark \ref{remark:race} for more details on cases where $\left(r_m/r_{m+1}\right)^d$ is not an integer.}*/
		\ENDFOR
            \STATE Let $M^* = M$ and \textbf{output:} $ Y_{M^*}^{\max} $. 
    % \STATE \textbf{Cleanup:} Arbitrarily play the remaining arms until all $T$ steps are used.  
	\end{algorithmic} 
\end{algorithm} 

\begin{definition} 
    \label{def:ace} 
    For a problem with ambient dimension $d$, zooming dimension $d_z$ and time horizon $T$, we denote $c_1=\frac{d_z-1}{d_z\cdot d}\log T$ and $c_{i+1} = {\eta c_i }$ for any $i\ge 1$, where $\eta=\frac{d+1-d_z}{d}$. Then we let $a_n=\lfloor\sum_{i=1}^nc_i\rfloor$, $b_n=\lceil\sum_{i=1}^nc_i\rceil$, and inductively define ACE Sequence $\{r_m\}_{m\in\mathbb{N}}$ as $r_m=\min\{r_{m-1}, 2^{-a_n}\}$ for $m=2n-1$ and $r_m=2^{-b_n}$ for $m=2n$. \textcolor{red}{Since every $c_i$ is positive, it is easy to see $\{r_m\}$ is a decreasing sequence.} 
    % If there exists $m$ such that $r_m=r_{m-1}$, then we skip the $m$-th batch when using ACE Sequence in BLiN.} 
\end{definition} 
Then we show that BLiN with ACE Sequence can achieve simple regret $\mathcal{O}(T^{-\frac{1}{d_z}})$ using only $\mathcal{O}(\log\log T)$ batches. 

The performance of BLiN is summarized below in Theorem \ref{thm:ace}. 

\begin{theorem}\label{thm:ace}

Output arm $\widetilde{x}^*$ of BLiN algorithm with total time horizon $T$ and ACE Sequence $\{r_m\}$ satisfies 
\begin{equation*}
    \Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z}},
\end{equation*}
where $d_z$ is the zooming dimension and $c$ is a constant. In addition, BLiN needs $\mathcal{O}(\log\log T)$ batches to achieve this simple regret.
\end{theorem} 

% \begin{lemma}\label{lem:concen}
%     For any cube $C\in\mathcal{A}_m$, selected arm $x_C$ and any arm $x\in C$,
%     \begin{equation*}
%         |\ell(x_C,n_m)-\mu(x)|\leq L\cdot r_m + n_m^{-\frac{1}{\beta}}.
%     \end{equation*}
% \end{lemma}
% \begin{proof}
%     Fix a cube $C\in\mathcal{A}_m$ and the selected arm $x_C$. Assumption \ref{ass:hoeffding} gives that
%     \begin{align*}
%         |\ell(x_C, n_m)-\mu(x_C)|\leq n_m^{-\frac{1}{\beta}}.
%     \end{align*}
%     By Lipschitzness of $\mu$, it is obvious that 
%     \begin{align*}
%         \left|\mu(x_C)-\mu(x)\right|\leq L\cdot r_m, \quad \forall x \in C.
%     \end{align*} 
%     Consequently, we have $|\ell(x_C,n_m)-\mu(x)|\leq L\cdot r_m + n_m^{-\frac{1}{\beta}}$.
% \end{proof} 

\begin{lemma}\label{nel}
    The optimal arm $x^*=\arg\max f(x)$ is not eliminated in a BLiN run.
\end{lemma}

\begin{proof}
    We use $q^*_m$ to denote the cube containing $x^*$ in $\A_m$. Here we proof that $q^*_m$ is not eliminated in round $m$.
    	
    For any cube $q \in \A_m$ and $x\in q$, we have 
    \begin{align*} 
    	f(x_{q_m^*})-f(x_q)\leq f(x^*) + L\cdot r_m- f(x) + L\cdot r_m\leq2Lr_m . 
    \end{align*} 
    Then from the elimination rule, $q^*_m$ is not eliminated. 
    % \textcolor{red}{May need to modify the elimination rule: replace $2r_m$ by $2Lr_m$}
\end{proof}

\begin{lemma}\label{lem:eli}
    For any $m\geq1$ and $x\in \cup_{q\in\mathcal{A}_m}q$, we have $\Delta_x\leq4Lr_{m-1}$.
\end{lemma}

\begin{proof}
    For $m=1$, the conclusion holds directly from the Lipschitzness of $f$. For $m>1$, let $q_{m-1}^*$ be the cube in $\A_{m-1}$ such that $x^* \in q_{m-1}^*$. From Lemma \ref{nel}, this cube $q_{m-1}^*$ is well-defined. 
    For any cube $q\in\mathcal{A}_m$ and $x\in q$, it is obvious that $x$ is also in the parent of $q$ (the cube in the previous round that contains $q$), which is denoted by $q_{par}$. 
    For any $x \in q$ and any $x_{q_{par}}$ in cube $q_{par}$, the Lipschitzness of $f$ implies that
    \begin{align*}
    	\Delta_x=f^*-f(x)\leq f(x_{q^*_{m-1}})+L \cdot r_{m-1}-f(x_{q_{par}}) + L \cdot r_{m-1}.
    \end{align*}
    	
    % Equality $n_{m-1}=\frac{1}{r_{m-1}^\beta}$ gives that 
    % \begin{align*}
    %     \Delta_x 
    %     &\le\ell(x_{C_{par}}, n_{m-1})-\ell(x_{C^*_{m-1}}, n_{m-1})+(2L+2)r_{m-1}. 
    % \end{align*}
    It is obvious that $Y_{m-1}^{\max}\geq  f(x_{q^*_{m-1}})$. Moreover, since the cube $C_{par}$ is not eliminated, from the elimination rule we have
    % \begin{align*}
    %     &\wh{\mu}_{m-1}(C^*_{m-1})-\wh{\mu}_{m-1}(C_{par})\\
    %     \le&
    %     \wh{\mu}_{m-1}^{\max}-\wh{\mu}_{m-1}(C_{par})\\
    %     \le& 
    %     4r_{m-1}.
    % \end{align*}
    \begin{align*}
        Y_{m-1}^{\max}-f(x_{q_{par}})\le 2Lr_{m-1}.
    \end{align*}
    Hence, we conclude that $\Delta_x\leq4Lr_{m-1}$.
\end{proof}



\begin{proof}
We let $B$ be the total number of batches of the BLiN run ($B-1$ batches in the for-loop and $1$ clean-up batch), and $N_m$ be the total budget of batch $m$. In the following analysis, we bound $N_m$ for $m=2n-1$ and $m=2n$ separately, and then obtain the simple regret upper bound. \textcolor{red}{For $m$ such that $r_m=r_{m-1}$, we skip batch $m$ and define $N_m=0$. Then the following bounds still hold. Thus, without loss of generality, we assume $r_m<r_{m-1}$.}

Firstly, we consider the case $m=2n-1$. \textcolor{red}{Recall that $r_m=\min\{r_{m-1}, 2^{-a_n}\}$, so $r_m<r_{m-1}$ yields that $r_m=2^{-a_n}$. For convenience, we let $\widetilde{r}_n=2^{-\sum_{i=1}^nc_i}$, and thus we have $\widetilde{r}_{n-1}\geq r_{m-1}\geq r_m\geq \widetilde{r}_{n}$.} Recall that $\mathcal{A}_{m-1}^+$ is set of cubes not eliminated in batch $m-1$, and $\cup_{C\in\mathcal{A}_{m-1}^+}C=\cup_{C^\prime\in\mathcal{A}_m}C^\prime$. Lemma \ref{lem:eli} implies that each cube in $\mathcal{A}_{m-1}^+$ is a subset of $S(4Lr_{m-1})$ %\textcolor{red}{(the covered region in def of zooming number may need to be $S(8Lr)$)}, 
and thus $\left|\mathcal{A}_{m-1}^+\right|\leq N_{r_{m-1}}\leq C_z\cdot r_{m-1}^{-d_z}$. The total budget of batch $m$ is
\begin{align*}
    N_m=|\mathcal{A}_m| = \left(\frac{r_{m-1}}{r_m}\right)^d\left|\mathcal{A}_{m-1}^+\right|
    \leq C_z\cdot\frac{r_{m-1}^{d+1-d_z}\cdot r_m^{-d}}{r_{m-1}} 
    \leq C_z\cdot\frac{\widetilde{r}_{n-1}^{d+1-d_z}\cdot\widetilde{r}_n^{-d}}{r_{m-1}}.
\end{align*}
For the numerator, we have
\begin{align*}
    \widetilde{r}_{n-1}^{d+1-d_z}\cdot\widetilde{r}_n^{-d}=2^{-\left(\sum_{i=1}^{n-1}c_i\right)(d+1-d_z)+\left(\sum_{i=1}^{n}c_i\right)d}=2^{\left(\sum_{i=1}^{n-1}c_i\right)(d_z-1)+c_nd}.
\end{align*}
Define $C_m=\left(\sum_{i=1}^{m-1}c_i\right)(d_z-1)+c_md$. Since $c_m=c_{m-1}\cdot\frac{d+1-d_z}{d}$, calculation shows that $C_m = (\sum_{i=1}^{m-2} c_i) (d_z-1)  + c_{m-1}d+ c_{m-1}(d_z-1-d)+c_md=C_{m-1}$. Thus for any $m$, we have $C_m=C_1=\frac{d_z-1}{d_z}\log T$. Hence,
\begin{equation*}
    N_m\leq C_z\cdot2^{\frac{d_z-1}{d_z}\log T}/r_{m-1}=C_z\cdot T^{\frac{d_z-1}{d_z}}/r_{m-1}.
\end{equation*}

Secondly, we consider the case $m=2n$. Recall that $r_{m-1}=\min\{r_{m-2}, 2^{-a_n}\}$. It is easy to verify that $r_{m-2}<2^{-a_n}$ only happens when $r_{m-2}=r_{m}$, so $r_m<r_{m-2}$ yields that $r_{m-1}=2^{-a_n}$. Lemma \ref{lem:eli} implies that each cube in $\mathcal{A}_m$ is a subset of $S(8Lr_m)$. Similar argument to the first case shows that $N_m\leq C_z\cdot r_m^{-d_z}$.

\textcolor{red}{Line 7 of Algorithm \ref{alg:small-d} ensures that the sum of budgets of full $B$ batches is greater than $T$.} Therefore, combining the above two cases, we have
\begin{align}\label{app-ace1}
    T\leq&\sum_{\substack{m=2n-1, \\ m\leq B }}C_z \cdot\frac{T^{\frac{d_z-1}{d_z}}}{r_{m-1}}+\sum_{\substack{m=2n,\\m\leq B}}C_z\cdot \frac{1}{r_m^{d_z}}.
\end{align}

\textcolor{red}{The rounding step in Definition \ref{def:ace} yields that $r_m\leq\frac{r_{m-1}}{2}$ for any $m$.} If $B$ is odd, from (\ref{app-ace1}) we have 
\begin{equation}\label{app-ace2}
    T\leq2C_z\cdot T^{\frac{d_z-1}{d_z}}\cdot\frac{1}{r_{B-1}}+2C_z\cdot\frac{1}{r_{B-1}^{d_z}}.
\end{equation}

We set $c_r=\max\{(4C_z)^\frac{1}{d_z}, 4C_z\}$, then $\frac{1}{c_r^{d_z}}+\frac{1}{c_r}\leq\frac{1}{2C_z}$. If $r_{B-1}>c_r\cdot T^{-\frac{1}{d_z}}$, then calculation shows that 
\begin{align*}
    2C_z\cdot T^{\frac{d_z-1}{d_z}}\cdot\frac{1}{r_{B-1}}+2C_z\cdot\frac{1}{r_{B-1}^{d_z}}<T,
\end{align*}
which contradicts (\ref{app-ace2}). Therefore, we have $r_{B-1}\leq c_r\cdot T^{-\frac{1}{d_z}}$. Lemma \ref{lem:eli} shows that $\Delta_x\leq4Lr_{B-1}$ for any $x\in\cup_{C\in\mathcal{A}_B}C$, so we have $\Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z}}$, where $c=8L\cdot\max\{c_r, 1\}$. 

If $B$ is even, from (\ref{app-ace1}) we have
\begin{equation*}
    T\leq2C_z\cdot T^{\frac{d_z-1}{d_z}}\cdot\frac{1}{r_{B}}+2C_z\cdot\frac{1}{r_{B}^{d_z}}.
\end{equation*}
Similar arguments yield that $r_B\leq c_r\cdot T^{-\frac{1}{d_z}}$. Lemma \ref{lem:eli} shows that $\Delta_x\leq4Lr_{B-1}$ for any $x\in\cup_{C\in\mathcal{A}_B}C$. \textcolor{red}{Moreover, since $B$ is even, from definition of ACE Sequence we have $r_{B-1}\leq2r_B$.} Consequently, in this case we also have $\Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z}}$.

Finally, we consider the communication bound. For any $B^*$, $\widetilde{r}_{B^*}=2^{-\sum_{i=1}^{B^*}c_i}=2^{-c_1\cdot\frac{1-\eta^{B^*}}{1-\eta}}=T^{-\frac{1}{d_z}}\cdot T^{\frac{\eta^{B^*}}{d_z}}$. Then by choosing $B^*\geq\frac{\log\log T-\log d_z}{\log\frac{d}{d+1-d_z}}$, we have $\frac{\eta^{B^*}}{d_z}\leq \frac{1}{\log T}$ and $\widetilde{r}_{B^*}\leq T^{-\frac{1}{d_z}}$. Definition \ref{def:ace} shows that $r_m<\widetilde{r}_{B^*}$ for any $m\geq2B^*$. As a consequence, no more than $\hat{B}=\frac{2\log\log T}{\log\frac{d}{d+1-d_z}} + 1$ batches are needed to achieve $r_{\hat{B}-1}\leq T^{-\frac{1}{d_z}}$
and 
\begin{equation*}
    \Delta_{\widetilde{x}^*}\leq(4L+4)r_{\hat{B}-1}\leq(4L+4)T^{-\frac{1}{d_z}}\leq c\cdot T^{-\frac{1}{d_z}},
\end{equation*}
where the first inequality follows from Lemma \ref{lem:eli}.
\end{proof}

==> tex/experiment.tex <==
\section{Numerical Experiments}

\subsection{$g_p(x)$}

In this experiment,  we test the performance of BLiN-MOS in optimizing $g_p(x) = 1-\frac{1}{p} \|x\|_{\infty}^p$ with $p = 1.5$ and $p = 5$. At the same time,  we run BLiN as a comparison. In detail,  we set the arm space $\mathcal{X} = [0, 1]^4$ and set the total budget $T = 2^{19}$. As mentioned in Observation \ref{obs:gp} and Proposition \ref{prop:gp},  when $p = 1.5$,  we have $d_z = \frac{4}{3} < d_s = \frac{8}{3}$,  and when $p = 5$,  we have $d_z = \frac{16}{5} > d_s = \frac{4}{5}$. As indicated in figure \ref{},  BLiN-MOS yields smaller simple regret than BLiN when $d_z > ds$ and BLiN performs better than BLiN-MOS when $d_z \leq d_s$.

% When running BLiN-MOS,  choose $k = 1.5$ when $p = 5$ and $k = 0.5$ when $p = 1.5$.

\begin{figure}
    \centering
    \subfloat[Experimental result of $g_p(x)$]{
        \label{fig:gp}
        \includegraphics[width = 0.45\linewidth]{figures/gp_ex.png}
        }
    \caption{}
    \label{}
\end{figure}


\iffalse
\subsection{a variant of the "Drop wave" function}

    In this experiment,  we hope to find the minimum value of the variant of the "Drop wave" function,  which is defined as below:
    $$
    f(x_1, x_2) = - \frac{1 + \cos(6 \sqrt{x_1^2 + x_2^2})}{\frac{1}{2}(x_1^2 + x_2^2) + 2},  x_1 \in [-1, 1],  x_2 \in [-1, 1].
    $$

    After scaling the function to $\mathcal{X} = [0, 1]^2$,  we rewrite this optimization problem as 
    $$
    \max_{[0, 1]^2} f(x) = \frac{1 + \cos(6 \times \|2x - 1\|_2)}{\frac{1}{2} \times \|2x - 1\|_2^2 +2}.
    $$

    As the maximum value is attained at $x = (\frac{1}{2}, \frac{1}{2})$, $q$ must be a cube of edge length $2^{-m}$ and with $(\frac{1}{2}, \frac{1}{2})$ as a corner point. Since $g(y) = \frac{1 + \cos(6 \times y)}{\frac{1}{2} \times y^2 + 2}$ is a decreasing function over $[0, \frac{\pi}{6}]$, if $\sqrt{2}\times 2^{-m} \geq \frac{\pi}{6}$, there exists $x \in q$ such that $1 + \cos(6 \times \|2x - 1\|_2) = 0$, so $f_q^{\min} = 0$; if $\sqrt{2}\times 2^{-m} < \frac{\pi}{6}$, then $f_q^{\min} = \frac{1 + \cos(6\times \sqrt{2} \times 2^{-m})}{2^{-2m} + 2}$.

    We first consider the case when $\sqrt{2}\times 2^{-m} \geq \frac{\pi}{6}$. As $f(x) \geq \frac{1 + 1 - \frac{1}{2}(6 \times \|2x - 1\|_2)^2 }{\frac{1}{2} \times \|2x - 1\|_2^2 +2}$,  we know $\mathbb{P} \left(f(X_q) > 1-\alpha \right) \geq \mathbb{P} \left( \frac{2 - \frac{1}{2}(6 \times \|2x - 1\|_2)^2 }{\frac{1}{2} \times \|2x - 1\|_2^2 +2} > 1-\alpha \right) = \mathbb{P} \left( \|2x - 1\|_2^2 < \frac{2\alpha}{18 + \frac{1}{2}(1-\alpha)} \right) \geq \frac{1}{2^{-2m}} \times \left( \sqrt{\frac{\alpha}{18 + \frac{1}{2}(1-\alpha)}} \right)^2 \geq \frac{4\alpha}{18 + \frac{1}{2}(1-\alpha)} \geq \frac{8}{37} \alpha$. Therefore,  we get $d_s = 1$ and $\kappa_s \geq \frac{8}{37}$.

    We then consider the case when $\sqrt{2}\times 2^{-m} < \frac{\pi}{6}$. Since $m$ is an integer, we have $m \geq 2$. Similarly,  it holds that 
    \begin{equation*}
    \begin{aligned}
    && & \mathbb{P} \left(f(X_q) > 1-\alpha + \alpha \frac{1 + \cos(6\times \sqrt{2} \times 2^{-m})}{2^{-2m} + 2} \right) \\
    && \geq & \mathbb{P} \left( \frac{2 - \frac{1}{2}(6 \times \|2x - 1\|_2)^2 }{\frac{1}{2} \times \|2x - 1\|_2^2 +2} > 1-\alpha + \alpha \frac{1 + \cos(6\times \sqrt{2} \times 2^{-m})}{2^{-2m} + 2} \right) \\
    && = & \mathbb{P} \left( \|2x - 1\|_2^2 < \frac{2\alpha \left( 1 - \frac{1 + \cos(6\times \sqrt{2} \times 2^{-m})}{2^{-2m} + 2} \right)}{18 + \frac{1}{2}\left(1-\alpha + \alpha \frac{1 + \cos(6\times \sqrt{2} \times 2^{-m})}{2^{-2m} + 2} \right)} \right) \\
    && \geq & \frac{1}{2^{-2m}} \times \frac{\alpha \left( \frac{1 + \cos(6 \sqrt{2} \times 2^{-m})}{2^{-2m} + 2} \right)}{18 + \frac{1}{2}(1-\alpha)} > 16\times \frac{ \frac{1 + \cos(\frac{3}{2}\sqrt{2})}{\frac{1}{16}+2}}{18 + \frac{1}{2}} \alpha.
    \end{aligned}
    \end{equation*}
    Consequently, $d_s = 1$ and $\kappa_s \geq \frac{32\times 16}{37 \times 33} \times (1+\cos (\frac{3}{2}\sqrt{2})) $.

    Combining the two cases above, we choose $d_s = 1$ and $\kappa_s = \frac{8}{37}$.
\fi



\iffalse
\subsection{Functions}


% \begin{proposition}
%     \label{prop:gp}
%     For $g_p(x) = 1-\frac{1}{p} \|x\|_{\infty}^p,  x \in [0, 1]^d$,  the scattering dimension $d_s = \frac{d}{p}$ and the scattering constant $\kappa_s = 1$.
% \end{proposition}

% \begin{proof}
%     Suppose $q = [0, r]^d$,  then $f^{\max}_q = 1 , f^{\min}_q = 1 - \frac{1}{p} r^p$,  $(1-\alpha)f^{\max}_q +\alpha f^{\min}_q = 1 - \frac{1}{p} r^p \alpha$.

%     \begin{equation*}
%         \begin{aligned}
%         && \mathbb{P} \left(f(x_q) \geq (1-\alpha)f^{\max}_q +\alpha f^{\min}_q \right) & = \mathbb{P} \left( \|x\|_{\infty}^p \leq r^p \alpha \right) \\
%         && & = \prod_{j=1}^d \mathbb{P} \left(|x_j| \leq r \alpha^{\frac{1}{p}}  \right) \\
%         && & =\alpha^{\frac{d}{p}}
%         \end{aligned}
%     \end{equation*}
% \end{proof}

\begin{lemma}
    \label{lem:func-1}
    For $f(x) = -|x-a|^{p},  \enspace p > 0,  \enspace x, a \in [0, 1]$,  the scattering dimension $d_s = \frac{1}{p}$ and the scattering constant $\kappa_s = 1$.
\end{lemma}

\begin{proof}
    Suppose $q = [l_1, l_2]$ and $a \in q$. We only prove the case when $\frac{l_1+l_2}{2} \geq a$ and the proof of the other circumstance is similar. When $\frac{l_1+l_2}{2} \geq a$,  we have $f^{\max}_q = 0$,  $f^{\min}_q = f(l_2) = -(l_2 - a)^p$.
    \begin{equation*}
        \begin{aligned}
            && \mathbb{P} \left(f(x_q) \geq (1-\alpha)f^{\max}_q +\alpha f^{\min}_q \right) & = \mathbb{P} \left( |x-a| \leq (l_2-a) \alpha^{\frac{1}{p}} \right) \\
            && & = \left\{
            \begin{aligned}
                && & \frac{ 2(l_2 - a)\alpha^{\frac{1}{p}}}{l_2 - l_1},  \enspace \text{ if } l_1 \leq a - (l_2 - a)\alpha^{\frac{1}{p}} \\
                && & \frac{a + (l_2 - a)\alpha^{\frac{1}{p}} - l_1}{l_2 - l_1},  \enspace \text{ if } l_1 > a - (l_2 - a)\alpha^{\frac{1}{p}}
            \end{aligned}
            \right.
        \end{aligned}
    \end{equation*}
    When $l_1 \leq a - (l_2 - a)\alpha^{\frac{1}{p}}$,  since $l_2 - l_1 = l_2 - a + a - l_1 \leq 2(l_2 - a)$,  we know $\frac{ 2(l_2 - a)\alpha^{\frac{1}{p}}}{l_2 - l_1} \geq \alpha^{\frac{1}{p}}$. When $l_1 > a - (l_2 - a)\alpha^{\frac{1}{p}}$,  $\alpha > \left(\frac{a-l_1}{l_2-a}\right)^p$. Denote $g(\alpha) = \frac{a + (l_2 - a)\alpha^{\frac{1}{p}} - l_1}{(l_2 - l_1)\alpha^{\frac{1}{p}}}$. From the fact that $g'(\alpha) = \frac{l_1-a}{p(l_2-l_1)\alpha^{\frac{1}{p}+1}} < 0$,  we get $g(\alpha) \geq g(1) = 1$. Therefore,  $\frac{a + (l_2 - a)\alpha^{\frac{1}{p}} - l_1}{l_2 - l_1} \geq \alpha^{\frac{1}{p}}$. We thus conclude that for $f(x)$,  $d_s = \frac{1}{p}$ and $\kappa_s = 1$.
\end{proof}



\begin{lemma}
    \label{lem:func_d}
    For $f(x) = -\|x - a\|_2^2,  \enspace x, a \in [0, 1]^d$,  it holds that $d_s = \frac{d}{2}$,  $\kappa_s = 1$.
\end{lemma}


\begin{proof}
    Suppose $q = \prod_{j=1}^d [l_{1j}, l_{2j}]$. $f(x) = - \| x - a \|_2^2 = - \sum_{j=1}^d |x_j - a_j|^2 $,  where $x_j$ and $a_j$ are the $j$-th dimensional component of $x$ and $a$ respectively.  Denote $q_j = [l_{1j},  l_{2j}]$ and $ f_j(x_j) = -|x_j - a_j|^2 $. By the definition of scattering dimension and scattering constant,  we only have to consider the case when $a_j \in q_j, \enspace j=1, 2, \cdots, d$. It is obvious that $ f^{\max}_q = \sum_{j=1}^d f_{j, q_j}^{\max},  f^{\min}_q = \sum_{j=1}^d f_{j, q_j}^{\min}$. Therefore,  we can rewrite $ \mathbb{P} \{ f(X_q) \geq f^{\max}_q - \alpha (f^{\max}_q - f^{\min}_q) \} $ as
    \begin{equation*}
        \begin{aligned}
        && \mathbb{P} \{ f(X_q) \geq f^{\max}_q - \alpha (f^{\max}_q - f^{\min}_q) \} & = \mathbb{P} \{ \sum_{j=1}^d f_j(X_{j, q_j}) \geq (1-\alpha) \sum_{j=1}^d f^{\max}_{j, q_j} + \alpha \sum_{j=1}^d f^{\min}_{j, q_j} \} \\
        && & \geq \prod_{j=1}^{d} \mathbb{P} \{ f_j(X_{j, q_j}) \geq (1-\alpha)f^{\max}_{j, q_j} + \alpha f^{\min}_{j, q_j} \} 
        \end{aligned}
    \end{equation*}
    By Lemma \ref{lem:func-1},  we know $\mathbb{P} \{ f_j(X_{j, q_j}) \geq (1-\alpha) f^{\max}_{j, q_j} + \alpha f^{\min}_{j, q_j} \} \geq \alpha^{\frac{1}{2}}$ holds for all $\alpha \in (0, 1)$ and for all $q_j$ with $a_j \in q_j \subseteq[0, 1]$. Therefore,  it holds that
    \begin{equation*}
        \mathbb{P} \{ f(X_q) \geq (1-\alpha) f^{\max}_q + \alpha f^{\min}_q \} \geq \alpha^{\frac{d}{2}},  \enspace \forall \alpha \in (0, 1), \enspace \forall q = \prod_{j=1}^d [l_{1j}, l_{2j}] \subseteq [0, 1]^d \text{ with } a\in q.
    \end{equation*}
\end{proof}




\begin{corollary}
    \label{cor:func_example}
    For the nonsmooth Lipschitz function $f(x) = \max \{ - \|x - (\frac{1}{5}, \frac{3}{10} ) \|_2 ^2,  - \| x - (\frac{7}{8},  \frac{3}{10} ) \|_2 ^2 \},  x \in [0, 1]^2$,  $\kappa_s = \frac{1}{2}$ and $d_s = 1$.
\end{corollary}

\begin{proof}

    $f(x) = - (\|x - (\frac{1}{5}, \frac{3}{10} ) \|_2 ^2 ) \mathbb{I}_{ \{ x_1 \leq \frac{43}{80} \} } - (\| x - (\frac{7}{8},  \frac{3}{10} ) \|_2 ^2) \mathbb{I}_{ \{ x_1 > \frac{43}{80} \} } $. Suppose $x^* \in q \subseteq [0, 1]^2$,  where $\arg\max_{[0, 1]^2}f(x)$ is denoted as $x^*$.

    If $q$ falls exactly within $[0, \frac{43}{80}] \times [0, 1]$ or within $[\frac{43}{80}, 1] \times [0, 1]$,  then by Lemma \ref{lem:func_2d},  we can draw the conclusion. 
    
    If the line $x_1 = \frac{43}{80}$ crosses $q$,  then $f^{\min}_q$ is reached on $x_1 = \frac{43}{80}$ and $f^{\max}_q$ is reached in the left region or the right region of $x_1 = \frac{43}{80}$. Suppose $q = [l_{11}, l_{21}] \times [l_{12}, l_{22}]$ and $f^{\max}_q$ is reached in the left region. Then $\frac{43}{80} - l_{11} \geq \frac{1}{2} (l_{21} - l_{11} )$. By Lemma \ref{lem:func_2d},  over $q' = [l_{11},  \frac{43}{80}] \times [l_{12}, l_{22}]$,  it holds that $\mathbb{P} \{ f(X_{q'}) \geq (1-\alpha) f^{\max}_{q'} + \alpha f^{\min}_{q'} \} \geq \alpha$. Since $\mathbb{P} \{ f(X_{q}) \geq (1-\alpha) f^{\max}_{q} + \alpha f^{\min}_{q} \} = \mathbb{P} \{ f(X_{q}) \geq (1-\alpha) f^{\max}_{q'} + \alpha f^{\min}_{q'} \}$,  we know 
    $$\mathbb{P} \{ f(X_{q}) \geq (1-\alpha) f^{\max}_{q} + \alpha f^{\min}_{q} \} \geq  \frac{\frac{43}{80} - l_{11} }{l_{21} - l_{11}} \mathbb{P} \{ f(X_{q'}) \geq (1-\alpha) f^{\max}_{q'} + \alpha f^{\min}_{q'} \} \geq \frac{1}{2} \alpha.
    $$ 
    This implies that for $f(x)$,  we have $\kappa_s = \frac{1}{2}$ and $d_s = 1$.

\end{proof}
\fi












\iffalse
\noindent Consider the case when $d = 1$. Let $f(x)$ be a real-valued Lipschitz piecewise linear function who has finite breakpoints over $q$. Set the slope of each segment of $f(x)$ as $k_1, k_2, \cdots, k_n$. Assume $k_i \neq 0,  i = 1, 2, \cdots, n$,  so that the density function of $f(X|_q)$ exists (cannot contain fragments of Dirac $\delta$ functions). Denote the set of this kind of functions as $\mathcal{F}$.


\begin{theorem}
    $\forall f(x) \in \mathcal{F},  f(x)$ satisfies Assumption \ref{assumption}.
\end{theorem}


\begin{proof}
\noindent Denote 
\begin{equation*}
\begin{aligned}
    K_1 := \{k_i|k_i > 0,  i = 1, 2, \cdots, n\},  \enspace N_1 := \#K_1\\
    K_2 := \{k_i|k_i < 0,  i = 1, 2, \cdots, n\}, \enspace N_2 := \#K_2
\end{aligned}
\end{equation*}

\begin{claim}
\label{claim1}
Let $\nu = \min_{1\leq s \leq N_1, 1\leq t \leq N_2} \{\frac{1}{k_s},  -\frac{1}{k_t} | k_s\in K_1,  k_t\in K_2\}$. Then it holds that 
\begin{equation*}
    p_{f(X|_q)} \geq \nu D(q)^{-1}
\end{equation*}
\end{claim}

\begin{proof}
 In fact,  the density function of $f(X|_q)$ is a staircase function,  and the values of each segment have forms like $\sum_{s=1}^{n_1}\frac{1}{k_sD(q)} - \sum_{t=1}^{n_2}\frac{1}{k_tD(q)}$,  where $n_1 \leq N_1,  n_2 \leq N_2,  k_s \in K_1,  k_t \in K_2$. Therefore,  the lower bound of $p_{f(X|_q)}$ is greater than $\min_{1\leq s \leq N_1, 1\leq t \leq N_2} \{\frac{1}{k_sD(q)},  -\frac{1}{k_tD(q)} | k_s\in K_1,  k_t\in K_2\} = \nu D(q)^{-1}$.
 \end{proof}
 

\begin{claim}
Let $\mu = \sum_{p=1}^{N_1}\frac{1}{k_s} -\sum_{q=1}^{N_2}\frac{1}{k_t}$,  where $k_s \in K_1,  k_t \in K_2$. Let $\kappa_- = \frac{\nu}{2\mu^2}$. Then it holds that 
 \begin{equation*}
 \kappa_-(1-\alpha)D(q) \leq f^*_q - CVaR_{\alpha}(f(X|_q))
 \end{equation*}
\end{claim}
 
\begin{proof}
 We know from the proof of \ref{claim1} that $p_{f(X|_q)}\leq \mu D(q)^{-1}$. Following this,  we have
 \begin{equation*}
     \int_{VaR_{\alpha}(f(X|_q))}^{f^*_q} p_{f(X|_q)}(y) \, dy \leq \mu D(q)^{-1}(f^*_q - VaR_{\alpha}(f(X|_q)))
 \end{equation*}
 The left side is equal to $ F_{f(X|_q)}(f^*_q) - F_{f(X|_q)}\left(VaR_{\alpha}(f(X|_q))\right)  = 1-\alpha$,  where $F_{f(X|_q)}$ is the cumulative distribution function of $f(X|_q)$. Consequently,  it holds that
 \begin{equation*}
    f^*_q - VaR_{\alpha}(f(X|_q)) \geq \frac{1}{\mu}(1-\alpha)D(q)
 \end{equation*}
In addition,  starting from the definition of $CVaR_{\alpha}(f(X|_q))$,  we have
\begin{equation*}
\begin{aligned}
    && CVaR_{\alpha}(f(X|_q)) &= \frac{1}{1-\alpha}\int_{\alpha}^1 VaR_{\gamma}(f(X|_q)) \, d\gamma \\
    && & =\frac{1}{1-\alpha}\left((1-\alpha)f^*_q-\int_{-\infty}^{f^*_q}[F_{f(X|_q)}(y)-\alpha]_+\right) \, dy \\
    && & =f^*_q - \frac{1}{1-\alpha}\int_{VaR_{\alpha}(f(X|_q))}^{f^*_q}(F_{f(X|_q)}(y)-\alpha) \, dy
\end{aligned}
\end{equation*}
Then, 
\begin{equation*}
    \begin{aligned}
        && f^*_q - CVaR_{\alpha}(f(X|_q)) & =\frac{1}{1-\alpha}\int_{VaR_{\alpha}(f(X|_q))}^{f^*_q}(F_{f(X|_q)}(y)-\alpha) \, dy \\
        && & \geq \frac{1}{1-\alpha}\int_{VaR_{\alpha}(f(X|_q))}^{f^*_q}\nu D(q)^{-1}\left(y-VaR_{\alpha}(f(X|_q))\right) \, dy \\
        && & = \frac{\nu}{2(1-\alpha)D(q)}\left(f^*_q-VaR_{\alpha}(f(X|_q))\right)^2 \\
        && & \geq \frac{\nu}{2(1-\alpha)D(q)} \cdot \frac{1}{\mu^2}(1-\alpha)^2D(q)^2 \\
        && & = \frac{\nu}{2\mu^2}(1-\alpha)D(q) = \kappa_-(1-\alpha)D(q)
    \end{aligned}
\end{equation*}
The first inequality holds because $p_{f(X|_q)} \geq \nu D(q)^{-1}$.
\end{proof}


\begin{claim}
Let $\kappa_+ = \frac{\mu}{2\nu^2}$. Then it holds that 
\begin{equation*}
f^*_q-CVaR_{\alpha}(f(X|_q)) \leq \kappa_+(1-\alpha)D(q)
\end{equation*}
\end{claim}

\begin{proof}
Since $p_{f(X|_q)} \geq \nu D(q)^{-1}$,  it holds that
\begin{equation*}
\begin{aligned}
    && \int_{VaR_{\alpha}(f(X|_q))}^{f^*_q} p_{f(X|q)}(y) \, dy &\geq \nu D(q)^{-1}(f^*_q-VaR_{\alpha}(f(X|_q))) \\
    && f^*_q-VaR_{\alpha}(f(X|_q)) &\leq \frac{1}{\nu}(1-\alpha)D(q)
\end{aligned}
\end{equation*}
Therefore, 
\begin{equation*}
\begin{aligned}
    && f^*_q - CVaR_{\alpha}(f(X|_q)) & =\frac{1}{1-\alpha}\int_{VaR_{\alpha}(f(X|_q))}^{f^*_q}(F_{f(X|_q)}(y)-\alpha) \, dy \\
    && & \leq \frac{1}{1-\alpha}\int_{VaR_{\alpha}(f(X|_q))}^{f^*_q}\mu D(q)^{-1}\left(y-VaR_{\alpha}(f(X|_q))\right) \, dy \\
    && & = \frac{\mu}{2(1-\alpha)D(q)}\left(f^*_q-VaR_{\alpha}(f(X|_q))\right)^2 \\
    && & \leq \frac{\mu}{2(1-\alpha)D(q)}\cdot \frac{1}{\nu^2}(1-\alpha)^2D(q)^2 \\
    && & = \frac{\mu}{2\nu^2}(1-\alpha)D(q) = \kappa_+(1-\alpha)D(q)
\end{aligned}
\end{equation*}
\end{proof}

Therefore,  $f(x) \in \mathcal{F}$ satisfies Assumption \ref{assumption}.

\end{proof}
\fi


==> tex/intro.tex <==

\section{Introduction}

% Random Search \citep{bergstra2012random} is one of the most widely-used method for HyperParameter Optimization (HPO). 

Optimizing nonsmooth nonconvex functions is one of the most important tasks in modern machine learning and related fields. 
Nonsmooth nonconvex optimization seeks to solve 
\begin{align*} 
    \min_{x \in S } f (x) , 
\end{align*} 
where $S$ is the feasible set, and $f$ is the nonsmooth nonconvex objective function. In addition, only zeroth-order information is available to the solver. These problems are usually difficult. Previously, various approaches have been developed to solve such problems, including bandit-based algorithms \citep[e.g.,][]{} and other types of methods \citep[e.g.,][]{}. In this paper, we use the principles of Lipschitz bandit algorithms to solve such optimization problems. 

% While classic theory of Lipschitz bandits has been well-established \citep{},  

% While 

% Among numerous methods for zeroth-order optimization, bandit-based methods form a prosperous cluster \citep{}. While 


\subsection{The Limitation of Classic Theory} 

The study of Lipschitz bandits dates back to at least \citep{agrawal1995continuum}, and a seminal milestone was reached when the concept of zooming dimension was introduced \citep{kleinberg2008multi,bubeck2008tree}; See the related works section for more details. Zooming dimension describes the function landscape by specifying how many balls are needed to cover/pack a near-optimal region of the function (See Section \ref{sec:zooming} for more details). Roughly speaking, functions of large zooming dimension have large near-optimal regions. Functions with large zooming dimension has two contrasting features: 1. The difference between near-optimal points is hard to distinguish \textbf{(N)}; 2. The near-optimal region is large \textbf{(P)}. The classic theory captures only the \textbf{(N)} side of the story: When the zooming dimension is large, the function values vary slowly and learning which point is \emph{exactly} optimal is difficult. In the language of Lipschitz bandits, the regret rate deteriorates as the zooming dimension increases. However, the \textbf{(P)} side of the story is missing: when the zooming dimension is large, the near-optimal is large. Further, when the near-optimal region is large, finding an \emph{approximately} optimal point is easy. 

% \textcolor{red}{(maybe use a table to summarize it)} 
% We summarize this dilemma in Table \ref{tab:}. 
% To better describe the function landscape, we introduce the concept of scattering dimension. 


\subsection{The Scattering Dimension and Our Results} 

To better describe the function landscape, we introduce the concept of \emph{scattering dimension}. 
While zooming dimension specifies how many balls are needed to cover/pack a near-optimal region, scattering dimension specifies how likely a random point in the domain hits a near-optimal region. Unlike the zooming dimension, the scattering dimension captures the \textbf{(P)} side of the function landscape. When the scattering dimension is small, a random point in the domain has a better chance to hit a near-optimal region. 

With the concept of scattering dimension, we study two algorithms, Batched Lipschitz Narrowing (BLiN) and Batched Lipschitz Narrowing with Maximum Order Statistics (BLiN-MOS), and their performance on zeroth-order nonsmooth nonconvex optimization. The algorithmic procedure of both BLiN and BLiN-MOS rely on the recent advances in Lipschitz bandits with batched feedback \citep{fenglipschitz}. Both BLiN and BLiN-MOS successively eliminate regions of non-optimal function values, adaptive to the function landscape. The performance of BLiN and BLiN-MOS are specified by zooming dimension and scattering dimension. 
% so that the domain is 
% the algorithms adaptive narrow the domain, and focus on regions of  to the function landscape. 
In particular, we show that for zeroth-order nonsmooth nonconvex optimization tasks with total time horizon $T$, the final optimality gap of BLiN is bounded by $ O (T^{-\frac{1}{d_z}}) $, where $d_z > 0$ is the zooming dimension. Also, the final optimality gap of BLiN-MOS is asymptotically bounded by $ O \( \( \frac{T}{\log T } \)^{-\frac{1}{d_s}} \) $ with high probability, where $d_z > 0$ is the zooming dimension. The cases where $d_z= 0$ or $d_s = 0$ are also considered. When $ d_z > d_s $, BLiN-MOS ourperforms BLiN, and vice versa. In addition, both BLiN and BLiN-MOS needs only $O (\log \log T)$ rounds of communications to achieve this bound. 

% \textcolor{red}{(Comment on communication complexity.)}

% we show that with proper partitioning of the space, only $ O (\log \log T) $ rounds of communication are  


\section{Related Works} 

Nonsmooth nonconvex optimization is a rich field that has attracted the attention of numerous researchers from various different angles. 
To name a few, simulated annealing \citep{} and Langevin dynamics based methods \citep{} escape local minima by a Gaussian perturbation in the dynamics, and have been extensively studied recently in machine learning, following the success of saddle-escaping effect of perturbed gradient descent \citep{}. Subgradient-based methods handles nonsmoothness in the objective, and have been analysed in many different setting, ranging from XXX \citep{} to YYY \citep{}. 
While these methods handles nonconvexity or nonsmoothness in the objective, they require first-order information to implement. 
% Zeroth order optimization. 

Bayesian optimization methods also form a large body of literature; See \citep{7352306} for an exposition. Different acquisition functions give rise to different Bayesian optimization schemes, including Gaussian Process Expected Improvement (GP-EI) \citep{10.1287/opre.9.2.145,jones1998efficient,pmlr-v151-tran-the22a}, Gaussian Process Upper Confidence Bound (GP-UCB) \citep{10.5555/3104322.3104451}, Gaussian Process Mutual Information (GP-MI) \citep{contal2014gaussian}, just to name a few. Bayesian optimization typically only rely on zeroth-order information and handles nonconvexity. However, Bayesian optimization methods impplicitly impose smoothness assumptions on the underlying objective. In particular, functions sampled from Gaussian processes with Gaussian kernel are infinitely differentiable. 
% Functions sampled from 
Therefore, such methods are not suitable for handling nonsmoothness in the domain. 
% Existing works simulated 


Perhaps the most related line of research is Lipschitz bandit algorithms \citep{agrawal1995continuum,kleinberg2005nearly,kleinberg2008multi,bubeck2008tree,bubeck2011x,fenglipschitz}. 




==> tex/mos.tex <==



\section{The BLiN-MOS Algorithm} 

\label{sec:mos} 

% \subsection{The Try-And-Eliminate Procedure} 

% As suggested by its name, the Batched Lipschitz Narrowing algorithms progressively narrow the search space. Such algorithms are executed in batches. In each batch, the algorithm performs guided trials, and eliminate regions of low payoffs. After each iteration, the problem space becomes narrower, and the algorithm repeats this try-and-eliminate procedure until a pre-determined terminating condition is met. In Figure \ref{}, an example run of batched narrowing is provided. Two algorithms of this kind are formally summarized in Algorithms \ref{alg:small-d} and \ref{alg:large-d}. 

The Batched Lipschitz Narrowing (BLiN) algorithm, as the name implies, progressively narrow the search space. Such algorithms operate in batches, where they perform guided trials and eliminate low-payoff regions. After each batch, the problem space shrinks, and the algorithm repeats this try-and-eliminate process until a pre-determined termination condition is met. 
% Figure \ref{} shows an example run of batched narrowing. 
We formally present two algorithms of this type --- Batched Lipschitz Narrowing (BLiN) and  Batched Lipschitz Narrowing with Maximum Ordered Statistics (BLiN-MOS). 

% \textcolor{red}{(need to specify $M$ in the algorithms.)} 



\begin{algorithm}[ht] 
	\caption{Batched Lipschitz Narrowing with Max Order Statistics (BLiN-MOS)} 
	\label{alg:large-d} 
	\begin{algorithmic}[1]  
		\STATE \textbf{Input.} Arm set $\A=[0,1]^d$; time horizon $T$. 
		\STATE \textbf{Initialization} Number of batches $M$; Edge-length sequence $\{r_m\}_{m=1}^{M+1}$; The first grid point $t_0=0$; Equally partition $\mathcal{A}$ to $r_1^d$ subcubes and define $\mathcal{A}_{1}$ as the collection of these subcubes. 
		% \STATE Compute $n_m=\frac{16\log T}{r_m^2}$ for $m=1,\cdots,B+1$. 
		\FOR{$m=1,2,\cdots,M$} 
                \STATE Compute $\alpha_m = r_m^k$, $\rho_m = L \alpha_m r_m$, and $ n_m^s = \frac{\log \epsilon }{ \log \(1 - \frac{\kappa_m \kappa_s}{d_s+1} \alpha_m^{d_s+1} \) }$, where $ \kappa_m $ lower bounds the density of the noise. 
                % $k > 0 $. 
                \STATE Compute $n_m^z=\frac{\log (1 / \epsilon) }{L^2 r_m^2}$ \textcolor{red}{ (need to check) } for $m=1,\cdots,M+1$. 
                \IF{$n_m^z \le n_m^s$}
                    \STATE For each cube $q\in\mathcal{A}_m$, play arms $x_{q,1},\cdots x_{q,n_m^z}$ from $q$ uniformly at random. 
                    \STATE Collect the rewards of all pulls up to $t_m$. Compute the average payoff $\wh{\mu}_m(q)=\frac{\sum_{i=1}^{n_m^z}y_{q,i} }{n_m}$ for each cube $q\in\mathcal{A}_m$, and let  $\wh{\mu}_m^{\max}=\max_{q\in\mathcal{A}_m}\wh{\mu}(q)$. /* $y_{q,i}$ is the noisy payoff associated with $x_{q,i}$. */ 
                    \STATE 
                    Let $\mathcal{A}_m' = \{ q \in \mathcal{A}_m: \wh{\mu}_m^{\max}- \wh{\mu}_m(q) \le 4 L r_m \}$. 
                    \STATE For each cube $ q \in \mathcal{A}_m'$, uniformly randomly play arms $ x_{q,n_m^z+1}, \cdots x_{q,n_m^s}$ from $q$. 
                    \STATE Compute $ Y_{q,n_m^s} = \max \{ y_{q,1} , y_{q,2} , \cdots, y_{q,n_m^s} \} $ and $ Y_m^{\max} := \max_{q \in \mathcal{A}_m } Y_{q,n_m^s} $. 
                    \STATE Let $\mathcal{A}_{m}'' = \{ q \in \mathcal{A}_m' : {Y}_m^{\max} - {Y}_{q,n_m^s} \le \rho_m \}$. 
                \ELSE 
                    \STATE For each cube $q\in\mathcal{A}_m$, play arms $x_{q,1},\cdots x_{q,n_m^s }$ from $q$. Denote the associated noisy payoff by $y_{q,1} , y_{q,2} , \cdots, y_{q,n_m^s} $. 
                    \STATE Compute $ Y_{q,n_m^s} = \max \{ y_{q,1} , y_{q,2} , \cdots, y_{q,n_m^s} \} $ and $ Y_m^{\max} := \max_{q \in \mathcal{A}_m } Y_{q,n_m^s} $. 
                    \STATE Let $\mathcal{A}_{m}' = \{ q \in \mathcal{A}_m : {Y}_m^{\max} - {Y}_{q,n_m^s} \le \rho_m \}$. 
                    \STATE For each cube $ q \in \mathcal{A}_m'$, uniformly randomly play arms $ x_{q,n_m^s+1}, \cdots x_{q,n_m^z}$ from $q$. 
                    \STATE Compute the average payoff $\wh{\mu}_m(q)=\frac{\sum_{i=1}^{n_m^z}y_{q,i} }{n_m}$ for each cube $q\in\mathcal{A}_m'$, and let  $\wh{\mu}_m^{\max}=\max_{z\in\mathcal{A}_m}\wh{\mu}(z)$. 
                    \STATE Let $\mathcal{A}_{m}'' = \{ q \in \mathcal{A}_m' : \wh{\mu}_m^{\max} - \wh{\mu}_{m} (q) \le 4 L r_m \}$. 
                \ENDIF 
                \STATE Compute $t_{m+1}=t_m+2(r_{m}/r_{m+1})^d\cdot|\mathcal{A}_{m }'' | $. 
                \IF{$t_{m+1}\geq T$}
                    \STATE Let $M^* = m$. \textbf{Terminate} the algorithm and \textbf{output} $ Y_{M^*}^{\max} $.  /* The last line of the algorithm is not executed if we enter this if condition */
                \ENDIF 
                \STATE Dyadically partition the cubes in $\mathcal{A}_{m }'' $, and collect these cubes to form $ \mathcal{A}_{m+ 1 } $. 
                    % = \{ I: \in  \mathcal{A}_{m+\frac{1}{2}} : \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m } \le \rho_m \} $
                % \ENDFOR 
		\ENDFOR 
        \STATE Let $M^* = M$ and \textbf{output:} $ Y_{M^*}^{\max} $. 
        % \STATE \textbf{Output:} $ Y_{M}^{\max} $. 
	\end{algorithmic} 
\end{algorithm} 

----------------------------------------------------

Consider the case with $k = 1$ and $r_m = 2^{-m}$. 


\begin{lemma} 
    \label{lem:event}
    Let $ W $ be an $iid$ zero-mean noise upper bounded by $1$. Let $\kappa_m$ lower bound the noise density. 
    Denote $ \rho_m = L \alpha_m r_m$. Let $n_m$ be defined as in Algorithm \ref{alg:large-d}. Let 
    \begin{align*} 
        \mathcal{E} := & \left\{ f_q^{\max} + 1 - Y_{q,n_m} \le \rho_m \text{ and } |\wh{\mu}_m (q) - f (x) | \le 2 L r_m, \; \forall x \in q \; \right. \\
        & \left. \forall m = 1,2,\cdots, M,\; \text{ and } \;  \forall q \in \mathcal{A}_m \text{ such that } x^* \in q \right\} , 
    \end{align*} 
    and let $\epsilon = \frac{1}{T^2}$. 
    Then $\Pr \( \mathcal{E}\) \ge 1 - \frac{1}{T}$. 
\end{lemma} 


\begin{proof} 
    Let $ \mu_q := \E_{x\sim \mathrm{Unif} (q)} \[ f (q) + W \]  $. 
    By Hoeffding's inequality and Lipschitzness of the function, we know that, with probability larger than $ 1 - \frac{1}{T^2} $, 
    \begin{align*} 
        | \wh{\mu}_m(q) - f (x) |
        \le 
        | \wh{\mu}_m(q) - \mu_q | + | \mu_q - f (x) | 
        \le 
        \sqrt{ \frac{ 2 \log T}{n_m^z} } + L r_m 
        \le 
        2 L r_m . 
    \end{align*} 
    In addition, using an argument similar to that leading to (\ref{}), we have 
    \begin{align*} 
        \Pr \( \frac{ f^* - f ( X ) }{ L \Theta } + Z > \beta \) 
        \le 
        1 - \frac{ \kappa_s \kappa_m }{ d_s + 1 } \beta^{d_s + 1} 
    \end{align*} 
\end{proof} 

----------------------------------------------------

% the problem space is narrower than the previous batch, and . 

% As demonstrated in Figure \ref{??}, s
Such procedures focus more resources on regions of promising function values. Both BLiN and BLiN-MOS are landscape-aware. Thus their convergence rates depend on $d_z$ and $d_s$. To fully unleash the power of BLiN and BLiN-MOS, we need to carefully choose the edge-length sequence $\{ r_m \}_{m=1}^{M+1}$. 
An immediate choice of $ \{ r_m \}_{m=1}^M $ is letting $ r_m = 2^{-m} $. This choice of the edge-length sequence leads to $O (\log T)$ rounds of communications. With a more careful choice of $ \{ r_m \}_{m=1}^M $, we can achieve a better communication complexity. This edge-length sequence is defined below in Definition \ref{def:ace}. 

\begin{definition} 
    \label{def:ace} 
    Denote $c_1 = \frac{d_z-1+k d_s }{(d+k d_s )(d_z+k d_s )}\log \frac{T}{\log T}$, $ c_{i+1} = \eta c_i,i\geq 1$, where $\eta = \frac{d+1-d_z}{d+k d_s }$. Let $a_n = \lfloor \sum_{i=1}^n c_i\rfloor$, $b_n = \lceil \sum_{i=1}^n c_i\rceil$. Define sequence $\{r_m\}_m $ as $r_m = \min \{ r_{m-1}, 2^{-a_n} \}$ for $m = 2n-1$ and $r_m = 2^{-b_n}$ for $m = 2n$.
    % (Here we suppose $\{r_m\}$ is a strictly decreasing sequence, see Remark \ref{rm:batch} for details). 
    Define sequence $\{\alpha_m\}_m$ as $\alpha_m = r_m^k,k>0$. 
\end{definition} 

% We start with some pro 

With the edge-length sequence defined above, we can state the main convergence results. 
% In particular, we need to pick $ \{ r_m \}_{m=1}^{M+1} $ so that 
The convergence rates depend on zooming dimension $d_z$ and scattering dimension $d_s$, as stated in Theorem \ref{thm:small-d}, Theorem \ref{thm:large-d} and Corollary \ref{cor1}. 

% To 

% This dependence on $d_s$ and $d_z$ means that BLiN and BLiN-MOS are landscape-aware, and adaptively narrows the domain. 


% in the following Theorems and Corollaries. 
% Theorems \ref{thm:small-d} and \ref{thm:large-d}. 

\begin{theorem}
% [\textcolor{red}{a theorem for algorithm \ref{alg:small-d} }]
    \label{thm:small-d}
    % \label{thm:ace}
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:small-d}. 
    Output arm $\widetilde{x}^*$ of BLiN algorithm with total time horizon $T$ and ACE Sequence $\{r_m\}$ satisfies 
    \begin{equation*} 
        \Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z}},
    \end{equation*}
    where $d_z$ is the zooming dimension and $c$ is a constant. In addition, BLiN needs $\mathcal{O}(\log\log T)$ batches to achieve this optimality gap. 
    % regret.
    % When $d_z = 0$, XXXXX 

    % When $d_z > 0$, XXXXX 
    
\end{theorem} 

% ----------------------------------------------------

% \begin{definition}
%     \label{def:opt-batch}
%     Denote $c_1 = \frac{d_z-1+k d_s }{(d+k d_s )(d_z+k d_s )}\log \frac{T}{\log T}$, $ c_{i+1} = \eta c_i,i\geq 1$, where $\eta = \frac{d+1-d_z}{d+k d_s }$. Let $a_n = \lfloor \sum_{i=1}^n c_i\rfloor$, $b_n = \lceil \sum_{i=1}^n c_i\rceil$. Define sequence $\{r_m\}$ as $r_m = 2^{-a_n}$ for $m = 2n-1$ and $r_m = 2^{-b_n}$ for $m = 2n$ (Here we suppose $\{r_m\}$ is a strictly decreasing sequence, see Remark \ref{rm:batch} for details). Define sequence $\{\alpha_m\}$ as $\alpha_m = r_m^k,k>0$.
% \end{definition}

\begin{theorem} 
    \label{thm:opt-batch} 
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:large-d}. 
    Let $T$ be the total time horizon such that $ (d+1-d_z) \log \frac{T}{\log T} - d d_z > 0 $ and let $\epsilon = \frac{1}{T^2}$. Let $ k \in \( 0, \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} \] $. Let $M \ge 2\times \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} +1$. Apply the sequence $\{r_m\}_{m=1}^{M}$ in Definition \ref{def:ace} to Algorithm \ref{alg:large-d}. 
    % With fixed budget $T$, 
    % the final simple regret satisfies 
    Then with probability exceeding $1 - \frac{1}{T}$, the final optimality gap satisfies  
    \begin{equation*} 
        f^*_q - Y^{\max}_{M^*} \leq cL\left(\frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }},
    \end{equation*} 
    where $Y^{\max}_{M^*}$ is the output of Algorithm \ref{alg:large-d} and $c$ is a constant independent of $T$. 
    % In addition, 
    % Moreover, only $2\times \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} +1$ total batches are needed to achieve this optimality gap. 
\end{theorem} 

\textcolor{red}{Since the lower bound of $\tilde{C}$ in Remark 1 is related to $k$, ranges of $k$ and $T$ in Theorem \ref{thm:opt-batch} and Corollary 1 need to be modified. If $\tilde{C}$ is set as $\tilde{C} = \frac{d+1-d_z}{d_z - 1 + kd_s}$, then $k \leq \frac{ \left( \log \frac{T}{\log T} - d - d_z\right) + \sqrt{\left( \log \frac{T}{\log T} - d - d_z\right)^2 + 4\left( (d_z-1)\log \frac{T}{\log T} - d d_z \right)} }{2d_s}$, and $\log \frac{T}{\log T} > \max\{d+d_z, \; d-d_z+2 + 2\sqrt{d-d_z+1 } \}$ is sufficient?}
% 
% ----------------------------------------------------

% Theorem \ref{thm:opt-batch} 


The results of Theorem \ref{thm:opt-batch} can be rephrased as follows. 

\begin{corollary} 
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:large-d} with $\epsilon = \frac{1}{T^2}$ and edge-length sequence defined in Definition \ref{def:ace}. For each total time horizon $ T \in \mathbb{N} $ such that $ (d+1-d_z) \log \frac{T}{\log T} - d d_z > 0 $, let $ k = \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} $. 
    % Define the edge-length sequence as 
    % $ Let $ \epsilon = \frac{1}{T^2} $ and 
    Then there exists a sequence $ \{ G_T \}_{T} $ such that (1) $ G_T = \mathcal{O} \( \( \frac{T}{\log T} \)^{-\frac{1}{d_s}} \) $, and (2) for each $T \in \mathbb{N}$,
    with probability exceeding $ 1 - \frac{1}{T} $, the final optimality gap of Algorithm \ref{alg:large-d} is no larger than $ G_T $.  
\end{corollary} 

\begin{proof}
    For any $T$, we let $ k $ take the maximum possible value in Theorem \ref{thm:opt-batch}. We know as $T$ approaches infinity, the value of $ \( \frac{ \kappa T (2^{d_z + kd_s} -1) }{2 C_z \log (T ) 2^{d_z + kd_s}} \)^{- \frac{ 1+k }{d_z + kd_s}} $ is of order $ \mathcal{O} \( \( \frac{T}{\log T} \)^{-\frac{1}{d_s}} \) $.
\end{proof} 


When $d_z \ge d_s$, we have $ -\frac{1+k}{d_z + k d_s} \le - \frac{1}{d_z} $. In this case, BLiN-MOS outperforms BLiN. When $d_z < d_s$, we have $ -\frac{1+k}{d_z + k d_s} > - \frac{1}{d_z} $. In this case, BLiN outperforms BLiN-MOS. 
% Moreover, when $d_z > d_s$, $-\frac{1+k}{d_z+k d_s}$ is decreasing with respect to $k$. 

The proof to Theorems \ref{thm:small-d} and \ref{thm:opt-batch} follow a similar path. Next we present the proof for Theorem \ref{thm:opt-batch}, and the proof of Theorem \ref{thm:small-d} can be found in the appendix. 

% ---------------------------------------------------- 

\begin{proof}[Proof of Theorem \ref{thm:opt-batch}] 
    Denote $\tilde{r}_n = 2^{-\sum_{i=1}^n c_i}$. 
    
    \textbf{Case I}: $m = 2n-1$. In this case, we have $r_m \geq \tilde{r}_n, r_{m-1} \leq \tilde{r}_{n-1}$. 
    Since $\Delta_x \leq 3Lr_{m-1}$ for any $x \in \cup_{q_m\in \mathcal{A}_m}q_m$, any cube in $\mathcal{A}_{m-\frac{1}{2}}$ is a subset of $S(3Lr_{m-1})$. Therefore,
    \begin{equation*}
        |\mathcal{A}_{m-\frac{1}{2}}| \leq N_{r_{m-1}} \leq C_z r_{m-1}^{-d_z}.
    \end{equation*}
    After partitioning $\mathcal{A}_{m-\frac{1}{2}}$ into $\mathcal{A}_m$, we get
    \begin{equation*}
        |\mathcal{A}_m| = \left(\frac{r_{m-1}}{r_m}\right)^d |\mathcal{A}_{m-\frac{1}{2}}| \leq \left(\frac{\tilde{r}_{n-1}}{\tilde{r}_n}\right)^d \cdot C_z r_{m-1}^{-d_z}.
    \end{equation*}
    Denote the total budget of the $m$-th batch as $N_m$, then
    \begin{equation*}
    \begin{aligned}
        && N_m = |\mathcal{A}_m| \cdot n_m & 
        \leq \left(\frac{r_{m-1}}{\tilde{r}_n}\right)^d \cdot C_z r_{m-1}^{-d_z} \cdot \frac{\log (1/\epsilon)}{\kappa_s \alpha_m^{ d_s }} 
        \leq \frac{C_z \log (1/\epsilon)}{\kappa_s } \cdot \frac{ \tilde{r}_{n-1}^{d-d_z+1} \cdot \tilde{r}_n^{-k d_s -d} }{r_{m-1}} \\
        && & = \frac{C_z \log (1/\epsilon)}{\kappa_s r_{m-1}} \cdot 2^{(d_z+k d_s -1)\sum_{i=1}^{n-1}c_i + (k 
        d_s +d)c_n}
    \end{aligned}
    \end{equation*}
    Define $C_n = (d_z+k d_s -1)\sum_{i=1}^{n-1}c_i + (k d_s +d)c_n$, then $C_n - C_{n-1} = (d_z-d-1)c_{n-1} + (k d_s +d)c_n = 0$. So for any $n > 1$, we have $C_n = C_1 = (k d_s +d)c_1$. Consequently, we obtain the upper bound of $N_m$ for $m = 2n-1$ as follows,
    \begin{equation*}
        N_m \leq \frac{C_z \log (1/\epsilon)}{\kappa_s r_{m-1}} \cdot \left(\frac{T}{\log T}\right)^{\frac{d_z+k d_s -1}{d_z+k d_s }}.
    \end{equation*}

    \textbf{Case II}: $m = 2n$.  Note that $r_{m-1} = \min\{r_{m-2},2^{-a_n} \} = r_{m-2}$ happens only when $\lceil \sum_{i=1}^{n-1}c_i \rceil > \lfloor \sum_{i=1}^{n}c_i \rfloor$. If the previous inequality holds, then $r_m = 2^{-\lceil \sum_{i=1}^{n}c_i \rceil } = 2^{-\lfloor \sum_{i=1}^{n}c_i \rfloor - 1} \geq 2^{-\lceil \sum_{i=1}^{n-1}c_i \rceil } = r_{m-2}$, which contradicts the assumption that $\{b_n\}$ is a strictly increasing sequence. Therefore, it must hold that $r_{m-1} = 2^{-a_n} = 2^{-b_n + 1} = 2r_m$. We thus conclude from Lemma \ref{lem:opt-gap} that any cube in $\mathcal{A}_m$ is a subset of $S(6Lr_m)$.  Therefore,
    \begin{equation*}
        N_m = |\mathcal{A}_m| \cdot n_m 
        \leq \frac{C_z\log (1/\epsilon)}{\kappa_s} \cdot r_m^{-d_z} \cdot r_m^{-k d_s }
    \end{equation*}

    Since the total budgets of all $M^*$ batches is $T$, 
    \begin{equation*}
    \begin{aligned}
        && T & \leq \sum_{m=2n-1, m\leq M^*} N_m + \sum_{m=2n, m\leq M^*} N_m \\
        && & \leq \frac{2C_z}{\kappa} \left( \sum_{m=2n-1, m\leq M^*} \frac{1}{r_{m-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k d_s }} + \sum_{m=2n, m\leq M^*} r_m^{-d_z-k d_s } \cdot \log T\right)
    \end{aligned}
    \end{equation*}
    
    Since $\{b_n\}$ is strictly increasing, we know that $r_{m} = 2r_{m+1} \geq 2\min\{r_{m+1},2^{-a_{\frac{m+1}{2}}}\} = 2r_{m+2}$ when $m$ is odd and $r_{m} \geq 2 r_{m+2}$ when $m$ is even. So $r_{m+2} \leq \frac{1}{2} r_m$ holds for any $m \in \mathbb{N}$. Following this, when $M^*$ is odd, $\sum_{m=2n-1,m\leq M^*} \frac{1}{r_{m-1}} \leq \left( \sum_{n=0}\frac{1}{2^n} \right) \cdot \frac{1}{r_{M^*-1}} = \frac{2}{r_{M^*-1}}$, $ \sum_{m=2n, m\leq M^*} \frac{1}{r_m^{d_z+k 
    d_s }} \leq \left(\sum_{n=0} \frac{1}{2^{n(d_z+k d_s )}}\right) \cdot {\frac{1}{r_{M^*-1}^{d_z+k d_s }}} = \frac{2}{r_{M^*-1}^{d_z+k 
    d_s }}$. Therefore, 
    \begin{equation*}
        T \leq \frac{4C_z}{\kappa_s} \cdot \left( \frac{1}{r_{M^*-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k 
        d_s }} + \frac{1}{r_{M^*-1}^{d_z+k d_s }} \cdot \log T \right).
    \end{equation*}
    Set $C = \max\{8C_z/\kappa_s,(8C_z/\kappa_s)^{\frac{1}{d_z+k 
    d_s }}\}$. We claim that $r_{M^*-1} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$ must hold. Otherwise, 
    \begin{equation*}
        \frac{4C_z}{\kappa_s} \cdot \left( \frac{1}{r_{M^*-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k d_s }} + \frac{1}{r_{M^*-1}^{d_z+k d_s }} \cdot \log T \right) < T,
    \end{equation*} 
    which yields contradiction. So we obtain $r_{M^*-1} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$, and $r_{M^*} \leq r_{M^*-1} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$.

    Similarly, when $M^*$ is even, we have
    \begin{equation*}
        T \leq \frac{4C_z\log T}{\kappa_s} \cdot \left( \frac{1}{r_{M^*}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} + \frac{1}{r_{M^*}^{d_z+k d_s }}\right).
    \end{equation*}
    Implementing the same deduction process as when $M^*$ is odd, we get $r_{M^*} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$.

    With $r_{M^*}$ upper bounded as above, the simple regret of the last batch $M^*$ can achieve an order smaller than or equal to $\mathcal{O}\left( \left( \frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }} \right)$:
    \begin{equation}
        \label{eq:simple-regret}
        f^*_q - Y^{\max}_{M^*} \leq \rho_{M^*} = L\alpha_{M^*} r_{M^*} = L r_{M^*}^{1+k } \leq cL\left(\frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }},
    \end{equation}
    where $c$ is a constant.

    To see that only $ O (\log \log T) $ batches are needed, we note that $\tilde{r}_{M} = 2^{-\sum_{i=1}^{M} c_i} = 2^{-c_1 \cdot \frac{1-\eta^{M}}{1-\eta}} = \left( \frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s } + \frac{\eta^{M}}{d_z+k d_s }}$. By letting $\frac{\eta^{M^{**}}}{d_z+k d_s } \leq \frac{ \textcolor{red}{\tilde{C}} }{\log \frac{T}{\log T}}$ ($\tilde{C}$ is a constant determined in Remark \ref{rm:batch} ), that is, choosing $M^{**} \geq \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s ) \textcolor{red}{ - \log \tilde{C} } }{\log \frac{d+k d_s }{d+1-d_z}}$, we can achieve $\tilde{r}_{M^{**}} \leq \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$. Since $r_m \leq \tilde{r}_{M^{**}}$ for $m\geq 2M^{**}$, only $2M^{**}+1$ batches are needed to achieve the simple regret in (\ref{eq:simple-regret}).
    

    Finally, the choice of $k$ in the final optimality gap is not arbitrary. 
    To ensure at least one round of narrowing, we need to ensure that $M^* \ge 1$. By (\ref{eq:lower-M-1}), it is sufficient to ensure that 
    \begin{align*}
        \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} \ge 1, 
    \end{align*}
    which implies 
    \begin{align*} 
        % \frac{1-d_z}{d_s} < 
        k 
        \le 
        \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} . 
        % k \le \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } . 
    \end{align*} 
\end{proof}


----------------------------------------------------

----------------------------------------------------


\begin{theorem}
    \label{thm:large-d} 
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:large-d}. Let $ T $ be the total time horizon, and let $ \epsilon = \frac{1}{T^2} $. In addition, let $T$ be large enough so that $ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z  > 0 $. Let $ k \in \( 0, \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } \] $. Define the edge-length sequence as $ r_m = 2^{-m}$. 
    % $ Let $ \epsilon = \frac{1}{T^2} $ and 
    Then with probability exceeding $ 1 - \frac{1}{T} $, the final optimality gap of Algorithm \ref{alg:large-d} is no larger than $ L \( \frac{ \kappa T (2^{d_z + kd_s} -1) }{2 C_z \log (T ) 2^{d_z + kd_s}} \)^{- \frac{ 1+k }{d_z + kd_s}} $.  
\end{theorem} 


\begin{corollary} 
    \label{cor1}
    Instate Assumption \ref{assumption:lip} and consider Algorithm \ref{alg:large-d} with $\epsilon = \frac{1}{T^2}$ and edge-length sequence $ r_m = 2^{-m} $. For each total time horizon $ T \in \mathbb{N} $ such that $ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 8 C_z \log ( T ) \kappa_s T } }{4 C_z \log ( T ) } \) - d_z  > 0 $, let $ k = \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 8 C_z \log ( T ) \kappa_s T } }{4 C_z \log ( T ) } \) - d_z }{ d_s } $. 
    % Define the edge-length sequence as 
    % $ Let $ \epsilon = \frac{1}{T^2} $ and 
    Then there exists a sequence $ \{ G_T \}_{T} $ such that (1) $ G_T = O \( \( \frac{T}{\log T} \)^{-\frac{1}{d_s}} \) $, and (2) for each $T \in \mathbb{N}$,
    with probability exceeding $ 1 - \frac{1}{T} $, the final optimality gap of Algorithm \ref{alg:large-d} is no larger than $ G_T $.  
\end{corollary} 

\begin{proof} 
    % It suffices to consider large $T$. 
    % When $k = \frac{}{} $
    By letting $ k = \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 8 C_z \log ( T ) \kappa_s T } }{4 C_z \log ( T ) } \) - d_z }{ d_s } $ in Theorem \ref{thm:large-d}, we know as $T$ approaches infinity, the value of $ \( \frac{ \kappa T (2^{d_z + kd_s} -1) }{2 C_z \log (T ) 2^{d_z + kd_s}} \)^{- \frac{ 1+k }{d_z + kd_s}} $ is of order $ O \( \( \frac{T}{\log T} \)^{-\frac{1}{d_s}} \) $. 
\end{proof} 

In addition, BLiN-MOS only needs $O (\log \log T)$ rounds of communications to asymptotically achieve the $O (T^{-\frac{1}{d_s}})$ regret bound, as stated in the following theorem. 
 
% \textcolor{red}{(Draw a figure to illustrate the algorithm procedure. )} 

% \subsection{When $d_z$ is small}
% : Simple is Good} 

% \textcolor{red}{Task for Yasong: Summarize some results from \citep{feng2023hpo}. } 

% \input{./tex/blie-theory.tex}

% \begin{lemma}
%     \label{lem:survive-small} 
%     Instate Assumption \ref{assumption:lip}. 
%     Throughout the entire procedure of Algorithm \ref{alg:small-d}, the optimal arm $x^*$ is not eliminated. 
% \end{lemma} 

% \begin{proof}
%     For any batch $m$, let $q_m^*$ be the cube in $\A_m$ that contains $x^*$, and let $q_m^{\max}$ be the cube in batch $m$ such that $ f (x_{q_m^{\max}}) = Y_m^{\max} $. Then for any $m = 1,2,\cdots$, we have 
%     \begin{align*}
%         Y_m^{\max} - f ( x_{q_m^*} ) 
%         = 
%         f ( x_{q_m^{\max}} ) - f ( x_{q_m^*} ) 
%         \overset{(i)}{\le} 
%         f ( x_{q_m^{\max}} ) - f^*  + L 2^{-m} 
%         \le 
%         L 2^{-m} , 
%     \end{align*}
%     where $(i)$ follows from Lipschitzness of $f$. 
%     The above derivation implies that $ q_m^* $ is not eliminated. Thus $x^*$ is not eliminated. 
%     % Let $q_m^*$ be a cube in $\mathcal{A}_m$ that contains $x^*$, and let $q_m^{\max} \in \arg \max_{q \in \mathcal{A}_m} {Y}_{q, n_m}^{\max} $.
%     % Under the event $\mathcal{E}$, we have 
%     % \begin{align*} 
%     %     \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} )) 
%     %     = 
%     %     \wh{c}_{n_m, \alpha_m} (f (X_{I_m^{\max}} )) - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} ))  
%     %     \le 
%     %     f_{I_m^{\max}}^* - f_{I_m^{*}}^* + \rho_m 
%     %     \le 
%     %     \rho_m , 
%     % \end{align*} 
%     % which implies that $ I_m^* $ is not eliminated. 
% \end{proof} 

% \begin{lemma} 
%     \label{lem:y-gap-small}
%     % Let $ f^* = \max_{x \in [0,1]^d} f (x) $. 
%     % Under event $\mathcal{E}$, 
%     Instate Assumption \ref{assumption:lip}. Then it holds that 
%     $f^* - Y_{m}^{\max} \le L2^{-m}$ for all $m = 1,2,\cdots$. 
% \end{lemma} 

% \begin{proof} 
%     Let $ q_m^* $ be the cube in $\mathcal{A}_m$ that contains $x^*$, and let $q_m^{\max}$ be the cube in batch $m$ such that $ f (x_{q_m^{\max}}) = Y_m^{\max} $. Then we have 
%     \begin{align*} 
%         f^* - Y_{m}^{\max} 
%         = 
%         f_{q_m^*}^{\max} - f (x_{q_m^{\max}})
%         \le 
%         f ( x_{q_m^*} ) + L2^{-m} - Y_{m}^{\max} 
%         \le 
%         L 2^{-m} . 
%     \end{align*} 
% \end{proof} 


% \begin{lemma} 
%     \label{lem:opt-gap-small}
%     Instate Assumption \ref{assumption:lip}.  The arms in $\mathcal{A}_m$ are $ L 2^{-m+1} $-optimal for all $ m = 1, 2, \cdots $. 
% \end{lemma} 

% \begin{proof} 
%     % The arms in $\mathcal{A}_m$ are 
%     Let $q$ be a cube in $\mathcal{A}_m $. By Lemma \ref{lem:y-gap-small}, we have 
%     \begin{align*}
%         % f_{q_m^*}^{\max} - f_q^{\max} 
%         % \le 
%         f_{q_m^*}^{\max} - f_q^{\max} 
%         \le 
%         Y_{q_m^*,n_m} + L 2^{-m} - Y_{q,n_m} 
%         \le 
%         Y_{m}^{\max} + L 2^{-m} - Y_{q,n_m} 
%         \le 
%         L 2^{- 2 m + 1 }, 
%     \end{align*}
%     where the last inequality follows from the fact that $ q $ is not eliminated. The above inequalities imply that
%     % it holds that 
%     \begin{align*}
%         f^* - f_{q}^{\min} 
%         \le 
%         f_{q_m^*}^{\max} - f_q^{\max} + L 2^{-m} 
%         \le
%         L 2^{-m} + L 2^{-2m+1} 
%         \le 
%         L 2^{-m+1}. 
%         % 
%     \end{align*}
% \end{proof} 



% -----------------------------------------------------------------


% We let $B$ be the total number of batches of the BLiE run ($B-1$ batches in the for-loop and $1$ clean-up batch), and $N_m$ be the total budget of batch $m$. In the following analysis, we bound $N_m$ for $m=2k-1$ and $m=2k$ separately, and then obtain the simple regret upper bound.

% Firstly, we consider the case $m=2k-1$. For convenience, we let $\widetilde{r}_k=2^{-\sum_{i=1}^kc_i}$, and thus we have $\widetilde{r}_{k-1}\geq r_{m-1}\geq r_m\geq \widetilde{r}_{k}$. Recall that $\mathcal{A}_{m-1}^+$ is set of cubes not eliminated in batch $m-1$, and $\cup_{C\in\mathcal{A}_{m-1}^+}C=\cup_{C^\prime\in\mathcal{A}_m}C^\prime$. Lemma \ref{lem:eli} implies that each cube in $\mathcal{A}_{m-1}^+$ is a subset of $S((4L+4)r_{m-1})$, and thus $\left|\mathcal{A}_{m-1}^+\right|\leq N_{r_{m-1}}\leq C_z\cdot r_{m-1}^{-d_z}$. The total budget of batch $m$ is
% \begin{align*}
%     N_m=& \; |\mathcal{A}_m|\cdot n_m = \left(\frac{r_{m-1}}{r_m}\right)^d\left|\mathcal{A}_{m-1}^+\right|\cdot n_m\\
%     \leq& \; C_z\cdot\frac{r_{m-1}^{d+1-d_z}\cdot r_m^{-d-\beta}}{r_{m-1}} 
%     \leq C_z\cdot\frac{\widetilde{r}_{k-1}^{d+1-d_z}\cdot\widetilde{r}_k^{-d-\beta}}{r_{m-1}}.
% \end{align*}
% For the numerator, we have
% \begin{align*}
%     \widetilde{r}_{k-1}^{d+1-d_z}\cdot\widetilde{r}_k^{-d-\beta}
%     =& \; 2^{-\left(\sum_{i=1}^{k-1}c_i\right)(d+1-d_z)+\left(\sum_{i=1}^{k}c_i\right)(d+\beta)} \\ 
%     =& \; 2^{\left(\sum_{i=1}^{k-1}c_i\right)(d_z+\beta-1)+c_m(d+\beta)}.
% \end{align*}
% Define $C_m=\left(\sum_{i=1}^{k-1}c_i\right)(d_z+\beta-1)+c_m(d+\beta)$. Since $c_m=c_{m-1}\cdot\frac{d+1-d_z}{d+\beta}$, calculation shows that $C_m = (\sum_{i=1}^{m-2} c_i) (d_z+\beta-1)  + c_{m-1}(d+\beta)+ c_{m-1}(d_z+\beta-1-d-\beta)+c_m(d+\beta)=C_{m-1}$. Thus for any $m$, we have $C_M=C_1=\frac{d_z+\beta-1}{d_z+\beta}\log T$. Hence,
% \begin{equation*}
%     N_m\leq C_z\cdot2^{\frac{d_z+\beta-1}{d_z+\beta}\log T}/r_{m-1}=C_z\cdot T^{\frac{d_z+\beta-1}{d_z+\beta}}/r_{m-1}.
% \end{equation*}

% Secondly, we consider the case $m=2k$. Lemma \ref{lem:eli} implies that each cube in $\mathcal{A}_m$ is a subset of $S(8L+8)r_m$. Similar argument to the first case shows that $\left|\mathcal{A}_m\right|\leq C_z\cdot r_m^{-d_z}$ and $N_m\leq C_z\cdot r_m^{-(d_z+\beta)}$.

% % The rounding step in Definition \ref{def:ace} yields that $r_m\leq\frac{r_{m-1}}{2}$ for any $m$. 
% Line 7 of Algorithm \ref{BLiN} ensures that the sum of budgets of full $B$ batches is greater than $T$. Therefore, combining the above two cases, we have
% \begin{align}\label{upp-budget-ace}
%     T\leq&\sum_{\substack{m=2k-1, \\ m\leq B }}C_z \cdot\frac{T^{\frac{d_z+\beta-1}{d_z+\beta}}}{r_{m-1}}+\sum_{\substack{m=2k,\\m\leq B}}C_z\cdot \frac{1}{r_m^{d_z+\beta}}.
% \end{align}

% % \begin{align}\label{upp-budget-ace}
% %     T\leq&\sum_{\substack{m=2k-1, \\ m\leq B }}C_z\cdot T^{\frac{d_z+\beta-1}{d_z+\beta}}\cdot\frac{1}{r_{m-1}}+\sum_{\substack{m=2k,\\m\leq B}}C_z\cdot \frac{1}{r_m^{d_z+\beta}}\nonumber\\
% %     \leq&2C_z\cdot T^{\frac{d_z+\beta-1}{d_z+\beta}}\cdot\frac{1}{r_{B}}+2C_z\cdot\frac{1}{r_{B}^{d_z+\beta}}.
% % \end{align}
% The rounding step in Definition \ref{def:ace} yields that $r_m\leq\frac{r_{m-1}}{2}$ for any $m$. If $B$ is odd, from (\ref{upp-budget-ace}) we have $T\leq2C_z\cdot T^{\frac{d_z+\beta-1}{d_z+\beta}}\cdot\frac{1}{r_{B-1}}+2C_z\cdot\frac{1}{r_{B-1}^{d_z+\beta}}$.  We set $c_r=\max\{(4C_z)^\frac{1}{d_z+\beta}, 4C_z\}$, then $\frac{1}{c_r^{d_z+\beta}}+\frac{1}{c_r}\leq\frac{1}{2C_z}$ and the above inequality implies that $r_{B-1}\leq c_r\cdot T^{-\frac{1}{d_z+\beta}}$. Lemma \ref{lem:eli} shows that $\Delta_x\leq(4L+4)r_{B-1}$ for any $x\in\cup_{C\in\mathcal{A}_B}C$, so we have $\Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z+\beta}}$, where $c=(8L+8)\cdot\max\{c_r, 1\}$. If $B$ is even, similar arguments also yleid that $\Delta_{\widetilde{x}^*}\leq c\cdot T^{-\frac{1}{d_z+\beta}}$. See Appendix \ref{app:race} for details.

% Finally, we consider the communication bound. For any $B^*$, $\widetilde{r}_{B^*}=2^{-\sum_{i=1}^{B^*}c_i}=2^{-c_1\cdot\frac{1-\eta^{B^*}}{1-\eta}}=T^{-\frac{1}{d_z+\beta}}\cdot T^{\frac{\eta^{B^*}}{d_z+\beta}}$. Then by choosing $B^*\geq\frac{\log\log T-\log(d_z+\beta)}{\log\frac{d+\beta}{d+1-d_z}}$, we have $\frac{\eta^{B^*}}{d_z+\beta}\leq\log T$ and $\widetilde{r}_{B^*}\leq T^{-\frac{1}{d_z+\beta}}$. Definition \ref{def:ace} shows that $r_m<\widetilde{r}_{B^*}$ for any $m\geq2B^*$. As a consequence, no more than $\hat{B}=\frac{2\log\log T}{\log\frac{d+\beta}{d+1-d_z}} + 1$ batches are needed to achieve $r_{\hat{B}-1}\leq T^{-\frac{1}{d_z+\beta}}$ and $\Delta_{\widetilde{x}^*}\leq (4L+4)T^{-\frac{1}{d_z+\beta}}\leq c\cdot T^{-\frac{1}{d_z+\beta}}$.

-----------------------------------------------------------------



\subsection{When $d_s$ is small} 
% : Max Order Statistics (MOS) is Helpful} 


% \begin{assumption}
%     \label{assumption:ord}
%     % We assume that the following items are true. 
%     % \begin{itemize}
%     There exists $\kappa \in (0,1) $, such that for any $\alpha \in [0, \frac{ 1 }{2} ]$, and any cube $q$
%     \begin{align*} 
%         \Pr \( f ( X_q ) \le f_q^{\max} -  \alpha ( f_q^{\max} - f_q^{\min} ) \) 
%         \le 
%         1 - \kappa \alpha . 
%     \end{align*} 
% \end{assumption}


Let $X_q$ denote the uniform random variable over $ q $.  




Consider $iid$ random variables $X_q^1, X_q^2, \cdots, X_q^n \in q $ and $Y_{q,n} = \max\{ f (X_q^1), f(X_q^2), \cdots, f(X_q^n) \} $. 
\begin{align*} 
    \Pr \( Y_{q,n} \le x \) 
    = 
    \prod_{i=1}^n \Pr \( f(X_q^i) \le x \) . 
\end{align*} 





% \begin{algorithm}[h]
% 	\caption{Optimization via Max Order Statistic (over $[0,1]^d$)} 
% 	\label{alg:new} 
% 	\begin{algorithmic}[1]  
%             \STATE \textbf{Assumption:} Suppose that the function $f$ has zooming dimension $d_z$ and zooming constant $C_z$. 
% 		\STATE \textbf{Input:} Time horizon $T$. $\epsilon \in (0,1)$. 
% 		\STATE \textbf{Initialization:} 
%   % Let $ \mathcal{A}_1 = \{ [0, \frac{1}{2}] , [\frac{1}{2}, 1] \} $. Let $ N_0 = 256A_\epsilon $. Let $ M = \lfloor \frac{ \log \( \frac{\gamma-1}{\gamma}\cdot \frac{T}{C_z N_0 } \) }{\log \gamma } \rfloor$. 
% 		\FOR{$m=1,2,\cdots,M$} 
%                 \STATE Compute $ n_m = \frac{\log \epsilon }{ \log \(1 - \kappa 2^{-m} \) } $. 
%                 % $\alpha_m = 1-(\frac{256 A_\epsilon }{ n_m })^{1/4} $, $\rho_m = 6 \kappa_+ \( \frac{A_\epsilon}{n_m} \)^{1/4} 2^{-m}$. 
%                 \FOR{cube $q \in \mathcal{A}_{m} $} 
%                     \STATE Uniformly randomly sample $n_m$ points from $q$, and compute $ Y_{q, n_m } $. 
%                     \STATE Compute $ Y_m^{\max} := \max_{q \in \mathcal{A}_m } Y_{q,n_m} $. 
%                     \STATE Let $\mathcal{A}_{m+\frac{1}{2}} = \{ q \in  \mathcal{A}_m : {Y}_m^{\max} - {Y}_{q,n_m} \le \rho_m \}$. /* Elimination step */
%                     \STATE Dyadically partition the cubes in $\mathcal{A}_{m + \frac{1}{2}}$, and collect these intervals to form $ \mathcal{A}_{m+ 1 } $. 
%                     % = \{ I: \in  \mathcal{A}_{m+\frac{1}{2}} : \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m } \le \rho_m \} $
%                 \ENDFOR 
% 		\ENDFOR
%             \STATE \textbf{Output}: $Y_{M}^{\max}$. 
%     % \STATE \textbf{Cleanup:} Arbitrarily play the remaining arms until all $T$ steps are used.  
% 	\end{algorithmic} 
% \end{algorithm} 


\begin{lemma}
    \label{lem:hp}
    Instate Assumptions \ref{assumption:lip}. For any $\alpha \in (0,1)$, any positive integer $n$ and any cube $q^*$ such that $x^* \in q^*$, it holds that 
    \begin{align*}
        \Pr \( f_{q^*}^{\max} - Y_{q^*,n} > \alpha L \D (q^*) \) 
        \le& \;  
        % \Pr \( f_q^{\max} - Y_{q,n} \ge \alpha \( f_q^{\max} - f_q^{\min} \) \) \\ 
        % =& \; 
        % \Pr \(  Y_{q,n} \le f_q^{\max} - \alpha \( f_q^{\max} - f_q^{\min} \) \) \\ 
        % =& \; 
        % \prod_{i=1}^n \Pr \( f ( X_q^i ) \le f_q^{\max} - \alpha \( f_q^{\max} - f_q^{\min} \) \) \\ 
        % \le& \; 
        (1 - \kappa_s \alpha^{d_s} )^n . 
    \end{align*}
    
    % Fix any $\epsilon \in (0,1)$, and let $ n_m = \frac{\log \epsilon}{(1 - \kappa 2^{-m})} $. Then we have 
    % \begin{align*} 
    %     \Pr \( f_q^{\max} - Y_{q,n_m} \le 2^{-m} \) \ge 1 - \epsilon .  
    % \end{align*} 
\end{lemma}

\begin{proof}
    It holds that 
    \begin{align*}
        \Pr \( f_{q^*}^{\max} - Y_{q^*,n} > \alpha L \D (q^*) \) 
        \le& \;  
        \Pr \( f_{q^*}^{\max} - Y_{q^*,n} > \alpha \( f_{q^*}^{\max} - f_{q^*}^{\min} \) \) \tag{by $L$-Lipschitzness} \\ 
        =& \; 
        \Pr \(  Y_{q^*,n} < f_{q^*}^{\max} - \alpha \( f_{q^*}^{\max} - f_{q^*}^{\min} \) \) \\ 
        =& \; 
        \prod_{i=1}^n \Pr \( f ( X_{q^*}^i ) < f_{q^*}^{\max} - \alpha \( f_{q^*}^{\max} - f_{q^*}^{\min} \) \) \\ 
        \le& \;  
        \( 1 - \kappa_s \alpha^{d_s} \)^n , 
        % \tag{by Assumption \ref{assumption:ord} and that $\{ X_{q^*}^i\}_{i=1}^n $ are $iid$} 
    \end{align*} 
    where the last inequality follows from Definition of scattering dimension and that $\{ X_{q^*}^i\}_{i=1}^n $ are $iid$.  
\end{proof} 

\begin{lemma} 
    \label{lem:event}
    Denote $ \rho_m = L \alpha_m r_m$. Let $n_m$ be defined as in Algorithm \ref{alg:large-d}. Let 
    \begin{align*} 
        \mathcal{E} := \left\{ f_q^{\max} - Y_{q,n_m} \le \rho_m, \; \forall m = 1,2,\cdots, M,\; \text{ and } \;  \forall q \in \mathcal{A}_m \text{ such that } x^* \in q \right\} , 
    \end{align*} 
    and let $\epsilon = \frac{1}{T^2}$. 
    Then $\Pr \( \mathcal{E}\) \ge 1 - \frac{1}{T}$. 
\end{lemma} 

\begin{proof} 

    Since at most $T$ arms are pulled, there are at most $T$ cubes that contain arms. We apply Lemma \ref{lem:hp} and take a union bound over these cubes to conclude the proof. 
\end{proof} 

\begin{proposition}
    \label{prop:inc}
    Let $\kappa \in (0,1]$ and $\gamma > 1$. 
    For any $ x \in [1,\infty) $, it holds that 
    \begin{align*}
        - \frac{\gamma^{x}}{\gamma \log (1 - \frac{\kappa}{\gamma}) } \le - \frac{1}{\log(1 - \kappa \gamma^{-x})} \le \frac{\gamma^{x}}{\kappa}. 
    \end{align*} 

\end{proposition}

\begin{proof}
    Consider function $h: [1, \infty ) \to \R$ defined as 
    \begin{align*} 
        h (x) = - \frac{\kappa }{ \gamma^x \log(1 - \kappa \gamma^{-x}) } . 
    \end{align*} 
    Clearly, $h(1) = - \frac{\kappa }{ \gamma \log (1 - \frac{\kappa}{\gamma}) } $. By noting $ \log(1 - \kappa \gamma^{-x}) = - \kappa \gamma^{-x} + o (\gamma^{-x})$ when $x$ is large, we know that 
    \begin{align*}
        \lim_{x \to \infty} h (x) = 1. 
    \end{align*} 
    Also, we know that 
    \begin{align*}
        h' (x) = \frac{\kappa \gamma^x \log \gamma}{ (\gamma^x \log (1 - \kappa \gamma^{-x}) )^2 } \( \log \( 1 - \kappa \gamma^{-x} \) + \frac{\kappa \gamma^{-x}}{1 - \kappa \gamma^{-x}} \). 
    \end{align*}
    Since $ \log (1-z) \ge \frac{-z}{\sqrt{1-z}} $ for all $z \in (0,1)$, we know $ h' (x) > 0 $ for all $x \in [1,\infty)$. 
    Thus $ h $ is increasing over $ [1,\infty) $. Therefore $ - \frac{\gamma^{x}}{\gamma \log (1 - \frac{\kappa}{\gamma}) } \le - \frac{1}{\log(1 - \kappa \gamma^{-x})} \le \frac{\gamma^{x}}{\kappa} $ for all $x \in [1,\infty)$. 
\end{proof}









\iffalse
\begin{lemma}
    \label{lem:survive} 
    Under the event $\mathcal{E}$, the optimal arm $x^*$ is not eliminated. 
\end{lemma} 

\begin{proof}
    Let $q_m^*$ be the cube in batch $m$ that contains $x^*$. Let $q_m^{\max}$ be the cube in batch $m$ such that $ Y_{q_m^{\max},n} =   Y_m^{\max} $. Then we have 
    \begin{align*}
        Y_m^{\max} - Y_{q_m^*,n}  
        = 
        Y_{q_m^{\max}}^{\max} - Y_{q_m^*,n}  
        \le 
        f_{q_m^{\max}}^{\max} - f_{q_m^{*}}^{\max} + L 2^{-2m} 
        \le 
        L 2^{-2m} , 
    \end{align*}
    which implies that $ q_m^* $ is not eliminated. Thus $x^*$ is not eliminated. 
    % Let $q_m^*$ be a cube in $\mathcal{A}_m$ that contains $x^*$, and let $q_m^{\max} \in \arg \max_{q \in \mathcal{A}_m} {Y}_{q, n_m}^{\max} $.
    % Under the event $\mathcal{E}$, we have 
    % \begin{align*} 
    %     \wh{C}_m^{\max} - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} )) 
    %     = 
    %     \wh{c}_{n_m, \alpha_m} (f (X_{I_m^{\max}} )) - \wh{c}_{n_m, \alpha_m} (f (X_{I_m^*} ))  
    %     \le 
    %     f_{I_m^{\max}}^* - f_{I_m^{*}}^* + \rho_m 
    %     \le 
    %     \rho_m , 
    % \end{align*} 
    % which implies that $ I_m^* $ is not eliminated. 
\end{proof} 

\begin{lemma} 
    \label{lem:y-gap}
    Let $ f^* = \max_{x \in [0,1]^d} f (x) $. 
    Under event $\mathcal{E}$, $f^* - Y_{m}^{\max} \le L2^{-2m}$. 
\end{lemma} 

\begin{proof} 
    Let $ q_m^* $ be the cube in $\mathcal{A}_m$ that contains $x^*$. Then we have 
    \begin{align*} 
        f^* - Y_{m}^{\max} 
        = 
        f_{q_m^*} - Y_{m}^{\max} 
        \le 
        Y_{q_m^*, n_m} + L2^{-2m} - Y_{m}^{\max} 
        \le 
        L 2^{-2m} . 
    \end{align*} 
\end{proof} 


\begin{lemma} 
    \label{lem:opt-gap}
    Under event $\mathcal{E}$, the arms in $\mathcal{A}_m$ are $ L 2^{-m+1} $-optimal for all $ m = 1,2,\cdots, M $. 
\end{lemma} 

\begin{proof} 
    % The arms in $\mathcal{A}_m$ are 
    Let $q$ be a cube in $\mathcal{A}_m $. By Lemma \ref{lem:y-gap}, we have 
    \begin{align*}
        % f_{q_m^*}^{\max} - f_q^{\max} 
        % \le 
        f_{q_m^*}^{\max} - f_q^{\max} 
        \le 
        Y_{q_m^*,n_m} + L 2^{-2m} - Y_{q,n_m} 
        \le 
        Y_{m}^{\max} + L 2^{-2m} - Y_{q,n_m} 
        \textcolor{red}{\le 
        L 2^{-2m+1}}, 
    \end{align*}
    where the last inequality follows from the fact that $ q $ is not eliminated. The above inequalies imply that
    % it holds that 
    \begin{align*}
        f^* - f_{q}^{\min} 
        \le 
        f_{q_m^*}^{\max} - f_q^{\max} + L 2^{-m} 
        \le
        \textcolor{red}{L 2^{-m} + L 2^{-2m+1} 
        \le 
        L 2^{-m+1}}. 
        % 
    \end{align*}
\end{proof} 
\fi


\begin{lemma}
    \label{lem:survive}
    Under the event $\mathcal{E}$, the optimal arm $x^*$ is not eliminated.
\end{lemma}

\begin{proof}
    Let $q^*_m$ be the cube in batch $m$ that contains $x^*$. Let $q_m^{\max}$ be the cube in batch $m$ such that $Y_{q_m^{\max},n_m} = Y_m^{\max}$. Then we have
    \begin{equation*}
    Y_m^{\max} - Y_{q_m^*,n_m} = Y_{q_m^{\max},n_m} - Y_{q_m^*,n_m} \leq f_{q_m^{\max}}^{\max} - f^{\max}_{q^*_m} + \rho_m \leq \rho_m,
    \end{equation*}
    which implies that $q^*_m$ is not eliminated in batch $m$. Thus $x^*$ is not eliminated.
\end{proof}


\begin{lemma}
    \label{lem:y-gap}
    Let $f^* = \max_{x\in [0,1]^d}f(x)$. Under event $\mathcal{E}$, $f^*-Y_m^{\max} \leq \rho_m$.
\end{lemma}

\begin{proof}
    Let $q^*_m$ be the cube in $\mathcal{A}_m$ that contains $x^*$. Then we have
    \begin{equation*}
    f^* - Y_m^{\max} = f^{\max}_{q^*_m} - Y_{q_m^{\max},n_m} \overset{(i)}{\leq} Y_{q^*_m,n_m} + \rho_m - Y_{q_m^{\max},n_m} \leq \rho_m, 
    \end{equation*}
    where $(i)$ follows from the definition of $\mathcal{E}$ (in Lemma \ref{lem:event}).
    % the first inequality holds because we indicated in Lemma \ref{lem:survive} that $q^*_m$ is not eliminated in batch $m$.
\end{proof}


\begin{lemma}
    \label{lem:opt-gap}
    Under event $\mathcal{E}$, for any $m = 1,2,\cdots,M$, any $q_m \in \mathcal{A}_m$ and any $x\in q_m$, $\Delta_x$ satisfies
    $$
    \Delta_x \leq 3Lr_{m-1},
    $$
    where $L$ is the Lipschitz constant of $f(x)$.
\end{lemma}

\begin{proof}
    Let $q_m$ be a cube in $\mathcal{A}_m$ and let $x \in q_m$. By the Lipschitzness of $f$, we have
    \begin{equation*}
        |f(x) - Y_{q_m,n_m}| \leq Lr_m
    \end{equation*}
    Denote $Par(q_m)$ as the cube in $\mathcal{A}_{m-1}$ which contains $q_m$. Since $x \in q_m$, we know $x \in Par(q_m)$ and $Par(q_m)$ is not eliminated after batch $m-1$. Hence, it follows that $Y_{m-1}^{\max} - Y_{Par(q_m),n_{m-1}} \leq \rho_{m-1}$. Therefore,
    \begin{equation*}
    \begin{aligned}
        && f^* - f(x) & \leq Y_{m-1}^{\max} + \rho_{m-1} - Y_{Par(q_m),n_{m-1}} + Lr_{m-1} \\
        && & \leq 2\rho_{m-1} + Lr_{m-1} \\
        && & \leq 3Lr_{m-1}
    \end{aligned}
    \end{equation*}
    
\end{proof}



% \begin{lemma} 
%     Let $ f^* = \max_{x \in [0,1]^d} f (x) $. 
%     Under event $\mathcal{E}$, $f^* - Y_{m}^{\max} \le L2^{-2m}$. 
% \end{lemma} 

% \begin{proof} 
%     Let $ q_m^* $ be the cube in $\mathcal{A}_m$ that contains $x^*$. Then we have 
%     \begin{align*} 
%         f^* - Y_{m}^{\max} 
%         = 
%         f_{q_m^*} - Y_{m}^{\max} 
%         \le 
%         Y_{q_m^*, n_m} + L2^{-2m} - Y_{m}^{\max} 
%         \le 
%         L 2^{-2m} . 
%     \end{align*} 
% \end{proof} 

% So the simple regret is 
% \begin{align*}
    
% \end{align*}

% \textcolor{red}{some }

% \section*{Some Draft Below} 

\begin{proof}[Proof of Theorem \ref{thm:large-d}]
    
    Let $d_z$ be the zooming dimension. Then by Lemma \ref{lem:opt-gap}, we have 
    \begin{align*} 
        | \mathcal{A}_m | \le C_z 2^{m d_z}. 
    \end{align*} 
    
    
    In total we play $T$ arms, and thus 
    \begin{align*} 
        \sum_{m=1}^{M^*} | \mathcal{A}_m | n_m = T . 
    \end{align*} 
    Since $ | \mathcal{A}_m | \le C_z 2^{m d_z}$ and $n_m \le \frac{\log (1/\epsilon)}{\kappa_s } 2^{k d_s m} $, the above implies 
    \begin{align*} 
        \frac{C_z \log (1/\epsilon)}{\kappa_s } \sum_{m = 1}^{M^*}  2^{(d_z + k d_s ) m} \ge T . 
    \end{align*}
    
    Rearranging terms gives 
    \begin{align} 
        M^* \ge \frac{ \log \( \frac{ \kappa_s T (2^{d_z + k d_s} -1) }{C_z \log (1 / \epsilon ) 2^{d_z + k d_s}} \) }{ (d_z + k d_s) \log 2 } . \label{eq:lower-M-1}
    \end{align} 
    
    Therefore, the final simple regret is smaller than or equals to 
    \begin{align*} 
        f^*_q - Y^{\max}_{M^*}
        =
        \rho_{M^*}
        \le 
        L \( \frac{ \kappa T (2^{d_z + k d_s} -1) }{C_z \log (1 / \epsilon ) 2^{d_z + k d_s }} \)^{- \frac{ 1+k }{d_z + k d_s}} . 
    \end{align*} 

    % Finally, let us check the 
    The choice of $k$ in the above inequality is not arbitrary. 
    To ensure at least one round of narrowing, we need to ensure that $M^* \ge 1$. By (\ref{eq:lower-M-1}), it is sufficient to ensure that 
    \begin{align*}
        \frac{ \log \( \frac{\kappa_s T \( 2^{d_z + k d_s} - 1 \) }{ C_z \log (1/\epsilon) 2^{d_z + k d_s} } \) }{ (d_z + k d_s) \log 2 } \ge 1, 
    \end{align*}
    which implies 
    \begin{align*} 
        k \le \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } . 
    \end{align*} 

    Since $ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z > 0 $, the high probability optimality gap in the theorem statement is true for any fixed $ k \in \( 0, \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } \] $. 

\end{proof} 



------------------------------------------------------------


% \subsection{Only Very Few Batches Are Needed}  

% \begin{definition}
%     \label{def:opt-batch}
%     Denote $c_1 = \frac{d_z-1+k d_s }{(d+k d_s )(d_z+k d_s )}\log \frac{T}{\log T}$, $ c_{i+1} = \eta c_i,i\geq 1$, where $\eta = \frac{d+1-d_z}{d+k d_s }$. Let $a_n = \lfloor \sum_{i=1}^n c_i\rfloor$, $b_n = \lceil \sum_{i=1}^n c_i\rceil$. Define sequence $\{r_m\}$ as $r_m = 2^{-a_n}$ for $m = 2n-1$ and $r_m = 2^{-b_n}$ for $m = 2n$ (Here we suppose $\{r_m\}$ is a strictly decreasing sequence, see Remark \ref{rm:batch} for details). Define sequence $\{\alpha_m\}$ as $\alpha_m = r_m^k,k>0$.
% \end{definition}

% \begin{theorem} 
%     \label{thm:opt-batch} 
%     Instate Assumption \ref{assumption:lip}. Apply the sequence $\{r_m\}$ in Definition \ref{def:opt-batch} to Algorithm \ref{alg:large-d}. 
%     Let $T$ be the total time horizon such that $ (d+1-d_z) \log \frac{T}{\log T} - d d_z > 0 $ and let $\epsilon = \frac{1}{T^2}$. Let $ k \in \( 0, \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} \] $. 
%     % With fixed budget $T$, 
%     % the final simple regret satisfies 
%     Then with probability exceeding $1 - \frac{1}{T}$, the final optimality gap satisfies  
%     \begin{equation*} 
%         f^*_q - Y^{\max}_M \leq cL\left(\frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }},
%     \end{equation*} 
%     where $M$ denotes the last batch, $Y^{\max}_M$ is the estimate of $f^*_q$ after $M$ batches and $c$ is a constant independent of $T$. Moreover, only $2\times \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} +1$ total batches are needed to achieve this simple regret.
% \end{theorem} 




\begin{proof}
    Following an argument similar to that for Corollary \ref{cor1}, we conclude the proof. 
\end{proof}


% --------------------------------------------

% Note that to ensure at least one round of narrowing. We need to ensure 
% \begin{align*} 
%     \frac{\log \log \frac{T}{\log T} - \log (d_z + k d_s)}{ \log \frac{d+k d_s}{d+1 - d_z} } \ge 1, 
% \end{align*} 
% which implies 
% \begin{align*} 
%     && & k > \frac{1-d_z}{d_s}, \\
%     && & k 
%     \le 
%     \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} .
% \end{align*} 



% With this choice of $k$, the simple regret, with probability exceeding $1 - \frac{1}{T}$, is bounded by  
% \begin{align*}
%     c L \( \frac{T}{\log T} \)^{- p (T, d, d_z, d_s) }, 
% \end{align*}
% where $p(T,d, d_z,d_s) = \frac{ \frac{\sqrt{(d+d_z)^2 + 4 \( (d+1-d_z)\log \frac{T}{\log T} - d d_z \) } - (d+d_z)}{2d_s} + 1}{ \frac{\sqrt{(d+d_z)^2 + 4 \( (d+1-d_z) \log \frac{T}{\log T} - d d_z \) } - (d+d_z)}{2}  + d_z} $. 

% -------------------------------------------- 


\begin{lemma}
    \label{lem:nm}
    When $\kappa \in (0,1]$, $\alpha_m$ defined in Definition \ref{def:opt-batch} satisfies
    \begin{equation*}
        -\frac{1}{\log (1-\kappa \alpha_m^{d_s} )} \leq \frac{1}{\alpha_m^{d_s} \kappa}, \forall m \geq 1
    \end{equation*}
    In particular, for $n_m = \frac{\log \epsilon}{\log (1-\kappa_s  \alpha_m^{d_s})}$, it holds that $n_m \leq \frac{\log (1/\epsilon)}{\kappa_s \alpha_m^{d_s}}$.
\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:nm}]
    Let $g(m) = -\frac{1}{\alpha_m^{-d_s } \log (1-\kappa \alpha_m^{ d_s })}$. From the fact that the sequence $\{\alpha_m^{d_s}\}$ is decreasing with respect to $m$ and $h(x) = -\frac{1}{x^{-1} \log(1-\kappa x)}$ is a decreasing function regarding $x \in (0,1]$, we know $\{g(m)\}$ is a sequence increasing with $m$. Since $0 < \eta < 1$, we have $\sum_{i=1}^{\infty} c_i = \frac{c_1}{1-\eta} < \infty $, which implies that both $\lim_{n\rightarrow +\infty} 2^{-kd_s \lfloor \sum_{i=1}^n c_i \rfloor} $ and $\lim_{n\rightarrow +\infty} 2^{-kd_s \lceil \sum_{i=1}^n c_i \rceil} $ are strictly larger than $0$. Hence, 
    \begin{equation*}
        \lim_{m\rightarrow +\infty} g(m) \leq \lim_{x\rightarrow 0} -\frac{x}{\log (1-\kappa x)} = \frac{1}{\kappa}\\
    \end{equation*}
    We thus obtain $g(m)\leq \frac{1}{\kappa}, \enspace i.e.\enspace -\frac{1}{\log (1-\kappa \alpha_m^{ d_s })} \leq \frac{1}{\alpha_m^{ d_s } \kappa}$.
\end{proof}


\iffalse
\begin{proof}[Proof of Theorem \ref{thm:opt-batch}]
    Denote $\tilde{r}_n = 2^{-\sum_{i=1}^n c_i}$. 
    
    When $m = 2n-1$, $r_m \geq \tilde{r}_n, r_{m-1} \leq \tilde{r}_{n-1}$. 
    Since $\Delta_x \leq 3Lr_{m-1}$ for any $x \in \cup_{q_m\in \mathcal{A}_m}q_m$, any cube in $\mathcal{A}_{m-\frac{1}{2}}$ is a subset of $S(3Lr_{m-1})$. Therefore,
    \begin{equation*}
        |\mathcal{A}_{m-\frac{1}{2}}| \leq N_{r_{m-1}} \leq C_z r_{m-1}^{-d_z}.
    \end{equation*}
    After partitioning $\mathcal{A}_{m-\frac{1}{2}}$ into $\mathcal{A}_m$, we get
    \begin{equation*}
        |\mathcal{A}_m| = \left(\frac{r_{m-1}}{r_m}\right)^d |\mathcal{A}_{m-\frac{1}{2}}| \leq \left(\frac{\tilde{r}_{n-1}}{\tilde{r}_n}\right)^d \cdot C_z r_{m-1}^{-d_z}.
    \end{equation*}
    Denote the total budget of the $m$-th batch as $N_m$, then
    \begin{equation*}
    \begin{aligned}
        && N_m = |\mathcal{A}_m| \cdot n_m & 
        \leq \left(\frac{r_{m-1}}{\tilde{r}_n}\right)^d \cdot C_z r_{m-1}^{-d_z} \cdot \frac{\log (1/\epsilon)}{\kappa_s \alpha_m^{ d_s }} 
        \leq \frac{C_z \log (1/\epsilon)}{\kappa_s } \cdot \frac{ \tilde{r}_{n-1}^{d-d_z+1} \cdot \tilde{r}_n^{-k d_s -d} }{r_{m-1}} \\
        && & = \frac{C_z \log (1/\epsilon)}{\kappa_s r_{m-1}} \cdot 2^{(d_z+k d_s -1)\sum_{i=1}^{n-1}c_i + (k 
        d_s +d)c_n}
    \end{aligned}
    \end{equation*}
    Define $C_n = (d_z+k d_s -1)\sum_{i=1}^{n-1}c_i + (k d_s +d)c_n$, then $C_n - C_{n-1} = (d_z-d-1)c_{n-1} + (k d_s +d)c_n = 0$. So for any $n > 1$, we have $C_n = C_1 = (k d_s +d)c_1$. Consequently, we obtain the upper bound of $N_m$ for $m = 2n-1$ as follows,
    \begin{equation*}
        N_m \leq \frac{C_z \log (1/\epsilon)}{\kappa_s r_{m-1}} \cdot \left(\frac{T}{\log T}\right)^{\frac{d_z+k d_s -1}{d_z+k d_s }}.
    \end{equation*}

    When $m = 2n$, $r_{m-1} = \min\{r_{m-2},2^{-a_n} \} = \min \{2^{-b_{n-1}} , 2^{-a_n} \}$. $r_{m-1} = r_{m-2}$ only happens when $\lceil \sum_{i=1}^{n-1}c_i \rceil > \lfloor \sum_{i=1}^{n}c_i \rfloor$. Under this circumstance, $r_m = 2^{-\lceil \sum_{i=1}^{n}c_i \rceil } = 2^{-\lfloor \sum_{i=1}^{n}c_i \rfloor - 1} \geq r_{m-2}$, which contradicts the assumption that $\{r_m\}$ is strictly decreasing. Therefore, it must hold that $r_{m-1} = 2^{-a_n} = 2^{-b_n + 1} = 2r_m$. We conclude from Lemma \ref{lem:opt-gap} that any cube in $\mathcal{A}_m$ is a subset of $S(6Lr_m)$.  Therefore,
    \begin{equation*}
        N_m = |\mathcal{A}_m| \cdot n_m 
        \leq \frac{C_z\log (1/\epsilon)}{\kappa_s} \cdot r_m^{-d_z} \cdot r_m^{-k d_s }
    \end{equation*}

    Since the total budgets of all $M$ batches is $T$, 
    \begin{equation*}
    \begin{aligned}
        && T & \leq \sum_{m=2n-1, m\leq M} N_m + \sum_{m=2n, m\leq M} N_m \\
        && & \leq \frac{2C_z}{\kappa} \left( \sum_{m=2n-1, m\leq M} \frac{1}{r_{m-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k d_s }} + \sum_{m=2n, m\leq M} r_m^{-d_z-k d_s } \cdot \log T\right)
    \end{aligned}
    \end{equation*}
    
    From the assumption that $\{r_m\}$ is strictly decreasing, we know $r_m \leq \frac{1}{2}r_{m-1}$ for any $m$. When $M$ is odd, $\sum_{m=2n-1,m\leq M} \frac{1}{r_{m-1}} \leq \left( \sum_{n=0}\frac{1}{2^n} \right) \cdot \frac{1}{r_{M-1}} = \frac{2}{r_{M-1}}$, $ \sum_{m=2n, m\leq M} \frac{1}{r_m^{d_z+k 
    d_s }} \leq \left(\sum_{n=0} \frac{1}{2^{n(d_z+k d_s )}}\right) \cdot {\frac{1}{r_{M-1}^{d_z+k d_s }}} = \frac{2}{r_{M-1}^{d_z+k 
    d_s }}$. Therefore, 
    \begin{equation*}
        T \leq \frac{4C_z}{\kappa_s} \cdot \left( \frac{1}{r_{M-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k 
        d_s }} + \frac{1}{r_{M-1}^{d_z+k d_s }} \cdot \log T \right).
    \end{equation*}
    Set $C = \max\{8C_z/\kappa_s,(8C_z/\kappa_s)^{\frac{1}{d_z+k 
    d_s }}\}$. If $r_{M-1} > C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$, then 
    \begin{equation*}
        \frac{4C_z}{\kappa_s} \cdot \left( \frac{1}{r_{M-1}} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} \left(\log T\right)^{\frac{1}{d_z+k d_s }} + \frac{1}{r_{M-1}^{d_z+k d_s }} \cdot \log T \right) < T,
    \end{equation*} 
    which yields contradiction. So we obtain $r_{M-1} \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$, and $r_M \leq \frac{1}{2} C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$.

    Similarly, when $M$ is even, we have
    \begin{equation*}
        T \leq \frac{4C_z\log T}{\kappa_s} \cdot \left( \frac{1}{r_M} \cdot T^{\frac{d_z+k d_s -1}{d_z+k d_s }} + \frac{1}{r_M^{d_z+k d_s }}\right).
    \end{equation*}
    Implementing the same deduction process as when $M$ is odd, we get $r_M \leq C \times \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$.

    With $r_M$ upper bounded as above, the simple regret of the last batch $M$ can achieve an order smaller than or equal to $\mathcal{O}\left( \left( \frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }} \right)$:
    \begin{equation}
        \label{eq:simple-regret}
        f^*_q - Y^{\max}_M \leq \rho_M = L\alpha_M r_M = L r_M^{1+k } \leq cL\left(\frac{T}{\log T}\right)^{-\frac{1+k }{d_z+k d_s }},
    \end{equation}
    where $c$ is a constant.

    To see that only $ O (\log \log T) $ batches are needed, we note that $\tilde{r}_{M} = 2^{-\sum_{i=1}^{M} c_i} = 2^{-c_1 \cdot \frac{1-\eta^{M}}{1-\eta}} = \left( \frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s } + \frac{\eta^{M}}{d_z+k d_s }}$. By letting $\frac{\eta^{M^*}}{d_z+k d_s } \leq \frac{ \textcolor{red}{\tilde{C}} }{\log \frac{T}{\log T}}$ ($\tilde{C}$ is a constant determined in Remark \ref{rm:batch} ), that is, choosing $M^* \geq \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s ) \textcolor{red}{ - \log \tilde{C} } }{\log \frac{d+k d_s }{d+1-d_z}}$, we can achieve $\tilde{r}_{M^*} \leq \left(\frac{T}{\log T}\right)^{-\frac{1}{d_z+k d_s }}$. Since $r_m \leq \tilde{r}_{M^*}$ for $m\geq 2M^*$, only $2M^*+1$ batches are needed to achieve the simple regret in (\ref{eq:simple-regret}).
    

    Finally, the choice of $k$ in the final optimality gap is not arbitrary. 
    To ensure at least one round of narrowing, we need to ensure that $M \ge 1$. By (\ref{eq:lower-M-1}), it is sufficient to ensure that 
    \begin{align*}
        \frac{\log \log \frac{T}{\log T} - \log (d_z+k d_s )}{\log \frac{d+k d_s }{d+1-d_z}} \ge 1, 
    \end{align*}
    which implies 
    \begin{align*} 
        % \frac{1-d_z}{d_s} < 
        k 
        \le 
        \frac{ \sqrt{ \( d+d_z \)^2 + 4 \( \( d+1-d_z \)  \log \frac{T }{\log T} - d d_z \) } - (d+d_z) }{2 d_s} . 
        % k \le \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } . 
    \end{align*} 

    % Since $ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z > 0 $, the high probability optimality gap in the theorem statement is true for any fixed $ k \in \( 0, \frac{ \log_2 \(  \frac{ \kappa_s T + \sqrt{\kappa_s^2 T^2 - 4 C_z \log (1/\epsilon) \kappa_s T } }{2 C_z \log (1/\epsilon)} \) - d_z }{ d_s } \] $. 
\end{proof}
\fi



\begin{remark}
    \label{rm:batch}
    If $c_i \geq 1$ for $i = 1,2,\cdots,M^*$, then it must hold that $\lceil \sum_{i=1}^n c_i \rceil > \lceil \sum_{i=1}^{n-1} c_i \rceil$ for $n = 1,2,\cdots,M^*$, which implies that the odd terms of $\{r_m\}$ are strictly decreasing when $m = 1,2,\cdots,2M^*$. To ensure this, we let $c_{M^*} = c_1\eta^{M^*-1} \geq 1$, which is equivalent to $M^* \leq \frac{\log \log \frac{T}{\log T} + \log(d_z-1+kd_s) - \log (d_z+kd_s) - \ log(d+1-d_z) }{\log \frac{d + kd_s}{d+1-d_z}}$. Let $\log \tilde{C} \geq \log \frac{d+1-d_z}{d_z - 1 + kd_s}$ and let $T$ be large enough such that $\log \log \frac{T}{\log T} > \log (d_z + kd_s) + \log \tilde{C}$.
\end{remark}



% \begin{assumption}
%     \label{assumption:ord}
%     There exists $\kappa \in (0,1) $, such that for any $\alpha \in [0, \frac{ 1 }{2} ]$, and any cube $q \subseteq [0,1]^d$ 
%     \begin{align*} 
%         \Pr \( f ( X_q ) \le f_q^{\max} -  \alpha ( f_q^{\max} - f_q^{\min} ) \) 
%         \le 
%         1 - \kappa \alpha . 
%     \end{align*} 
% \end{assumption}







==> tex/order-stat-opt.tex <==
% \section{Via Order Statistics}


% Then we have 
% \begin{align*} 
%     \Pr \( f_q^{\max} - Y_q^{\max,n} \ge \epsilon \) 
%     = 
%     \Pr \( Y_{q}^{\max,n} \le f_q^{\max} - \epsilon \) 
%     = 
%     \prod_{i=1}^n \Pr \( f ( X_q^i ) \le f_q^{\max} - \epsilon \) 
%     \le 
%     (1 - \kappa \epsilon )^n . 
% \end{align*} 


% Let's assume that $ \Pr \( X_i \le x \) \ge  $. 

% Variance of $ X_n^{\max} $ satisfies 

% Define $ Y_q := f (X_q) $ where $  $ 
% Let $ $

==> tex/preliminary.tex <==
% \section{Settings and Preliminaries} 


\section{A Note on the Zooming Dimension} 

Throughout the paper, we will use the following conventions and notations. Firstly, we assume that the objective function is $L$-Lipschitz.
\begin{assumption}
    \label{assumption:lip}
    The objective function $f$ is $L$-Lipschitz. 
\end{assumption}

% Let $f : [0,1]^d \to \R$ be $L$-Lipschitz. 
For any cube $q \subseteq [0,1]^d$, we write 
\begin{align} 
    f_q^{\max} := \sup_{x \in q} f (x) \quad \text{ and } \quad f_q^{\min} := \inf_{x \in q} f (x) . \label{eq:fq} 
\end{align} 
Also, we define $ f^* : =  \sup_{x \in [0,1]^d} f (x) $, $x^* = \arg\max_{x \in [0,1]^d} f (x)$ and define $\Delta_x := f^* - f (x)$. Throughout the paper, we will use some bandit terminology. For example, by an arm $x$ we refer to a point $x$ in the domain. By pulling/playing an arm $x$, we mean choosing a point $x$ in the domain. 


 

\subsection{Doubling Metric Spaces and the $([0,1]^d, \| \cdot \|_\infty)$ Metric Space}

By the Assouad's embedding theorem \citep{assouad1983plongements}, the (compact) doubling metric space $ ( \mathcal{A} , d_{\mathcal{A}} ) $ can be embedded into a Euclidean space with some distortion of the metric; See \citep{pmlr-v119-wang20q} for more discussions in a machine learning context. Due to existence of such embedding, the metric space $ ([0,1]^d, \| \cdot \|_{\infty})  $, where metric balls are hypercubes, is sufficient for the purpose of our paper. For the rest of the paper, we will use hypercubes in algorithm design for simplicity, while our algorithmic idea generalizes to other doubling metric spaces.


\subsection{Zooming Numbers and Zooming Dimensions} 
\label{sec:zooming} 

An important concept for bandit problems in metric spaces is the zooming number and the  zooming dimension \citep{kleinberg2008multi, bubeck2008tree, slivkins2011contextual}, which we discuss now. 
% For any function $f : [0,1]^d \to \R$ and $x \in [0,1]^d$, we 

% Let's recap the zooming number and zooming dimension. 
Define the set of $\rho$-optimal arms as $ S (r) = \{ x \in [0,1]^d : \Delta_x \le \rho \} $. For any $\rho=2^{-i}$, the decision space $[0,1]^d$ can be equally divided into $2^{di}$ cubes with edge length $\rho$, which we call \textit{standard cubes} (also referred to as dyadic cubes). 
% Henceforth, all cubes are standard cubes unless otherwise noted. 
The $\rho$-zooming number is defined as \textcolor{red}{\quad need to revise, $S(6\rho)$ or $S(8\rho)$}
\begin{align*} 
    N_\rho := \#\{C: \text{$C$ is a standard cube with edge length $\rho$ and $C\subset S( \textcolor{red}{8L} \rho )$}\} . 
\end{align*} 

In words, $N_\rho$ is the $\rho$-packing number of the set $S(\textcolor{red}{8L}\rho)$ in terms of standard cubes. % The upper bound of regret for Lipschitz bandits problem without batched setting
% (e.g., \citet{slivkins2011contextual}) \textcolor{red}{add some reference about zooming algorithm}
% takes the form
% \begin{align}\label{sliv_bound}
%     \E [R(T)]\leq R_z(T)\triangleq C_0\cdot\inf_{r_0}\left\{r_0T+\sum_{r=2^{-i},r\geq r_0}\frac{N_r}{r}\log T\right\},
% \end{align} 
% where $C_0>0$ is a constant. 
The zooming dimension is then defined as 
\begin{align*} 
    d_z := \min \{  d\geq0: \exists a>0,\;N_\rho \le a \rho^{-d},\;\forall \rho = 2^{-i} \text{ for some $i \in \mathbb{N}$} \}. 
\end{align*} 
Moreover, we define the zooming constant $C_z$ as the minimal $a$ to make the above inequality true for $d_z$, $C_z=\min\{  a>0:\;N_\rho \le a \rho^{-d_z},\;\forall \rho=2^{-i} \text{ for some $i \in \mathbb{N}$} \}$.

Zooming dimension $d_z$ can be significantly smaller than ambient dimension $d$ and can be zero. For a simple example, consider a problem with ambient dimension $d=1$ and expected reward function $\mu(x)=x$ for $0\leq x\leq1$. Then for any $\rho=2^{-i}$ with $i\geq4$, we have $S(2 \rho)=[1- 2\rho,1]$ and $N_\rho=16$. Therefore, for this problem the zooming dimension equals to $0$, with zooming constant $C_z=16$. \textcolor{red}{(revise this example)} 





% \subsection{Goal}

% \begin{itemize} 
%     \item Our goal is to optimize 
% \end{itemize} 


% \subsection{CVaR}
       
% Conditional Value at Risk (CVaR) is an important statistic of distributions and finds its applications in domains like finance. 

% \begin{definition}[VaR and CVaR]
%     \label{def:cvar}
%     Fix $\alpha \in (0,1]$. The value at risk at level $\alpha$ (or upper $\alpha$-quantile) of a random variable $X$ is $\mathrm{VaR}_\alpha (X) := \inf \left\{ \xi | \Pr (X \le \xi)  \ge \alpha \right\}$. The conditional value at risk at level $\alpha$ of a random variable $X$ is defined as
%     \begin{align}
%         \mathrm{CVaR}_\alpha (X) = \mathrm{VaR}_\alpha (X) + \frac{1}{1-\alpha} \E \( \left\lfloor X - \mathrm{VaR}_\alpha (X) \right\rfloor_+ \), 
%     \end{align}
%     where $ \left\lfloor z \right\rfloor_+ = \max\( 0, z \)$ for any number $z$. 
%     When the random variable $X$ has positive density at $ \mathrm{VaR}_\alpha (X) $, then 
%     \begin{align}
%         \mathrm{CVaR}_\alpha (X) = \E \[ X | X \ge \mathrm{VaR}_\alpha (X) \]. 
%         % (cite this proposition. )
%     \end{align} 
% \end{definition} 

% % \begin{remark} 
% In different contexts, the quantities $ \mathrm{VaR}_\alpha $ and $\mathrm{CVaR}_\alpha$ may be defined with respect to either upper quantile or lower quantile. For the purpose of this paper, we stick to the version defined in Definition \ref{def:cvar}. 
% % \end{remark} 


% \subsection{CVaR Estimation}

% We use the recent results by \cite{prashanth2020concentration}. The Let $\{X_i\}_{i=1}^n$ be $n$ $i.i.d.$ samples drawn from the distribution
% of $X$. Let $\{X_{[i]}\}_{i=1}^n$ be the order statistics of $\{X_i\}_{i=1}^n$ i.e., $X_{[1]} \le X_{[2]} \le \cdots \le X_{[n]}.$ Let $\wh{F}_n(\cdot)$ be the empirical distribution function calculated using $\{X_i\}_{i=1}^n$, defined as
% \begin{align*}
%     \wh{F}_n (x) 
%     := 
%     \frac{1}{n} \sum_{i=1}^n \ind_{ \[ X_i \le x\] } , \quad \forall x \in \R . 
% \end{align*}
% Notice that CVaR is a conditional expectation, where the conditioning event
% requires VaR. Thus, CVaR estimation requires VaR to be
% estimated as well. Let $\wh{v}_{n,\alpha}$ and $\wh{c}_{n,\alpha}$ denote the estimates of VaR and CVaR at level $\alpha$ using the $n$ samples $\{X_i\}_{i=1}^n$.
% These quantities are defined as follows (Serfling, 2009): 
% \begin{align*}
%     \wh{v}_{n,\alpha} &= X_{[\lceil n \alpha \rceil ]} \\
%     \wh{c}_{n,\alpha} &= \frac{1}{n(1-\alpha)} \sum_{i=1}^n X_i \ind_{ \[ X_i \ge \wh{v}_{n,\alpha} \] } . 
% \end{align*}


% \begin{theorem}[\cite{prashanth2020concentration}] 
%     \label{thm:cvar-concen} 
%     The $r.v.$ $X$ is continuous with a density $f_X$ that satisfies the following condition: There exist universal constants $\eta, \delta > 0$ such that $f_X(x) > \eta$ for all $ x \in \[ \text{VaR}_\alpha (X) - \frac{\delta}{2} , \text{VaR}_\alpha (X) + \frac{\delta}{2} \] $ and all $\alpha \in (0,1]$. 
    
%     Let $\{X_i\}_{i=1}^n$ be $n$ $i.i.d.$ samples drawn from the distribution of $X$. 
%     Let $\wh{c}_{n,\alpha}$ be the $\mathrm{CVaR}$ estimate based on $\{X_i\}_{i=1}^n$. If $X_i, i = 1, \cdots , n$ are $\sigma$-sub-Gaussian. 
%     Then, for any $\epsilon > 0$, we have
%     \begin{align*}
%         \Pr \( \left| \wh{c}_{n, \alpha} - \mathrm{CVaR}_\alpha (X) \right| > \epsilon \) 
%         \le 
%         2 \exp \( - \frac{n \epsilon^2 (1-\alpha)^2}{8 \sigma^2} \) + 4 \exp \( -\frac{n (1 - \alpha)^2 \eta^2 \min ( \epsilon^2, 4 \delta^2 ) }{64} \) 
%     \end{align*} 
% \end{theorem} 



==> tex/scattering.tex <==

\section{From the Zooming Dimension to the Scattering Dimension}


\subsection{The Curse and Blessing of Zooming Dimension} 


The term zooming dimension was coined to characterize the landscape of the underlying function \citep{kleinberg2008multi,bubeck2011x}. 
According to classical theory, functions with smaller zooming dimension are easier to learn, because larger zooming dimension means more arms are similar and harder to distinguish. 
On the other hand, larger zooming dimension also implies a larger near-optimal region, which increases the chance of finding a near-optimal region by a random sample in the domain. 
To sum up, a function with large zooming dimension has two contrasting features: 
% \begin{itemize} 

\noindent $\bullet$ \textbf{(The Curse of Zooming Dimension)} 
When the zooming dimension $d_z$ is large, the difference between arms is small. From this perspective, the problem is hard when $d_z$ is large. 

\noindent $\bullet$ \textbf{(The Blessing of Zooming Dimension)} When the zooming dimension $d_z$ is large, the region of near-optimal arms is large. From this perspective, the problem is easy when $d_z$ is large. 
% \end{itemize} 

However, existing theory only focuses on the negative side of zooming dimension and shows that the regret rate deteriorates as $d_z$ increases. The positive effect of zooming dimension has been largely overlooked. In this paper, we propose a new notion that captures the blessing side of zooming dimension. 

% However, existing theory only captures one side of the story. Namely, the regret rate worsens as $d_z$ increases. While the cursing side of zooming dimension is well-studied by existing theory, the blessing side of zooming has been largely overlooked. In this paper, we introduce a new concept that captures the blessing side of zooming dimension. 

\subsection{The Scattering Dimension} 

As discussed above, the zooming dimension alone is not sufficient to efficiently instruct the difficulty level of finding a near-optimal arm. To address this issue, we introduce the concept of \emph{scattering dimension} in Definition \ref{def:ord}. 


\begin{definition}
    \label{def:ord}
    % We assume that the following items are true. 
    % \begin{itemize}
    For a Lipschitz function $f : [0,1]^d \to \R$ whose maximum is obtained at $x^*$, define the scattering dimension $ d_s $ of $f$ as  
    \begin{align*}
        d_s := \inf \{ \tilde{d} \ge 0 :&\; \exists \kappa \in (0,1], \text{ such that } \Pr \( f ( X_q ) < f_q^{\max} -  \alpha ( f_q^{\max} - f_q^{\min} ) \) 
        \le 
        1 - \kappa \alpha^{ \tilde{d} }, \\ 
        &\; \forall \text{ cube } q \subseteq [0,1]^d \text{ with $x^* \in q$},\;  \forall \alpha \in (0,\frac{1}{2}] \} . 
    \end{align*} 

    In addition, we define the scattering constant $\kappa_s$ to be 
    \begin{align*}
        \kappa_s := \max \{ \kappa \in (0,1] :&  \Pr \( f ( X_q ) < f_q^{\max} -  \alpha ( f_q^{\max} - f_q^{\min} ) \) 
        \le 
        1 - \kappa \alpha^{d_s}, \\ 
        &\; \forall \text{ cube } q \subseteq [0,1]^d \text{ with } x^* \in q,\;  \forall \alpha \in (0,\frac{1}{2}] \} . 
    \end{align*}
\end{definition} 

% \textcolor{red}{In Definition1, need to specify that $q$ is a cube but not an arbitrarily shaped region?}


As Definition \ref{def:ord} implies, lower scattering dimension makes a near-optimal region easier to find by random sampling. In the classic theory based on zooming dimension, we also know that higher zooming dimension implies a larger near-optimal region. This indicates that there is a trade-off between zooming dimension and scattering dimension: a function with large zooming dimension tends to have small scattering dimension, and vice versa.

% From the definition, we see that smaller scattering dimension makes it easier for a random guess to hit a near-optimal region. 
% In the classic theory based on zooming dimension, we know that larger zooming dimension means that the near-optimal region is large. This suggests that a function with large zooming dimension tends to have small scattering dimension, and vice versa. 

\subsubsection{The Zooming-Scattering Trade-off} 

We will illustrate the trade-off between zooming and scattering dimension via the following example function. 
% illustrate the characteristics of zooming dimension via the following example function $g_p$. 
% As its definition implies, functions with larger zooming dimension 
Let $g_p(x) = 1 - \frac{1}{p} \| x \|_\infty^p$ be a function defined over $[0,1]^d$ for some $d \ge 1$ and $p\ge1$. Figure \ref{fig:demo} illustrates $g_p $ with $p=1,3,5,10$ and $d = 1$. We observe the following property for such function $g_p$. 
\begin{observation}
    \label{obs:gp}
    Let $p \ge 1$, and let $ g_p (x) : [0,1]^d \to \R$ be defined as $ g_p (x) = 1 - \frac{1}{p} \| x \|_\infty^p $. The zooming dimension of $g_p$ is $d_z = \frac{p-1}{p} d $. 
\end{observation}

\begin{figure}
    \centering
    \includegraphics[width = 0.45 \textwidth]{figures/gp.png} 
    % \includegraphics[width = 0.45 \textwidth]{figures/p10.png} 
    \caption{The plots of $ g_p $ with $p = 1,3,5,10$.} 
    \label{fig:demo} 
\end{figure}


% Since $ g_p (x) = 1 - \frac{1}{p} \( \max_i x_i \)^p $, we know 

Clearly $ g_p (x) $ is 1-Lipschitz. By definition of $g_p$, the $8L \rho$-optimal arms form a cube $ [0, ( 8L p \rho )^{\frac{1}{p}} ]^d $. We need $ \( 8L p \)^{\frac{d}{p}} \rho^{\frac{p-1}{p} d } $ cubes of edge-length $ \rho $ to cover $ [0, (8L p \rho)^{\frac{1}{p}} ]^d $. Thus the zooming dimension of $ g_p $ is $d_z = \frac{p-1}{p} d$.

As $p$ approaches infinity, the zooming dimension converges to $d$ and the zooming constant converges to 1. According to classic theory \citep{kleinberg2008multi,bubeck2011x}, the performance of an optimal-seeking algorithm deteriorates as $p$ increases. The intuition behind this theory is that when $d_z$ is large, the arms are nearly indistinguishable. However, the function landscape of $g_p$ flattens as $p \to \infty $, and the problem of finding a near-optimal point becomes easier. In fact, when $p$ is large, $g_p$ has a small scattering dimension, and a random point in $[0,1]^d$ is close to optimal. 



==> tex/sketch-old.tex <==

\begin{assumption} 
    \label{assumption} 
    We assume the function of interest $f$ is defined over a bounded Euclidean domain $\mathcal{X} \subseteq [0,1]^d$. 
    For easier representation, we take $\mathcal{X} = [0,1]^d$ unless otherwise stated. 
\end{assumption} 

% \begin{definition}[Identifiable Function]
% A function $f : [0,1]^d \rightarrow \mathbb{R}$ is said to be $\eta$-identifiable if there exists $ B \subseteq [0,1]^d $ such that the followings are both satisfied:
% \begin{enumerate} 
%     \item $B$ is convex and $ |B| = \eta $; 
%     \item for all convex $B' \subseteq B$, $ \inf_{x\in B'} f (x) \ge \sup_{x \in \mathcal{X} \setminus B' } f (x)  $. 
% \end{enumerate} 
% % for all $ $
% \end{definition} 

\begin{definition}[Identifiable Function and Identifier Set]
    \label{def:id}
    % An equivalent definition of identifiable function is as follows. 
    A function $f : [0,1] \rightarrow [0,1]$ is said to be $\eta$-\textbf{identifiable} if for all intervals $ I = [a,b] \subseteq [0,1] $ of length smaller than or equal to $\eta$ the followings are satisfied:
    \begin{enumerate} 
        % \item $I = [a,b]$ is an interval of length smaller $\eta$. 
        \item $f$ is differentiable and $m$-strongly concave on $I$. 
        \item $ f (a) = f (b) \ge \sup_{x \in [0,1] \setminus I} f (x)$. 
    \end{enumerate} 
    We call such an interval $I$ an $\eta$-\textbf{identifier} set of $f$ or simply an $\eta$-identifier of $f$. 
    
    % Let $\eta^{\max}$ be the maximum $\eta$ such that $f$ is $\eta$ identifiable. 
    An interval $I$ is called the maximal identifier set of $f$ or simply maximal identifier of $f$ if 
    $$
    I = \bigcup \left\{ I': I' \text{ is } \eta \text{-identifiable for some } \eta \in [0,1] \right\} . 
    $$
    Finally, given a function $f$, we say a number $\eta$ is  $f$-\textbf{admissible} if $f$ has an $\eta$-identifier. 
\end{definition} 

Intuitively, identifiable functions are functions that are strongly concave (or convex) near its unique global maximum (or minimum). 

Some direct results of Definition \ref{def:id} (and Assumption \ref{assumption}) are summarized in Proposition \ref{prop:basic}. 

\begin{proposition} 
    \label{prop:basic}
    
    \begin{enumerate}
        \item Concave functions are  $\eta$-identifiable for some $ \eta \le 1 $. 
        \item Let $\eta$ be an arbitrary $f$-admissible number. If $x^*$ is the maximizer of function $f$, then $ x^* \in I$ for any $\eta$-identifiable interval $ I $. 
    \end{enumerate}
\end{proposition} 

For easier discussion, we introduce the following terminology in Definition \ref{def:partition}. 

% \begin{definition}[Regular Partitions]
% \label{def:partition}
%     A partition $\mathcal{P}$ is called a regular partition if any $P \in \mathcal{P}$ is a rectangle. In addition, a partition $ \mathcal{P} $ is called a binary regular partition if $\mathcal{P}$ is a regular parition and $|\mathcal{P}| = 2$, where $|\mathcal{P}|$ is the cardinality of $\mathcal{P}$. 
% \end{definition} 


\begin{definition}[Paired Partitions] 
\label{def:partition}
    % We say two (hyper-)rectangles $R$ and $R'$ are parallel if $R \subseteq R'$ and $ R' \setminus R $ is a rectangle. 
    % If two rectangles $R$ and $R'$ are parallel, we write $R \parallel R'$. 
    If $\mathcal{P} = \{ I_1, I_2 \}$ and $\mathcal{Q} = \{ I_1', I_2 \}$ be two partitions (of the same interval) such that $I_1, I_2, I_1', I_2'$ are all intervals, we say $\mathcal{P} $ and $\mathcal{Q}$ are paired partitions. 
    % Equivalently, two partitions $\mathcal{P} = \{ P_1, P_2 \}$ and $\mathcal{Q} = \{ Q_1, Q_2 \}$ are paired partitions if $P_i \parallel Q_j$ . 
    % A partition $\mathcal{P}$ is called a regular partition if any $P \in \mathcal{P}$ is a rectangle. In addition, a partition $ \mathcal{P} $ is called a binary regular partition if $\mathcal{P}$ is a regular parition and $|\mathcal{P}| = 2$, where $|\mathcal{P}|$ is the cardinality of $\mathcal{P}$. 
\end{definition} 

% \begin{proposition} 
%     Two parallel rectangles $R$ and $R'$ can be written as $R= [a,b] \times \prod_{i=1}^{d-1} [a_i, b_i]$ and $R' = [a',b'] \times \prod_{i=1}^{d-1} [a_i', b_i']$ such that $a = a' $, $b \neq b'$ and $(a_i, b_i ) = (a_i', b_i' ) $ for all $i = 1, 2, \cdots, d-1$. 
% \end{proposition} 

\begin{definition}[] 
    \label{def:rectangle-minus} 
    Let $R$ and $R'$ be two parallel rectangles such that $R = [a,b] \times \prod_{i=1}^d [a_i, b_i] $ and $R' = [a,b'] \times \prod_{i=1}^d [a_i, b_i] $. We define the operation $R \jian R' := |b - b'|$. 
\end{definition} 

% In Figure \ref{fig:pair-partition}, we give an example of parallel rectangles and paired partitions. 

% We use $x^*$ to denote the maximizer of $f$, and use $$ 

\begin{lemma} 
    \label{lem:core}
    Let $ f $ be an $\eta$-identifiable function whose maximum is obtained at $x^*$. Let $ B $ be an $\delta$-identifier of $f$ ($\delta \le \eta$). 
    Let $\mathcal{P} = \{ P_1, P_2 \}$ and $  \mathcal{Q} = \{ Q_1, Q_2 \}$ be two paired partitions. If $ Q_1 \parallel P_1$ and $ P_1 \jian Q_1 = \delta$, then $P^* \in \arg \max_{P \in \{P_1, P_2, Q_1, Q_2 \} } \cvar_\alpha ( f (X|_P)) $ contains $x^*$ for $\alpha = $ what sth what. 
\end{lemma} 

\begin{proof}
    % Since $ \big| |P_1| - |Q_1| \big| = \delta $ and $\mathcal{P}$ and $\mathcal{Q}$ are paired partitions, one of $P_1, P_2, Q_1, Q_2$ must contain $ x^* $. 
    % Without loss of generality, let $P_1 \parallel Q_1$. we consider two cases: In \textbf{Case I}, $B \subseteq P_1 $ and $B \subseteq Q_1$ contain $B$. In \textbf{Case II}, $B \subseteq P_1$ and $ B \nsubseteq Q_1 $ and $B \nsubseteq Q_2$. 
    
    \textbf{Case I:} $B \subseteq P_1 $ and $B \subseteq Q_1$. Let $\alpha = \eta^d$. By item 3 in Definition \ref{def:id}, we know $\cvar_\alpha ( f (X|_{P_1})) \ge $
    % $B \subseteq P_1$ and $ B \nsubseteq Q_1 $ and $B \nsubseteq Q_2$. Without loss of generality, 
\end{proof}

Next we introduce Lemma \ref{lem:core}, which lays the foundation of our algorithms. 

% \begin{lemma} 
%     \label{lem:core}
%     Let $ f $ be an $\eta$-identifiable function whose maximum is obtained at $x^*$. Let $\mathcal{P} = \{ P_1, P_2 \}$ and $  \mathcal{Q} = \{ Q_1, Q_2 \}$ be two binary regular partitions. For a set $P \subset [0,1]^d$, let $X|_P$ be the random variable $ X|_P \sim \text{Uniform} (P)$. If $\big| |P_1| - |Q_1| \big| \ge \eta$, then $P^* \in \arg \max_{P \in \{P_1, P_2, Q_1, Q_2 \} } \cvar_\alpha ( f (X|_P)) $ contains $x^*$ for $\alpha = $what sth what. 
% \end{lemma} 


% \begin{proof} 
%     Let $B $ be an identifier set of $f$. 
    
%     For 
    
    
    
%     \textbf{Case I:} $ B \subseteq P_1  $ (or $B \subseteq P_2$) and $ B \nsubseteq Q_1 $ and $ B \nsubseteq Q_2 $.  
% \end{proof} 



\begin{lemma}[CVaR gap]
    Let $ f : [0,1] \rightarrow [0,1] $ be an $\eta$-identifiable function. Let $I \subset [0,1]$ be a $\delta$-identifier of $f$ ($\delta \le \eta \; sth$). If $\mathcal{P} = \{ J_1, J_2 \}$ is a partition such that $J_1 \supseteq I$, then $\cvar_\delta (f(X|_{P_1})) \ge \cvar_\delta (f(X|_{P_2})) +  $. 
\end{lemma}

\begin{proof} 
    test 
\end{proof} 
